Uncertainty-Aware Attention for Reliable Interpretation and Prediction

Attention mechanism is effective in both focusing the deep learning models on relevant features and interpreting them. However, attentions may be unreliable since the networks that generate them are often trained in a weakly-supervised manner. To overcome this limitation, we introduce the notion of input-dependent uncertainty to the attention mechanism, such that it generates attention for each feature with varying degrees of noise based on the given input, to learn larger variance on instances it is uncertain about. We learn this Uncertainty-aware Attention (UA) mechanism using variational inference, and validate it on various risk prediction tasks from electronic health records on which our model significantly outperforms existing attention models. The analysis of the learned attentions shows that our model generates attentions that comply with clinicians' interpretation, and provide richer interpretation via learned variance. Further evaluation of both the accuracy of the uncertainty calibration and the prediction performance with "I don't know" decision show that UA yields networks with high reliability as well.

==> IDK.tex <==
\begin{figure*}
\small
\begin{tabular}{c c c c c c}
\hspace{-0.12in}
\includegraphics[height=2.2cm]{figure/IDK_physionet_mortality.pdf}&
\hspace{-0.15in}
\includegraphics[height=2.2cm]{figure/IDK_physionet_stay.pdf}&
\hspace{-0.15in}
\includegraphics[height=2.2cm]{figure/IDK_physionet_cardiac.pdf}&
\hspace{-0.15in}
\includegraphics[height=2.2cm]{figure/IDK_physionet_recovery.pdf}&
\hspace{-0.15in}
\includegraphics[height=2.2cm]{figure/IDK_pancreatic.pdf}&
\hspace{-0.15in}
\includegraphics[height=2.2cm]{figure/IDK_sepsis.pdf}\\
\hspace{-0.12in}(a) PhysioNet & (b) PhysioNet & (c) PhysioNet & (d) PhysioNet & (e) Pancreatic & (f) MIMIC \\
  - Mortality & - Stay $<$ 3 & - Cardiac & - Recovery & Cancer & - Sepsis \\
\end{tabular}
\vspace{-0.16in}  
\caption{\small Experiments on prediction reliability. The line charts show the ratio of correct predictions and the ratio of incorrect predictions as a function of the uncertainty threshold on all datasets.}\label{fig:ratio}
\vspace{-0.25in}  
\end{figure*}


%Previous IDK setting
%\begin{figure*}
%\small
%\begin{tabular}{c c c c c c}
%\hspace{-0.28in}
%\includegraphics[height=2.0cm]{figure/IDK_physionet_mortality.pdf}&
%\hspace{-0.26in}
%\includegraphics[height=2.0cm]{figure/IDK_physionet_stay.pdf}&
%\hspace{-0.26in}
%\includegraphics[height=2.0cm]{figure/IDK_physionet_cardiac.pdf}&
%\hspace{-0.26in}
%\includegraphics[height=2.0cm]{figure/IDK_physionet_recovery.pdf}&
%\hspace{-0.26in}
%\includegraphics[height=2.0cm]{figure/IDK_pancreatic.pdf}&
%\hspace{-0.26in}
%\includegraphics[height=2.0cm]{figure/IDK_sepsis.pdf}\\
%\hspace{-0.14in}(a) PhysioNet & (b) PhysioNet & (c) PhysioNet & (d) PhysioNet & (e) Pancreatic & (f) MIMIC \\
%  - Mortality & - Stay $<$ 3 & - Cardiac & - Recovery & Cancer & - Sepsis \\
%\end{tabular}
%\vspace{-0.15in}  
%\caption{\small Experiments on prediction reliability. The stacked bar charts show the ratio IDK and incorrect predictions for different rate of correct prediction.}%\label{fig:ratio}
%\vspace{-0.25in}  
%\end{figure*}


%\begin{figure*}[t]
%	\subfigure[PhysioNet-Mortality]{\includegraphics[height=2.1cm]{figure/IDK_physionet_recovery.pdf}}
%	\hfill
%	\subfigure[PhysioNet-Stay$<$ 3]{\includegraphics[height=2.1cm]{figure/IDK_physionet_recovery.pdf}} 
%	\hfill
%	\subfigure[PhysioNet-Cardiac]{\includegraphics[height=2.1cm]{figure/IDK_pancreatic.pdf}} 
%	\hfill
%	\subfigure[PhysioNet-Recovery]{\includegraphics[height=2.1cm]{figure/IDK_sepsis.pdf}}
%	\hfill
%	\subfigure[Pancreatic Cancer]{\includegraphics[height=2.1cm]{figure/IDK_sepsis.pdf}}
%	\hfill
%	\subfigure[MIMIC-Sepsis]{\includegraphics[height=2.1cm]{figure/IDK_sepsis.pdf}}
%	\caption{Experiments on prediction reliability. The stacked bar charts show the ratio IDK and incorrect predictions for different rate of correct prediction.}\label{fig:ratio}
%\end{figure*}




==> application.tex <==
\section{Application to classification from time-series data}
Our variational attention model is generic and can be applied to any generic deep neural network that leverages attention mechanism. However, in this section, we describe its application to prediction from time-series data, since our target application is risk analysis from electronic health records.

\paragraph{Review of the RETAIN model}
As a base deep network for learning from time-series data, we consider RETAIN~\cite{retain}, which is an attentional RNN model with two types of attentions--across \emph{timesteps} and across \emph{features}. RETAIN obtains state-of-the-art performance on risk prediction tasks from electronic health records, and is able to provide useful interpretations via learned attentions. 
%We first introduce the notation for \cite{retain}. Suppose there are patients $n=1,...,N$. Each patient $n$ has timestep $i=1,...,T(n)$, and the corresponding set of input features up to timestep $i$ is denoted as $\bbX_{i}^{(n)}=\left\{\bx_1^{(n)},...,\bx_i^{(n)}\right\}$, where $\bx \in \real^{r}$. The corresponding set of binary labels is only provided at the last timestep $T{(n)}$, denoted as $y^{(n)}$. The whole training dataset is then $\D = \left\{\left(\bx_1^{(n)},...,\bx_{T(n)}^{(n)}, y^{(n)}\right)\right\}_{n=1}^N$. When we are interested in timestep $i$, its intermediate timesteps are indexed as $j=1,...,i$. We will not specify patient index for variables if context is clear. 

We now briefly review the overall structure of RETAIN. We match the notation with those in the original paper for clear reference. Suppose we are interested in a timestep $i$. With the input embeddings $\bv_1,\dots,\bv_i$, we generate two different attentions: across timesteps ($\alpha$) and features ($\bbeta$).
\begin{align}
&\bg_i,...,\bg_1 = \rnn_\alpha (\bv_i,...,\bv_1;\bs\omega), 
&\bh_i,...,\bh_1 = \rnn_\bbeta (\bv_i,...,\bv_1;\bs\omega),\label{eq:rnn} \\
&e_j = \bw_\alpha^\T \bg_j + b_\alpha\ \ \text{for}\ \ j=1,...,i, 
&\bd_j = \bW_\bbeta \bh_j + \bb_\bbeta\ \ \text{for}\ \ j=1,...,i,\label{eq:retain_logit} \\
&\alpha_1,...,\alpha_i = \softmax(e_1,...,e_i), 
&\bbeta_j = \tanh(\bd_j)\ \ \text{for}\ \  j=1,...,i.\label{eq:retain}
\end{align}
%\begin{align}
%\alpha_1,\alpha_2,...,\alpha_i = \softmax(e_1,e_2,...,e_i), \quad
%\bbeta_j = \tanh(\bd_j)\ \ \text{for}\ \ j=1,...,i.\label{eq:retain}
%\end{align}
The parameters of two RNNs are collected as $\bs\omega$. From the RNN outputs $\bg$ and $\bh$, the attention logits $e$ and $\bd$ are generated, followed by squashing functions $\softmax$ and $\tanh$ respectively. %$\bd_1,\dots,\bd_i$ denote logits of each attention repectively, generated by two different RNNs with the same input $\bv_1,\dots,\bv_i$.
%$\rnn(\cdot)$ denotes a generic recurrent neural networks, such as LSTM and GRU.
%
%Another attention $\bbeta_j \in [-1,1]^r$ for timestep $j$ and across features $k=1,...,r$ is generated as
%\begin{equation}
%\begin{aligned}
%\bh_i,\bh_{i-1},...,\bh_1 &= \rnn_\bbeta (\bv_i,\bv_{i-1},...,\bv_1;\bs\omega) \\
%\bd_j &= \bW_\bbeta \bh_j + \bb_\bbeta \\
%\bbeta_j &= \tanh(\bd_j)\ \ \ \text{for}\ \ \ j=1,...,i.
%\label{eq:beta}
%\end{aligned}
%\end{equation}
Then the generated two attentions $\alpha$ and $\bbeta$ are multiplied back to the input embedding $\bv$, followed by a convex sum $\bc$ up to timestep $i$: $\bc_i = \sum_{j=1}^{i}\alpha_j\bbeta_j\odot\bv_j$. A final linear predictor is learned based on it: $\widehat{y}_i = \sigm(\bw^\T\bc_i + b)$.

%\begin{align}
%\bc_i = \sum_{j=1}^{i}\alpha_j\bbeta_j\odot\bv_j,\quad
%\widehat{y}_i = \sigm(\bw^\T\bc_i + b)
%\label{eq:final_prediction}
%\end{align}

%\begin{equation}
%\begin{aligned}
%\frac{1}{N}\sum_{n=1}^{N}
%\left\{
%y^{(n)}\log(\widehat{y}^{(n)})
%+(1-y^{(n)})\log(1-\widehat{y}^{(n)})
%\right\}\nonumber
%\end{aligned}
%\end{equation}
%Note that unlike in~\citep{retain}, the label is only provided at the end of the timestep for each patient.

The most important feature of RETAIN is that it allows us to interpret what the model has learned as follows. What we are interested in is \emph{contribution}, which shows $x_{k}$'s aggregate effect to the final prediction at time $j$. Since RETAIN has attentions on both timesteps ($\alpha_j$) and features ($\bbeta_{j}$), the computation of aggregate contribution takes both of them into consideration when computing the final contribution of an input data point at a specific timestep: $\omega(y,x_{j,k}) = \alpha_j \bw^\T (\bbeta_j\odot \bW_{emb}[:,k]) x_{j,k}$. 
%\begin{equation}
%\begin{aligned}
%\omega(y,x_{j,k}) = \alpha_j \bw^\T (\bbeta_j\odot \bW_{emb}[:,k]) x_{j,k}
%\label{eq:contribution}
%\end{aligned}
%\end{equation}
In other words, it is a certain portion of logit $\sigm^{-1}(\widehat{y}_i) = \bw^\T \bc_i + b$ for which $x_{j,k}$ is responsible.

\paragraph{Interpretation as a probabilistic model}
%For a given timestep $i$, we define the set of inputs for it as $\bX_i = [\bx_1...\bx_i]$. Suppose each patient $n$ has a sequence of record that consists of timesteps $t=1,...,T(n)$. Then,
%\begin{align}
%\D=\{\bX,\bY\},\quad
%\bX = \left\{\bX_{T(n)}^{(n)}\right\}_{n=1}^N,\quad
%\bY = \left\{y^{(n)}\right\}_{n=1}^N
%\nonumber
%\end{align}
The interpretation of RETAIN as a probabilistic model is quite straightforwrad. First, the RNN parameters $\bs\omega$ \eqref{eq:rnn} as gaussian latent variables \eqref{eq:uncertainty} are approximated with MC dropout with fixed probabilities \cite{dropout_as_bayesian, rnn_dropout, bayesian_lstm}. The input dependent latent variables $\bZ$ \eqref{eq:uncertainty} simply correspond to the collection of $e$ and $\bd$ \eqref{eq:retain_logit}, the attention logits. The log variances of $e$ and $\bd$ are generated in the same way as their mean, from the output of RNNs $\bg$ and $\bd$ but with different set of parameters. Also the reparameterization trick for diagonal gaussian is simple \cite{vae}.
%$\rnn_\alpha$ in \eqref{eq:alpha} and $\rnn_\bbeta$ in \eqref{eq:beta} is set to $\bs\omega$. It means that each $\rnn$ has dropout regularization with fixed probabilities~\cite{rnn_dropout}.
%Next we discuss about $\bZ$, our latent variables for generating attentions. First, recap the definition of $p_\theta$ in \eqref{eq:aleatoric_uncertainty}. Then, it is straightforward that the mean $\bs\mu_j$ corresponds to the concatenation $[e_j;\bd_j]$ in \eqref{eq:alpha} and \eqref{eq:beta}, respectively. The variance term $\bs\sigma_j$ is generated in the same way as $\bs\mu_j$, from the output of $\rnn_\alpha$ and $\rnn_{\bbeta}$, respectively. We then combine $\bs\mu_j + \bs\sigma_j\odot\bs\varepsilon$ as before, which simply corresponds to $\bz_j$, where we sample $\bs\varepsilon\sim\N(\mathbf{0},\mathbf{I})$ for reparameterization trick. $\theta$ corresponds to all the parameters associated with generating $\bs\mu_j$ and $\bs\sigma_j$. Then we define the collection $\bZ_i = [\bz_1\dots\bz_i]$ and the aggregate set of latent variables $\bZ = \{\bZ_{T(n)}^{(n)}\}_{n=1}^N$.  
%In the same way, we generate another set of $\mu_j^q$ and $\sigma_j^q$ in \eqref{eq:q_gaussian} from the output of $\rnn_\alpha$ and $\rnn_\bbeta$. $\phi$ is defined to be all the parameters associated with generating $\mu_j^q$ and $\sigma_j^q$. When training, we sample $z$ from $z = \mu_j^q + \sigma_j^q \varepsilon$, while $\mu_j^p$ and $\sigma_j^p$ are trained via KL term (Eq.\eqref{eq:kl_normal}). 
%When testing, we sample $z$ from $z = \mu_j + \sigma_j \varepsilon$. We are now equipped with $p_\theta(z_j|\bx,\bs\omega)$,
% and $q_\phi(z_j|\bx,y,\bs\omega)$, 
%In conclusion, our latent variable $\bZ$ is defined as
%\begin{equation}
%\begin{aligned}
%\bZ_i=[[e_1+\sigma^e_1\varepsilon;\bd_1+\bs\sigma^d_1\odot\bs\varepsilon]...[e_i+\sigma^e_1\varepsilon;\bd_i+\bs\sigma^d_1\odot\bs\varepsilon]]
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\bZ = \left\{\bZ_{T(n)}^{(n)}\right\}_{n=1}^N.
%\end{aligned}
%\end{equation}
%How to utilize label $y$ as an input to $q_\phi(z_j|\bx,y,\bs\omega)$ is an open question, since the formulation does not tell us anything about it. If we naively put $y$ to $q_\phi(z_j|\bx,y,\bs\omega)$ in the form of $[\bg_j; y]$ or $[\bh_j; y]$, and nothing to $p_\theta(z_j|\bx,\bs\omega)$, then two pipelines for training and testing become different with performances being degenerated. \cite{cvae} thus suggests $p_\theta$ to generate a pseudo label $\widetilde{y}_i$ with some additional parameters. Then the input to $p_\theta$ network would take the form $[\bg_j; \widetilde{y}]$ or $[\bh_j; \widetilde{y}]$, which is consistent with the input to $q_\phi$. It is also known to effectively deepen the network \citep{cvae}. More specifically,
%\begin{equation}
%\begin{aligned}
%\bu_i,\bu_{i-1},...,\bu_1 &= \rnn_{\widetilde{y}}(\bv_i,\bv_{i-1},...,\bv_1) \\
%\widetilde{y}_i &= \bw_{\widetilde{y}}^\T \bu_i + b_{\widetilde{y}} 
%\end{aligned}
%\end{equation}
%%The detailed architecture of our model is depicted in Figure \ref{fig:mainmodel}.
We now maximize the ELBO \eqref{eq:each_obj}, equipped with all the components $\bX$,$\bY$,$\bZ$, and $\bs\omega$ as in the previous section.
%, and epistemic/heteroscedastic uncertainties can be sampled from Eq. \eqref{eq:sample_epistemic} and Eq. \eqref{eq:sample_aleatoric}.




==> approach.tex <==
\section{Approach}
We now describe our uncertainty-aware attention model. Let $\D = \{\bX_i, \bY_i\}$ be a dataset containing a set of input datapoints $\bX = [\bx^{(1)}\dots\bx^{(N)}]$ and the corresponding set of labels, $\bY=[\by^{(1)}\dots\by^{(N)}]$. We drop index superscript $(i)$ when dealing with a single datapoint. 
%For example, if the task is image annotation~\citep{show_attend_tell}, then $\{\bX, \by}$ takes

%Our goal is to learn stochastic attentions \emph{having low variances}. The existing deterministic attention mechanisms ignore this variance, and simply finds the best mapping that minimizes a given loss function. The idea is, if it is reliable, then the variance should be limited. We do not want attentions to have high variance if 

We first present a general framework of a stochastic attention mechanism. Let $\bv(\bx) \in \real^{i\times r}$ be an intermediate feature from an arbitrary neural network. From $\bv(\bx)$, a set of random variable $\ba \in \real^{i}$ is conditionally generated from some distribution $p(\ba|\bx)$, and element-wisely multiplied back to $\bv(\bx)$ along axis 1. Then summation along axis 1 results in a set of context vectors $\bc \in \real^r$, on which we perform final prediction $\hat{\by}$.
\begin{align}
\bc(\bx) &= \sum \ba \odot \bv(\bx) 
\nonumber \\
\hat{\by} &= f(\bc(\bx))
\nonumber
\end{align}
where $f$ is a mapping from $\bc$ to the predicted label $\hat{\by}$. 

The attention could be generated either deterministically, or stochastically. The stochastic attention mechanism is proposed in~\cite{show_attend_tell}, where they generate $\ba \in \{0,1\}$ from Bernoulli distribution. This variable is learned by maximizing the evidence lower bound (ELBO) with additional regularizations for reducing variance of gradients. In~\cite{show_attend_tell}, the stochastic attention is shown to perform better than the deterministic counterpart, on image annotation task.

\subsection{Stochastic attention with input-adaptive Gaussian noise}
However, there are two drawbacks in modeling stochastic attention directly with Bernoulli distribution as done in~\cite{show_attend_tell}. First, the variance $\sigma^2$ is completely dependent on the retain probability $\mu$; that is, $\sigma^2 = \mu(1-\mu)$. This model thus cannot generate $\ba$ with low variance if $\mu$ is around $0.5$, and vice versa, due to the intrinsic nature of the distribution. 
To overcome such limitations, we disentangle the attention strength $\ba$ from the attention uncertainty, such that the uncertainty could vary even with the same attention strength. 

Secondly, such input-independent modeling of variance $\sigma^2$ makes it difficult to model the amount of uncertainty for each input, which is crucial for reliable machine learning. Even when given the same prediction tasks and the same set of features, the amount of uncertainty for each feature may largely vary among different instances. For instance, 

Therefore, we model the standard deviation $\sigma$, which is indicative of the uncertainty, as an \emph{input-adaptive} function, such that it can reflect different amount of confidence the model has for each feature, for a given instance.
%Specifically, we propose to use Gaussian additive noise instead of Bernoulli as the distribution of attention.
%Therefore, we propose to use Gaussian noise instead of Bernoulli distribution, in order to express different amount of variances for different input points, even with same mean:

\begin{align}
p(\bs\omega) &= \N(\mathbf{0}, \tau^{-1}\bI)
\label{eq:epistemic_uncertainty} \\
p_\theta(\bz|\bx,\bs\omega)
&= \prod_{j=1}^{i} \N(\mu_j^p(\bx,\bs\omega;\theta),\sigma_j^p(\bx,\bs\omega;\theta)^2)
\label{eq:aleatoric_uncertainty} \\
\ba &= \pi(\bz)\label{eq:squashing}
\end{align}

Note that Gaussian is on the input to the attentions in Eq. \eqref{eq:aleatoric_uncertainty}, followed by some squashing function $\pi(\cdot)$ in Eq. \eqref{eq:squashing} (e.g. sigmoid or hyperbolic tangent). 

In the above equation, we assumed that we use a common, shared set of $\theta$ for generating $\mu^p$ and $\sigma^p$. The motivation is that $\mu^p$ and $\sigma^p$ should be generated in relation to others, as if the variation is high ($\sigma$ is high) then this means that the given input is uncertain and $\mu$ should be lowered to reflect it. However they could be modeled with separate sets of parameters as well.


%Also note that $\mu$ and $\sigma$ are modeled with different set of parameters, although they are denote as general $\theta$.
We also assume that a subset of the neural network parameters $\bs\omega$, associated with generating $\mu^p$ and $\sigma^p$, is from zero-mean isotropic Gaussian prior with precision $\tau$ (Eq. \eqref{eq:epistemic_uncertainty}), whose role will be discussed in Section~\ref{section:two_uncertainties} in more detail. 

\subsection{Variational inference}
Let $\bZ$ be the set of latent variables $[\bz^{(1)}\dots\bz^{(N)}]$ that stand for attention weight before squashing. 

In neural network, the posterior distribution $p(\bZ,\bs\omega|\D)$ is usually intractable due to nonlinear dependency between variables. Thus, we utilize variational inference, which is an approximation method that has been shown to be successful in many applications of neural networks~\cite{vae,cvae}, along with reprameterization tricks for pathwise backpropagation~\cite{variational_dropout,concrete_dropout}. We first define our variational distribution as
\begin{equation}
\begin{aligned}
q(\bZ,\bs\omega|\D) = q_\bM(\bs\omega|\bX,\bY)q_\phi(\bZ|\bX,\bY,\bs\omega)
\end{aligned}
\end{equation}
We set $q_\bM(\bs\omega|\bX,\bY)$ to dropout approximation, with variational paramters $\bM$ for point estimates of $\bs\omega$~\cite{dropout_as_bayesian}.
Also, we model $q_\phi(\bZ|\bX,\bY,\bs\omega)$ as decomposable by each instance and each element, which follows univariate gaussian with another set of parameters $\phi$.
\begin{equation}
\begin{aligned}
q_\phi(\bZ|\bX,\bY,\bs\omega) &= \prod_{n=1}^{N} \prod_{j=1}^{i} q_\phi\left(z_j^{(n)}|\bx^{(n)},\by^{(n)},\bs\omega\right) \\
q_\phi(z_j|\bx,\by,\bs\omega) &= \N\left(\mu_j^q(\bx,\by,\bs\omega;\phi), \sigma_j^q(\bx,\by,\bs\omega;\phi)^2\right)
\label{eq:q_gaussian}
\end{aligned}
\end{equation}

We then minimize $\kl[q_\phi(\bZ,\bs\omega|\D)\|p(\bZ,\bs\omega|\D)]$. It is known to be equivalent to maximizing the evidence lower bound:
\begin{align}
&\log p(\bY|\bX) \nonumber \\
\geq &\ \E_{\bs\omega\sim q_\bM(\bs\omega|\bX,\bY), \bZ \sim q_\theta(\bZ|\bX,\bY,\bs\omega)}\left[\log p(\bY|\bX,\bZ)\right]
\label{eq:expected_log_likelihood} \\
&- \kl[q_\bM(\bs\omega|\bX,\bY)\|p(\bs\omega)]
\label{eq:kl_epistemic} \\
&- \kl[q_\phi(\bZ|\bX,\bY,\bs\omega)\|p_\theta(\bZ|\bX,\bs\omega)]
\label{eq:kl_aleatoric}
\end{align}
%where $\theta$ is parameters associated with generating $\bZ$ from the prior distribution $p(\bZ|\bX,\bs\omega)$. 
where we approximate the expectation in Eq. \eqref{eq:expected_log_likelihood} via Monte-Carlo sampling with sample size $1$. KL divergence term in Eq. \eqref{eq:kl_epistemic} nicely reduces to $\ell_2$ regularization for $\bM$ with dropout approximation~\cite{dropout_as_bayesian}. KL term in Eq.~\eqref{eq:kl_aleatoric} can be decomposed as sum of individual instance and elements, which is simply the KL divergence between two univariate Gaussians (Eq. \ref{eq:aleatoric_uncertainty}, Eq.\ref{eq:q_gaussian}):
\begin{equation}
\begin{aligned}
\kl[q_\phi\|p_\theta] = \log\frac{\sigma^q}{\sigma^p} + \frac{(\sigma^p)^2 + (\mu^p-{\mu^q})^2}{2(\sigma^q)^2} + const.\label{eq:kl_normal}
\end{aligned}
\end{equation}
%where we denote $\{\mu_\phi, \sigma_\phi\}$ from $q_\phi$ and $\{\mu_\theta, \sigma_\theta\}$ from $p_\theta$, for notational simplicity.
Consequently, our final maximization objective is:
\begin{equation}
\begin{aligned}
\loss&(\theta,\phi,\bM;\bX,\bY) =\sum_{n=1}^{N}\Big\{\log p_\theta(\by^{(n)}|\tilde{\bz}^{(n)},\bx^{(n)}) \\
&- \kl\left[q_\phi(\bz^{(n)}|\bx^{(n)},\by^{(n)})\|p_\theta(\bz^{(n)}|\bx^{(n)})\right] \Big\} - \lambda \|\bM\|^2
\label{eq:each_obj}
\end{aligned}
\end{equation}
where we first sample random weights with dropout masks
$\widetilde{\bs\omega} \sim q_\bM(\bs\omega|\bX,\bY)$ and sample $\bz$ such that $\tilde{\bz} = g(\bx,\tilde{\bs\varepsilon},\widetilde{\bs\omega}), \tilde{\bs\varepsilon} \sim \N(\mathbf{0},\bI)$, with a pathwise derivative function $g$. $\lambda$ is a tunable hyperparameter; however in practice it can be simply set to common $\ell_2$ decay shared throughout the network, including other deterministic weights.

\paragraph{Inference}
When testing with a novel input instance $\bx^*$, we can compute the probability of having the correct label $y*$ by our model, $p(\by^*|\bx^*)$, as follows: 
 
\begin{align}
p(\by^*|\bx^*) = \iint p(\by^*&|\bx^*,\bz)p(\bz|\bx^*,\bs\omega)p(\bs\omega|\bX,\bY) d\bs\omega d\bz
\nonumber \\
\approx \frac{1}{S}\sum_{s=1}^{S} p&(\by^*|\bx^*,\tilde{\bz}^{(s)}) \nonumber \\
\tilde\bz^{(s)} &{\sim} p_\theta(\bz|\bx^*,\widetilde{\bs\omega}^{(s)})
\label{eq:sample_aleatoric} \\
\widetilde{\bs\omega}^{(s)} &\sim\ q_\bM(\bs\omega|\bX,\bY)
\label{eq:sample_epistemic}
\end{align}

Alternatively, we can simply put the expectation inside:
\begin{align}
p(\by^*|\bx^*) \approx p(\by^*|\bx^*,\E[\bz|\bx^*,\E[\bs\omega]])
\end{align}
which is a usual practice for many practitioners and works well in practice.
%In mini-batch framework, we randomly sample $B$ training instances and corresponding $\tilde{\bs\varepsilon}$ every iteration, compute \eqref{eq:each_obj} for all those samples, and optimize via stochastic gradient descent. 

\subsection{Epistemic and Heteroscedastic uncertainty}\label{section:two_uncertainties}
One important aspect of our model, in terms of graphical representation is that the distribution $p(\bs\omega)$ in Eq. \eqref{eq:epistemic_uncertainty} is independent of $\bx$, while the distribution $p_\theta(\bz|\bx,\bs\omega)$ in Eq. \eqref{eq:aleatoric_uncertainty} is conditional on $\bx$. That is, $p(\bs\omega)$ tends to capture uncertainty of model parameters (epistemic uncertainty), while $p_\theta(\bz|\bx,\bs\omega)$ reacts sensitively to uncertainty in data, varying across different input points (heteroscedastic uncertainty)~\cite{what_uncertainty}. These two uncertainties are not clearly separable as neither of them can be used alone as posterior process that captures both model and data uncertainties. However, if \emph{modeled together}, it has been empirically shown that epistemic uncertainty mainly captures uncertainty from lack of data, while heteroscedastic uncertainty captures intrinsic noise in data (e.g., noise in label) varying across different input points~\cite{what_uncertainty}. 

Based on this simple observation, we apply the same idea to attention mechanisms. In \cite{what_uncertainty}, they model $p_\theta(\bz|\bx,\bs\omega)$ at the end of the prediction. However, in such way we cannot analyze where the observed uncertainties come from. By modeling heteroscedastic uncertainties on \emph{attention mechanism} which is interpretable, we can successfully investigate \emph{which components} are uncertain, as well as \emph{how much} they are uncertain. To obtain each of uncertainties, we just sample from Eq. \eqref{eq:sample_aleatoric} and Eq. \eqref{eq:sample_epistemic}. When considering only a single type of uncertainty, we sample either $\bs\omega$ or $\bz$ alone. We perform experiments to show how our model captures each of uncertainties on several dataset.


















\iffalse
\subsection{Variational Inference}
We want to make attention $\alpha$ in~\eqref{eq:alpha} and $\bbeta$ in~\eqref{eq:beta} to be random variables, so that the contribution in \eqref{eq:contribution} is also a random variable. Then we could measure how reliable a learned contribution is, in other words, how reliable our interpretation toward the generated outcome is.

%Let $\bbX_i = \{\bx_j\}_{j=1}^i$ for brevity. 
In order to make our model probabilistic, we interpret input to the attentions, $e_j$ and $\bd_j$, as latent variables, and give some appropriate prior distributions, parameterized by $\theta$:
\begin{equation}
\begin{aligned}
p_\theta(e_j|\bbX_i) &= p_\theta(e_j|\bg_i) \\
p_\theta(\bd_j|\bbX_i) &= \prod_{k=1}^{r} p_\theta(d_{j,k}|\bh_i)
\label{eq:prob_attention}
\end{aligned}
\end{equation}
Define $\bbZ_i = \{e_1,...,e_i,\bd_1,...,\bd_i\}$ and $\bbZ_i^{(n)}$ for $n$-th patient.
The goal of learning is then to learn the joint posterior $p(\bbZ_i|\bbX_i,\D)$, and apply it to a novel input $\bbX_i^*$ for some $i$. However, there are nonlinear transformations on $\bbZ_i$ to generate attentions, and further nonlinear transformation to compute $\widehat{y}_i$ makes it intractable to compute the true posterior.

We thus adopt variational inference to solve the problem. 
%Let $\bz_i = \{e_1,...,e_i,\bh_1,...,\bh_i\}$ for brevity. Then,
Our variational distribution, parameterized by $\phi$, is decomposable as
\begin{equation}
\begin{aligned}
&q_\phi(\bbZ_i|\bbX_i,y) \\
&= q_\phi(e_1,...,e_i,\bd_1,...,\bd_i|\bbX_i,y) \\
%&= \prod_{j=1}^i q(e_j|\bbX_i,y)\prod_{j=1}^i\prod_{k=1}^r q(d_{j,k}|\bbX_i,y) \\
&= \prod_{j=1}^i q_\phi(e_j|\bg_i,y)\prod_{j=1}^i\prod_{k=1}^r q_\phi(d_{j,k}|\bh_i,y)
\end{aligned}
\end{equation}
The KL divergence is then:
\begin{equation}
\begin{aligned}
&\ \kl\left[q_\phi(\bbZ_i|\bbX_i,y) \| p_\theta(\bbZ_i|\bbX_i)\right] \\
= &\ \sum_{j=1}^{i}\kl\left[q_\phi(e_j|\bg_i,y)\|p_\theta(e_j|\bg_i)\right] \\
 &\ + \sum_{j=1}^{i} \sum_{k=1}^{r} \kl\left[q_\phi(d_{j,k}|\bh_i,y)\|p_\theta(d_{j,k}|\bh_i)\right]
 \label{eq:decomposable_posterior}
\end{aligned}
\end{equation}
which is for a single patient. We then sum up all the KL divergences for patients $n=1,...,N$ to get the aggreagated KL divergence.

Define $\bbX=\left\{\bbX_{T(1)}^{(1)},...,\bbX_{T(N)}^{(N)}\right\}$, $\by=\left\{y^{(1)},...,y^{(N)}\right\}$, and $\bbZ = \left\{\bbZ_{T(1)}^{(1)},...,\bbZ_{T(N)}^{(N)}\right\}$. Our optimization objective is the evidence lower bound (ELBO):
\begin{equation}
\begin{aligned}
&\log p(\by|\bbX;\theta, \phi) \\
&\geq \sum_{n=1}^{N} \sum_{i=1}^{T(n)}\Big\{ \E_{q_\phi \left(\bbZ_i^{(n)}|\bbX_i^{(n)},y^{(n)}\right)}\big[\log p_\theta (y^{(n)}|\bbX_i^{(n)},\bbZ_i^{(n)})\big]\\ &-\kl\left[q_\phi(\bbZ_i^{(n)}|\bbX_i^{(n)},y^{(n)}) \| p_\theta(\bbZ_i^{(n)}|\bbX_i^{(n)})\right]\Big\}
\label{eq:objective}
\end{aligned}
\end{equation}
which we can optimize with mini-batch gradient descent~\citep{vae}. And for a single instance in mini-batch, the expectation in \eqref{eq:objective} is approximated with Monte-Carlo sampling, with the number of sampling set to $1$ as usual.

\subsection{Structure of the posterior}
Overall, there are two options to model $q(\bbZ_i|\bbX_i,y)$~\cite{cvae}:
\begin{itemize}
	\item $q(\bbZ_i|\bbX_i,y) = p_\theta(\bbZ_i|\bbX_i)$
	\item $q(\bbZ_i|\bbX_i,y) = q_\phi(\bbZ_i|\bbX_i,y) \neq p_\theta(\bbZ_i|\bbX_i)$
\end{itemize}
First option means we just put the recognition network to be the same as the prior network. This is less plausible in terms of variational inference, as the posterior $q$ does not refer to the label. However, it empirically shows competitive performance~\cite{cvae}, on which we verify the same competencies.

If we go for the second option, then how to model the pipeline of input $y$ to the recognition network $q(\bbZ_i|\bbX_i,y)$ is an open question. One can come up with a naive concatenation $[\bbX_i; y]$ as an input to the recognition network. However, the prior network $p(\bbZ_i|\bbX_i)$ cannot access to the label as an input, resulting in inconsistency between training and testing pipeline. It causes a significant drop in performance~\citep{cvae}. 

To make it consistent, \cite{cvae} suggests $p$ to generate a pseudo label $\widetilde{y}_i$ with some additional parameters. Then the input to $p$ network would take the form $[\bbX_i; \widetilde{y}]$, which is consistent with $[\bbX_i; y]$. The detailed architecture is depicted in Figure \ref{fig:mainmodel}. It is also known to effectively deepen the network \citep{cvae}. More specifically,
\begin{equation}
\begin{aligned}
\bu_i,\bu_{i-1},...,\bu_1 &= \rnn_{\widetilde{y}}(\bv_i,\bv_{i-1},...,\bv_1) \\
\widetilde{y}_i &= \bw_{\widetilde{y}}^\T \bu_i + b_{\widetilde{y}} \\
\end{aligned}
\end{equation}
and in \eqref{eq:alpha} and \eqref{eq:beta}, we redefine $e_j$ and $\bd_j$ as
\begin{equation}
\begin{aligned}
e_j &= \bw_\alpha^\T [\bg_j; \widetilde{y}] + b_\alpha \\
\bd_j &= \bW_\bbeta [\bh_j; \widetilde{y}] + \bb_\bbeta \\
\end{aligned}
\end{equation}
for $j=1,...,i$. For the recognition network, $\widetilde{y}$ is replaced with the true label $y$.

\subsection{Assumptions on distribution}
\hb{What kinds of \{prior, posterior\} pairs of distributions would be possible? And what would it be the corresponding $\kl[q\|p]$? If we find the relationship between types of prior-posterior distributions and uncertainty properties we want to encode, then it would be great. }

\paragraph{gaussian, gaussian}
The most simple assumption on the prior and posterior distribution would be gaussian distribuion. Univariate gaussian is also easily reparameterized as $x = \mu + \sigma\varepsilon$, with $\varepsilon \sim \N(0,1)$. 


In \eqref{eq:prob_attention}, we let
\begin{equation}
\begin{aligned}
p_\theta(e_j|\bg_i) &=  \N\left(\mu^{e}_{j}(\bg_i),\{\sigma^{e}_{j}(\bg_i)\}^2\right) \\
p_\theta(d_{j,k}|\bh_i) &= \N\left(\mu_{j,k}^d(\bd_i),\{\sigma^{d}_{j,k}(\bd_i)\}^2\right)
\label{eq:distribution}
\end{aligned}
\end{equation}
and in \eqref{eq:decomposable_posterior},
\begin{equation}
\begin{aligned}
q_\phi(e_j|\bg_i,y) &= \N\left(\mu^e_{j}(\bg_i,y),\{{\sigma^{e}_{j}}(\bg_i,y)\}^2\right) \\
q_\phi(d_{j,k}|\bh_i,y) &=\N\left(\mu^{d}_{j,k}(\bh_i,y),\{{\sigma^{d}_{j,k}}(\bh_i,y)\}^2\right)
\end{aligned}
\end{equation}
To generalize, suppose $p = \N(\mu_1,\sigma_1^2)$ and $q = \N(\mu_2,\sigma_2^2)$.
The KL divergence between them is:
\begin{equation}
\begin{aligned}
\kl[q\|p] = \log\frac{\sigma_1}{\sigma_2} + \frac{\sigma_2^2 + (\mu_2-\mu_1)^2}{2\sigma_1^2} + const.
\end{aligned}
\end{equation}
where $\mu_1$,$\mu_2$,$\sigma_1$, and $\sigma_2$ are easily optimized via backpropagation.
\fi

==> approachOne.tex <==
\section{Approach}
We now describe our uncertainty-aware attention model. Let $\D$ be a dataset containing a set of $N$ input data points $\bX = [\bx^{(1)}\dots\bx^{(N)}]$ and the corresponding labels, $\bY = [\by^{(1)}\dots\by^{(N)}]$. For notational simplicity, we suppress the data index $n=1,\dots,N$ when it is clear from the context.
%For example, if the task is image annotation~\citep{show_attend_tell}, then $\{\bX, \by}$ takes

%Our goal is to learn stochastic attentions \emph{having low variances}. The existing deterministic attention mechanisms ignore this variance, and simply finds the best mapping that minimizes a given loss function. The idea is, if it is reliable, then the variance should be limited. We do not want attentions to have high variance if 

We first present a general framework of a stochastic attention mechanism. Let $\bv(\bx) \in \real^{r\times i}$ be the concatenation of $i$ intermediate features, each column of which $\bv_j(\bx)$ is a length $r$ vector, from an arbitrary neural network. From $\bv(\bx)$, a set of random variables $\{\ba_j\}_{j=1}^i$ is conditionally generated from some distribution $p(\ba|\bx)$ where the dimension of $\ba_j$ depends on the model architecture.  Then, the context vector $\bc \in \real^r$ is computed as follows:
% and element-wisely multiplied back to $\bv(\bx)$ along axis 1. Then summation along axis 1 results in a set of context vectors $\bc \in \real^r$, on which we perform final prediction $\hat{\by}$.
\begin{align*}
	\bc(\bx) = \sum_{j=1}^i \ba_j \odot \bv_j(\bx),\quad\hat{\by} = f(\bc(\bx)) 
\end{align*}
where the operator $\odot$ is properly defined according to the dimensionality of $\ba_j$; if $\ba_j$ is a scalar, it is simply the multiplication while for $\ba_j \in \real^r$, it is the element-wise product. The function $f$ here produces the prediction $\hat{\by}$ given the context vector $\bc$. 

The attention could be generated either deterministically, or stochastically. The stochastic attention mechanism is proposed in~\cite{show_attend_tell}, where they generate $\ba_j \in \{0,1\}$ from Bernoulli distribution. This variable is learned by maximizing the evidence lower bound (ELBO) with additional regularizations for reducing variance of gradients. In~\cite{show_attend_tell}, the stochastic attention is shown to perform better than the deterministic counterpart, on image annotation task.

\subsection{Stochastic attention with input-adaptive Gaussian noise}
Despite the performance improvement in \cite{show_attend_tell}, there are two limitations in modeling stochastic attention directly with Bernoulli (or Multinoulli) distribution as \cite{show_attend_tell} does, in our purposes:

\textbf{1) The variance $\sigma^2$ of Bernoulli is completely dependent on the allocation probability $\mu$.}

Since the variance for Bernoulli distribution is decided as $\sigma^2 = \mu(1-\mu)$, the model thus cannot generate $\ba$ with low variance if $\mu$ is around $0.5$, and vice versa. 
To overcome such limitation, we disentangle the attention strength $\ba$ from the attention uncertainty so that the uncertainty could vary even with the same attention strength. 

\textbf{2) The vanilla stochastic attention models the noise independently of the input.} 

This  makes it infeasible to model the amount of uncertainty for each input, which is a crucial factor for reliable machine learning. Even for the same prediction tasks and for the same set of features, the amount of uncertainty for each feature may largely vary across different instances. %For instance, \hb{to be filled out..}

To overcome these two limitations, we model the standard deviation $\sigma$, which is indicative of the uncertainty, as an \emph{input-adaptive} function $\sigma(\mbf{x})$, enabling to reflect different amount of confidence the model has for each feature, for a given instance. As for distribution, we use \emph{Gaussian} distribution, which is probably the most simple and efficient solution for our purpose, and also easy to implement.

We first assume that a subset of the neural network parameters $\bs\omega$, associated with generating attentions, has zero-mean isotropic Gaussian prior with precision $\tau$. Then the attention scores before squashing, denoted as $\bz$, are generated from conditional distribution $p_\theta(\bz|\bx,\bs\omega)$, which is also Gaussian:
%Specifically, we propose to use Gaussian additive noise instead of Bernoulli as the distribution of attention.
%Specifically, we use Gaussian distribution instead of Bernoulli distribution, in order to express different amount of variances for different input points, even with same mean:
\begin{align}
	p(\bs\omega) = \N(\mathbf{0}, \tau^{-1}\bI),\quad
	p_\theta(\bz|\bx,\bs\omega) = \N(\bs\mu(\bx,\bs\omega;\theta),\diag(\bs\sigma^2(\bx,\bs\omega;\theta))) \label{eq:uncertainty}
\end{align}
where $\bs\mu(\cdot,\bs\omega;\theta)$ and $\bs\sigma(\cdot,\bs\omega;\theta)$ are mean and s.d., parameterized by $\theta$. Note that 
%Gaussian is on the input to the attentions in Eq. \eqref{eq:aleatoric_uncertainty}, followed by  
$\bs\mu$ and $\bs\sigma$ are generated from the same layer, but with different set of parameters, although we denote those parameters as $\theta$ in general.
%In the above equation, we assumed that we use a common, shared set of $\theta$ for generating $\mu$ and $\sigma$. The motivation is that $\mu^p$ and $\sigma^p$ should be generated in relation to others, as if the variation is high ($\sigma$ is high) then this means that the given input is uncertain and $\mu$ should be lowered to reflect it. However they could be modeled with separate sets of parameters as well.
The actual attention $\ba$ is then obtained by applying some squashing function $\pi(\cdot)$ to $\bz$ (e.g. sigmoid or hyperbolic tangent):
%\begin{align}
	$\ba = \pi(\bz)$. %\label{eq:squashing}
%\end{align}
%Also note that $\mu$ and $\sigma$ are modeled with different set of parameters, although they are denote as general $\theta$.
%(Eq. \eqref{eq:epistemic_uncertainty}), whose role will be discussed in Section~\ref{section:two_uncertainties} in more detail. 
For comparison, one can think of the vanilla stochastic attention of which variance is independent of inputs.
\begin{align}
p(\bs\omega) = \N(\mathbf{0}, \tau^{-1}\bI),\quad
p_\theta(\bz|\bx,\bs\omega) = \N(\bs\mu(\bx,\bs\omega;\theta),\diag(\bs\sigma^2)) \label{eq:vanila_stochastic_attention}
\end{align}
However, as we mentioned, this model cannot express different amount of uncertainties over features.

One important aspect of our model is that, in terms of graphical representation, the distribution $p(\bs\omega)$ is independent of $\bx$, while the distribution $p_\theta(\bz|\bx,\bs\omega)$ is conditional on $\bx$. That is, $p(\bs\omega)$ tends to capture uncertainty of model parameters (epistemic uncertainty), while $p_\theta(\bz|\bx,\bs\omega)$ reacts sensitively to uncertainty in data, varying across different input points (heteroscedastic uncertainty)~\cite{what_uncertainty}. 
%These two uncertainties are not clearly separable as neither of them can be used alone as posterior process that captures both model and data uncertainties. However, 
When \emph{modeled together}, it has been empirically shown that the quality of uncertainty improves~\cite{what_uncertainty}. Such modeling both input-agnostic and input-dependent uncertainty is especially important in risk analysis tasks in healthcare, to capture both the uncertainty from insufficient amount of clinical data (e.g. rare diseases), and the uncertainty that varies from patients to patients (e.g. sepsis).
%epistemic uncertainty mainly captures uncertainty from lack of data, while heteroscedastic uncertainty captures intrinsic noise in data (e.g., noise in label) varying across different input points~\cite{what_uncertainty}. 

==> approachTwo.tex <==
%\subsection{Uncertainty modeling}\label{section:two_uncertainties}
%\hb{input dependent uncertainty is important...}
\subsection{Variational inference}
We now model what we have discussed so far. Let $\bZ$ be the set of latent variables $\{\bz^{(n)}\}_{n=1}^{N}$ that stands for attention weight before squashing. In neural network, the posterior distribution $p(\bZ,\bs\omega|\D)$ is usually computationally intractable since $p(\D)$ is so due to nonlinear dependency between variables. Thus, we utilize variational inference, which is an approximation method that has been shown to be successful in many applications of neural networks~\cite{vae,cvae}, along with reprameterization tricks for pathwise backpropagation~\cite{variational_dropout,concrete_dropout}. 

Toward this, we first define our variational distribution as
\begin{equation}
\begin{aligned}
q(\bZ,\bs\omega|\D) = q_\bM(\bs\omega|\bX,\bY)q(\bZ|\bX,\bY,\bs\omega).
\end{aligned}
\end{equation}
We set $q_\bM(\bs\omega|\bX,\bY)$ to dropout approximation \cite{dropout_as_bayesian} with variational parameter $\bM$. \cite{dropout_as_bayesian} showed that a neural network with Gaussian prior on its weight matrices can be approximated with variational inference, in the form of dropout sampling of deterministic weight matrices and $\ell_2$ weight decay.
For the second term, we drop the dependency on $\bY$ (since it is not available in test time) and simply set $q(\bZ|\bX,\bY,\bs\omega)$ to be equivalent to $p_\theta(\bZ|\bX,\bs\omega)$, which works well in practice~\citep{cvae,show_attend_tell}.
%as decomposable by each instance and each element, which follows univariate gaussian with another set of parameters $\phi$.
%\begin{equation}
%\begin{aligned}
%q_\phi(\bZ|\bX,\bY,\bs\omega) &= \prod_{n=1}^{N} \prod_{j=1}^{i} q_\phi\left(z_j^{(n)}|\bx^{(n)},\by^{(n)},\bs\omega\right) \\
%q_\phi(z_j|\bx,\by,\bs\omega) &= \N\left(\mu_j(\bx,\by,\bs\omega;\phi), \sigma_j(\bx,\by,\bs\omega;\phi)^2\right)
%\label{eq:q_gaussian}
%\end{aligned}
%\end{equation}

Under the SGVB framework \cite{vae}, we 
%then minimize $\kl[q_\phi(\bZ,\bs\omega|\D)\|p(\bZ,\bs\omega|\D)]$. It is known to be equivalent to 
maximize the evidence lower bound (ELBO):
\begin{align}
\log p(\bY|\bX) \geq \ &\E_{\bs\omega\sim q_\bM(\bs\omega|\bX,\bY), \bZ \sim p_\theta(\bZ|\bX,\bs\omega)}\left[\log p(\bY|\bX,\bZ,\bs\omega)\right]
\label{eq:expected_log_likelihood} \\
&- \kl[q_\bM(\bs\omega|\bX,\bY)\|p(\bs\omega)] - \kl[q(\bZ|\bX,\bY,\bs\omega)\|p_\theta(\bZ|\bX,\bs\omega)]
\label{eq:kl}
\end{align}
%where $\theta$ is parameters associated with generating $\bZ$ from the prior distribution $p(\bZ|\bX,\bs\omega)$. 
where we approximate the expectation in \eqref{eq:expected_log_likelihood} via Monte-Carlo sampling. The first KL term nicely reduces to $\ell_2$ regularization for $\bM$ with dropout approximation~\cite{dropout_as_bayesian}. 
The second KL term vanishes as the two distributions are equivalent.
%KL term in Eq.~\eqref{eq:kl_aleatoric} can be decomposed as sum of individual instance and elements, which is simply the KL divergence between two univariate Gaussians (Eq. \ref{eq:aleatoric_uncertainty}, Eq.\ref{eq:q_gaussian}):
%\begin{equation}
%\begin{aligned}
%\kl[q_\phi\|p_\theta] = \log\frac{\sigma^q}{\sigma^p} + \frac{(\sigma^p)^2 + (\mu^p-{\mu^q})^2}{2(\sigma^q)^2} + const.\label{eq:kl_normal}
%\end{aligned}
%\end{equation}
%where we denote $\{\mu_\phi, \sigma_\phi\}$ from $q_\phi$ and $\{\mu_\theta, \sigma_\theta\}$ from $p_\theta$, for notational simplicity.
Consequently, our final maximization objective is:
%\begin{equation}
%\begin{aligned}
%\loss&(\theta,\phi,\bM;\bX,\bY) =\sum_{n=1}^{N}\Big\{\log p_\theta(\by^{(n)}|\tilde{\bz}^{(n)},\bx^{(n)}) \\
% &- \kl\left[q_\phi(\bz^{(n)}|\bx^{(n)},\by^{(n)})\|p_\theta(\bz^{(n)}|\bx^{(n)})\right] \Big\} - \lambda \|\bM\|^2
%\label{eq:each_obj}
%\end{aligned}
%\end{equation}
\begin{align}
\loss(\theta,\bM;\bX,\bY) =\sum \log p_\theta(\by^{(n)}|\tilde{\bz}^{(n)},\bx^{(n)}) - \lambda \|\bM\|^2 \label{eq:each_obj}
\end{align}
where we first sample random weights with dropout masks
$\widetilde{\bs\omega} \sim q_\bM(\bs\omega|\bX,\bY)$ and sample $\bz$ such that $\tilde{\bz} = g(\bx,\tilde{\bs\varepsilon},\widetilde{\bs\omega}), \tilde{\bs\varepsilon} \sim \N(\mathbf{0},\bI)$, with a pathwise derivative function $g$ for reparameterization trick. $\lambda$ is a tunable hyperparameter; however in practice it can be simply set to common $\ell_2$ decay shared throughout the network, including other deterministic weights.

When testing with a novel input instance $\bx^*$, we can compute the probability of having the correct label $y^*$ by our model, $p(\by^*|\bx^*)$ with Monte-Carlo sampling: 
\begin{align}
p(\by^*|\bx^*) = \iint p(\by^*|\bx^*,\bz)p(\bz|\bx^*,\bs\omega)p(\bs\omega|\bX,\bY) \text{d}\bs\omega \text{d}\bz \approx \frac{1}{S}\sum_{s=1}^{S} p(\by^*|\bx^*,\tilde{\bz}^{(s)}) \label{eq:test}
\end{align}
where we first sample dropout masks $\widetilde{\bs\omega}^{(s)} \sim\ q_\bM(\bs\omega|\bX,\bY)$ and then sample $\tilde\bz^{(s)} \sim p_\theta(\bz|\bx^*,\widetilde{\bs\omega}^{(s)})$.
%Alternatively, we can simply put the expectation inside $p(\by^*|\bx^*) \approx p(\by^*|\bx^*,\E[\bz|\bx^*,\E[\bs\omega]])$ which is a usual practice for many practitioners and works well in practice.

%In mini-batch framework, we randomly sample $B$ training instances and corresponding $\tilde{\bs\varepsilon}$ every iteration, compute \eqref{eq:each_obj} for all those samples, and optimize via stochastic gradient descent. 
\paragraph{Uncertainty Calibration} The quality of uncertainty from \eqref{eq:test} can be evaluated with reliability diagram shown in Figure \ref{fig:reliability_diagram}. Better calibrated uncertainties produce smaller \emph{gaps} beween model confidences and actual accuracies, shown in green bars. Thus, the perfect calibration occurs when the confidences exactly matches the actual accuracies: $p(\text{correct}|\text{confidence}=\rho)=\rho, \forall\rho\in[0,1]$ \cite{guo17}. Also, \cite{ece,guo17} proposed a summary statistic for calibration, called the Expected Calibration Error (ECE). It is the expected \emph{gap} w.r.t. the distribution of model confidence (or frequency of bins):
\begin{align}
	\text{ECE} = \E_\text{confidence}\big[|p(\text{correct}|\text{confidence})-\text{confidence}|\big]\label{eq:ece}
\end{align}

\iffalse
\subsection{Variational Inference}
We want to make attention $\alpha$ in~\eqref{eq:alpha} and $\bbeta$ in~\eqref{eq:beta} to be random variables, so that the contribution in \eqref{eq:contribution} is also a random variable. Then we could measure how reliable a learned contribution is, in other words, how reliable our interpretation toward the generated outcome is.

%Let $\bbX_i = \{\bx_j\}_{j=1}^i$ for brevity. 
In order to make our model probabilistic, we interpret input to the attentions, $e_j$ and $\bd_j$, as latent variables, and give some appropriate prior distributions, parameterized by $\theta$:
\begin{equation}
\begin{aligned}
p_\theta(e_j|\bbX_i) &= p_\theta(e_j|\bg_i) \\
p_\theta(\bd_j|\bbX_i) &= \prod_{k=1}^{r} p_\theta(d_{j,k}|\bh_i)
\label{eq:prob_attention}
\end{aligned}
\end{equation}
Define $\bbZ_i = \{e_1,...,e_i,\bd_1,...,\bd_i\}$ and $\bbZ_i^{(n)}$ for $n$-th patient.
The goal of learning is then to learn the joint posterior $p(\bbZ_i|\bbX_i,\D)$, and apply it to a novel input $\bbX_i^*$ for some $i$. However, there are nonlinear transformations on $\bbZ_i$ to generate attentions, and further nonlinear transformation to compute $\widehat{y}_i$ makes it intractable to compute the true posterior.

We thus adopt variational inference to solve the problem. 
%Let $\bz_i = \{e_1,...,e_i,\bh_1,...,\bh_i\}$ for brevity. Then,
Our variational distribution, parameterized by $\phi$, is decomposable as
\begin{equation}
\begin{aligned}
&q_\phi(\bbZ_i|\bbX_i,y) \\
&= q_\phi(e_1,...,e_i,\bd_1,...,\bd_i|\bbX_i,y) \\
%&= \prod_{j=1}^i q(e_j|\bbX_i,y)\prod_{j=1}^i\prod_{k=1}^r q(d_{j,k}|\bbX_i,y) \\
&= \prod_{j=1}^i q_\phi(e_j|\bg_i,y)\prod_{j=1}^i\prod_{k=1}^r q_\phi(d_{j,k}|\bh_i,y)
\end{aligned}
\end{equation}
The KL divergence is then:
\begin{equation}
\begin{aligned}
&\ \kl\left[q_\phi(\bbZ_i|\bbX_i,y) \| p_\theta(\bbZ_i|\bbX_i)\right] \\
= &\ \sum_{j=1}^{i}\kl\left[q_\phi(e_j|\bg_i,y)\|p_\theta(e_j|\bg_i)\right] \\
 &\ + \sum_{j=1}^{i} \sum_{k=1}^{r} \kl\left[q_\phi(d_{j,k}|\bh_i,y)\|p_\theta(d_{j,k}|\bh_i)\right]
 \label{eq:decomposable_posterior}
\end{aligned}
\end{equation}
which is for a single patient. We then sum up all the KL divergences for patients $n=1,...,N$ to get the aggreagated KL divergence.

Define $\bbX=\left\{\bbX_{T(1)}^{(1)},...,\bbX_{T(N)}^{(N)}\right\}$, $\by=\left\{y^{(1)},...,y^{(N)}\right\}$, and $\bbZ = \left\{\bbZ_{T(1)}^{(1)},...,\bbZ_{T(N)}^{(N)}\right\}$. Our optimization objective is the evidence lower bound (ELBO):
\begin{equation}
\begin{aligned}
&\log p(\by|\bbX;\theta, \phi) \\
&\geq \sum_{n=1}^{N} \sum_{i=1}^{T(n)}\Big\{ \E_{q_\phi \left(\bbZ_i^{(n)}|\bbX_i^{(n)},y^{(n)}\right)}\big[\log p_\theta (y^{(n)}|\bbX_i^{(n)},\bbZ_i^{(n)})\big]\\ &-\kl\left[q_\phi(\bbZ_i^{(n)}|\bbX_i^{(n)},y^{(n)}) \| p_\theta(\bbZ_i^{(n)}|\bbX_i^{(n)})\right]\Big\}
\label{eq:objective}
\end{aligned}
\end{equation}
which we can optimize with mini-batch gradient descent~\citep{vae}. And for a single instance in mini-batch, the expectation in \eqref{eq:objective} is approximated with Monte-Carlo sampling, with the number of sampling set to $1$ as usual.

\subsection{Structure of the posterior}
Overall, there are two options to model $q(\bbZ_i|\bbX_i,y)$~\cite{cvae}:
\begin{itemize}
	\item $q(\bbZ_i|\bbX_i,y) = p_\theta(\bbZ_i|\bbX_i)$
	\item $q(\bbZ_i|\bbX_i,y) = q_\phi(\bbZ_i|\bbX_i,y) \neq p_\theta(\bbZ_i|\bbX_i)$
\end{itemize}
First option means we just put the recognition network to be the same as the prior network. This is less plausible in terms of variational inference, as the posterior $q$ does not refer to the label. However, it empirically shows competitive performance~\cite{cvae}, on which we verify the same competencies.

If we go for the second option, then how to model the pipeline of input $y$ to the recognition network $q(\bbZ_i|\bbX_i,y)$ is an open question. One can come up with a naive concatenation $[\bbX_i; y]$ as an input to the recognition network. However, the prior network $p(\bbZ_i|\bbX_i)$ cannot access to the label as an input, resulting in inconsistency between training and testing pipeline. It causes a significant drop in performance~\citep{cvae}. 

To make it consistent, \cite{cvae} suggests $p$ to generate a pseudo label $\widetilde{y}_i$ with some additional parameters. Then the input to $p$ network would take the form $[\bbX_i; \widetilde{y}]$, which is consistent with $[\bbX_i; y]$. The detailed architecture is depicted in Figure \ref{fig:mainmodel}. It is also known to effectively deepen the network \citep{cvae}. More specifically,
\begin{equation}
\begin{aligned}
\bu_i,\bu_{i-1},...,\bu_1 &= \rnn_{\widetilde{y}}(\bv_i,\bv_{i-1},...,\bv_1) \\
\widetilde{y}_i &= \bw_{\widetilde{y}}^\T \bu_i + b_{\widetilde{y}} \\
\end{aligned}
\end{equation}
and in \eqref{eq:alpha} and \eqref{eq:beta}, we redefine $e_j$ and $\bd_j$ as
\begin{equation}
\begin{aligned}
e_j &= \bw_\alpha^\T [\bg_j; \widetilde{y}] + b_\alpha \\
\bd_j &= \bW_\bbeta [\bh_j; \widetilde{y}] + \bb_\bbeta \\
\end{aligned}
\end{equation}
for $j=1,...,i$. For the recognition network, $\widetilde{y}$ is replaced with the true label $y$.

\subsection{Assumptions on distribution}
\hb{What kinds of \{prior, posterior\} pairs of distributions would be possible? And what would it be the corresponding $\kl[q\|p]$? If we find the relationship between types of prior-posterior distributions and uncertainty properties we want to encode, then it would be great. }

\paragraph{gaussian, gaussian}
The most simple assumption on the prior and posterior distribution would be gaussian distribuion. Univariate gaussian is also easily reparameterized as $x = \mu + \sigma\varepsilon$, with $\varepsilon \sim \N(0,1)$. 


In \eqref{eq:prob_attention}, we let
\begin{equation}
\begin{aligned}
p_\theta(e_j|\bg_i) &=  \N\left(\mu^{e}_{j}(\bg_i),\{\sigma^{e}_{j}(\bg_i)\}^2\right) \\
p_\theta(d_{j,k}|\bh_i) &= \N\left(\mu_{j,k}^d(\bd_i),\{\sigma^{d}_{j,k}(\bd_i)\}^2\right)
\label{eq:distribution}
\end{aligned}
\end{equation}
and in \eqref{eq:decomposable_posterior},
\begin{equation}
\begin{aligned}
q_\phi(e_j|\bg_i,y) &= \N\left(\mu^e_{j}(\bg_i,y),\{{\sigma^{e}_{j}}(\bg_i,y)\}^2\right) \\
q_\phi(d_{j,k}|\bh_i,y) &=\N\left(\mu^{d}_{j,k}(\bh_i,y),\{{\sigma^{d}_{j,k}}(\bh_i,y)\}^2\right)
\end{aligned}
\end{equation}
To generalize, suppose $p = \N(\mu_1,\sigma_1^2)$ and $q = \N(\mu_2,\sigma_2^2)$.
The KL divergence between them is:
\begin{equation}
\begin{aligned}
\kl[q\|p] = \log\frac{\sigma_1}{\sigma_2} + \frac{\sigma_2^2 + (\mu_2-\mu_1)^2}{2\sigma_1^2} + const.
\end{aligned}
\end{equation}
where $\mu_1$,$\mu_2$,$\sigma_1$, and $\sigma_2$ are easily optimized via backpropagation.
\fi

==> benefit_input_dp.tex <==
\begin{table*}[h]
\small
\centering
\label{benefit_input_dp}
\begin{tabular}{@{}cccl@{}}
\toprule
\multicolumn{1}{l}{} & Gaussian Noise & 97\% Missing Rate &  \\ \midrule
RETAIN-DA & 0.7692 & 0.7129 &  \\
UA & \textbf{0.7868} & 0.7372 &  \\
UA+ & 0.7864 & \textbf{0.7643} &  \\ \bottomrule
\end{tabular}
\vspace{0.1in}
\caption{\small Classification performance of RETAIN and uncertainty-aware attention models on PhysioNet-Mortality dataset. The reported numbers are AUROC.}
\end{table*}


==> discuss.tex <==
\section{Conclusion}
We proposed uncertainty-aware attention mechanism, which generates attention weights following Gaussian distribution with learned mean and variance, that are decoupled and trained in input-adaptive manner. This input-adaptive noise modeling allows to capture heteroscedastic uncertainty, or the instance-specific uncertainty, which in turn yields more accurate calibration of prediction uncertainty. We trained it using variational inference and validated on eight different tasks from three electronic health records, on which it significantly outperformed the baselines and provided more accurate and richer interpretations. Further analysis of prediction reliability shows that our model is accurately calibrated and thus can defer predictions when making prediction with ``I don't know'' option. As future work, we plan to apply our model to tasks such as image annotation and machine translation.

%UA generates attention weights that follows Gaussian distribution with learned mean and variance, that are decoupled and trained in input-adaptive manner. Thus it is able to more accurately measure uncertainty, compared to stochastic attention that generates attentions from Bernoulli distribution, and set large degree of uncertainty if the model is uncertain about the contribution of specific features from a given instance. 


==> ece_table.tex <==
\begin{table*}[t]
\label{tbl:others}
\begin{center}
\begin{tabular}{| c | c c c |}
\hline
& PhysioNet-Mortality & MIMIC-Sepsis & Pancreatic Cancer\\
\hline

RETAIN    & 8.25    & 2.48  & 7.93  \\
RETAIN-SA & 27.03   & 3.01  & 15.8  \\
\hline
UA-Indep.   & 0000    & 0.00  & 0.00  \\
UA        & \bf 1.12    & 2.07  & 2.32  \\
UA+       & 5.27    & \bf 1.78  & \bf 2.28  \\
\hline
%UCA-PseudoLabel & & & \\
%UCA-TrueLabel & & & \\
\end{tabular}
\end{center}
\caption{\small Uncertainty calibration performance of various attention models measured with Expected Calibration Error (ECE).}
\end{table*}

==> ece_table_new.tex <==
\begin{table*}[t]
\begin{center}
\small
\resizebox{12cm}{!}{
\begin{tabular}{| c | c c c c | c | c |}
\hline
& \multicolumn{4}{c|}{PhysioNet} & Pancreatic & MIMIC \\
\cline{2-5} 
& Mortality & Stay $< 3$ & Cardiac & Recovery & Cancer & Sepsis \\
\hline
%RNN & & & \\
RETAIN-DA~\cite{retain}           & 7.23 $\pm$ 0.56      & 2.04 $\pm$ 0.56      & 5.70 $\pm$ 1.56      & 4.89 $\pm$ 0.97     & 5.45 $\pm$ 0.79     & 3.05 $\pm$ 0.56     \\
RETAIN-SA~\cite{show_attend_tell} & 7.70 $\pm$ 0.60      & 3.77 $\pm$ 0.07      & 8.82 $\pm$ 0.64      & 5.39 $\pm$ 0.80     & 9.69 $\pm$ 3.90     & 5.75 $\pm$ 0.29     \\
\hline
UA-Independent                    & 5.03 $\pm$ 0.94      & 2.74 $\pm$ 1.44      & 3.55 $\pm$ 0.56      & 4.87 $\pm$ 1.46     & 4.51 $\pm$ 0.72     & 2.04 $\pm$ 0.62     \\
UA                                & \bf 4.22 $\pm$ 0.82  & \bf 1.43 $\pm$ 0.53  & 3.33 $\pm$ 0.96      & 4.46 $\pm$ 0.73     & 3.61 $\pm$ 0.55     & \bf 1.78 $\pm$ 0.41 \\
UA+                               & 4.41 $\pm$ 0.52      & 1.68 $\pm$ 0.16      & \bf 2.66 $\pm$ 0.16  & \bf 3.98 $\pm$ 0.59 & \bf 3.22 $\pm$ 0.69 & 2.04 $\pm$ 0.62     \\
\hline
%UCA-PseudoLabel & & & &\\
%UCA-TrueLabel & & & &\\
\end{tabular}
}
\\
\caption{\small Mean Expected Calibration Error (ECE) of various attention models over 5 random splits.}
\label{tbl:ece}
\end{center}
\vspace{-0.15in}
\end{table*}

\begin{figure*}
\small
\begin{tabular}{c c c c c c}
\hspace{-0.14in}
\includegraphics[height=2.2cm]{figure/IDK_physionet_mortality.pdf}&
\hspace{-0.12in}
\includegraphics[height=2.2cm]{figure/IDK_physionet_stay.pdf}&
\hspace{-0.12in}
\includegraphics[height=2.2cm]{figure/IDK_physionet_cardiac.pdf}&
\hspace{-0.12in}
\includegraphics[height=2.2cm]{figure/IDK_physionet_recovery.pdf}&
\hspace{-0.12in}
\includegraphics[height=2.2cm]{figure/IDK_pancreatic.pdf}&
\hspace{-0.12in}
\includegraphics[height=2.2cm]{figure/IDK_sepsis.pdf}\\
\hspace{-0.10in}(a) PhysioNet & (b) PhysioNet & (c) PhysioNet & (d) PhysioNet & (e) Pancreatic & (f) MIMIC \\
  - Mortality & - Stay $<$ 3 & - Cardiac & - Recovery & Cancer & - Sepsis \\
\end{tabular}
\vspace{-0.16in}  
\caption{\small Experiments on prediction reliability. The line charts show the ratio of incorrect predictions as a function of the ratio of correct predictions for all datasets.}\label{fig:ratio}
\vspace{-0.25in}  
\end{figure*}

%UA-Gaussian & 0.7604$\pm$ 0.02 & 0.8554$\pm$ 0.02 & 0.9578$\pm$ 0.01 & 0.9053$\pm$ 0.01 & 0.8612$\pm$ 0.03 & \bf 0.8012$\pm$ 0.01\\



==> experiment.tex <==
\section{Experiments}
\vspace{-0.1in}
We validate the performance of our model on various risk prediction tasks from multiple EHR datasets, for both the prediction accuracy (Section 5.3) and prediction reliability (Section 5.4).

\subsection{Tasks and datasets}
%We test our model on three different EHR datasets with six different binary classification tasks. 

%each of which contains $80\%$ of the samples for training, $10\%$ for test, and the remaining $10\%$ for validation. 

\paragraph{1) PhysioNet} This dataset~\cite{physio2012} contains 4,000 medical records from ICU\footnote{We only use the TrainingSetA, for which the labels were available}. Each record contains 48 hours of records, with 155 timesteps, each of which contains 36 physiolocial signals including \emph{heart rate}, \emph{repiration rate} and \emph{temperature}. The challenge comes with four binary classification tasks, namely, 1) \textit{Mortality prediction},  2) \textit{Length-of-stay less than 3 days:} whether the patient will stay in ICU for less than three days, 3) \textit{Cardiac conditon:} whether the patient will have a cardiac condition, and 4) \textit{Recovery from surgery:} whether the patient was recovering from surgery.

\paragraph{2) Pancreatic Cancer}This dataset is a subset of an EHR database consisting of anonymized medical check-up records from 2002 to 2013, which includes around 1.5 million records. We extract $3,699$ patient records from this database, among which $1,233$ are patients diagnosed of pancreatic cancer. The task here is to predict the onsets of pancreatic cancer in 2013 using the records from 2002 to 2012 ($11$ timesteps), that consists of 34 variables regarding general information (e.g., sex, height, past medical history, family history) as well as vital information (e.g., systolic pressure, hemoglobin level, creatinine level) and risk inducing behaviors (e.g., tobacco and alcohol consumption).

\paragraph{3) MIMIC-Sepsis} This is the subset of the MIMIC III dataset~\cite{mimic3_ref} for sepsis prediction, which consists of 58,000 hospital admissions for 38,646 adults over 12 years. We use a subset that consists of 22,395 records of patients over age 15 and stayed in ICUs between 2001 and 2012, among which 2,624 patients are diagnosed of sepsis. We use the data from the first 48 hours after admission (24 timesteps). For features at each timestep, we select 14 sepsis-related variables including arterial blood pressure, heart rate, FiO2, and Glass Coma Score (GCS), following the clinicians' guidelines. We use Sepsis-related Organ Failure Assessment scores (SOFA) to determine the onset of sepsis.

For all datasets, we generates five random splits of training/validation/test with the ratio of $80\%:10\%:10\%$. For more detailed description of the datasets, please see \textbf{supplementary file}. 

%\paragraph{4) Pediatric Intensive Care Unit (P-ICU)} This dataset consists of electronic health records from a pediatric ICU at a major hospital, which contains records of 1632 patients. The patients' age ranges from 2 months to 19 years, with the average age of 5.8 years. We extract 9 physiological markers including \emph{pulse}, \emph{temperature}, and \emph{systolic blood pressure} from ICU records for every hour. We consider the mortality prediction task on this dataset, using records that cover the first 12 hours after ICU admission, where each hour is considered a timestep. The number of positive cases here is $116$. 
%\input{maintable}

\subsection{Baselines}
\vspace{-0.1in}
We now describe our uncertainty-calibrated attention models and relevant baselines.

\textbf{1) RETAIN-DA:} The recurrent attention model in~\cite{retain}, which uses deterministic soft attention.\\
\textbf{2) RETAIN-SA:} RETAIN model with the stochastic hard attention proposed by~\cite{show_attend_tell}, that models the attention weights with multinoulli distribution, which is learned by variational inference.\\
\textbf{3) UA-independent:} The input-independent version of our uncertainty-aware attention model in \eqref{eq:vanila_stochastic_attention} whose variance is modeled indepently of the input.\\
\textbf{4) UA:} Our input-dependent uncertainty-aware attention model in \eqref{eq:uncertainty}.\\ 
\textbf{5) UA+:} The same as UA, but with additional modeling of input-adaptive noise at the final prediction as done in~\cite{what_uncertainty}, to account for output uncertainty as well.\\

For network configuration and hyperparameters, see \textbf{supplementary file}. We will also release the codes for reproduction of the results.
%\paragraph{Network configuration and parameters} We trained all the models using Adam~\cite{adam} optimizer with dropout regularization. We set the maximum iteration for Adam optimizer as $100,000$, and for other hyperparameters, we searched for the optimal values by cross-validation, within predefined ranges as follows: Mini batch size: $\{32, 64, 128, 256\}$, learning rate: $\{0.01, 0.001, 0.0001\}$, \textit{L-2} regularization: $\{0.02, 0.002, 0.0002, 0.0004\}$, and dropout rate $\{0.1, 0.15, 0.2, 0.25, 0.3, 0.4, 0.5\}$. See supplementary file for more details on the network configurations.

%\input{other_table}


\subsection{Evaluation of the binary classification performance}
\input{physionet_table}
We first examine the prediction accuracy of baselines and our models in a standard setting where the model always makes a decision. Table~\ref{tbl:physionet} contains the accuracy of baselines and our models measured in area under the ROC curve (AUROC). We observe that UA variants significantly outperforms both RETAIN variants with either deterministic or stochastic attention mechanisms on all datasets. Note that RETAIN-SA, that generates attention from Bernoulli distribution, performs the worst. This may be because the model is primarily concerned with whether to attend or not to each feature, which makes sense when most features are irrelevant, such as with machine translation, but not in the case of clinical prediction where most of the variables are important. UA-independent performs significantly worse than UA or UA+, which demonstrates the importance of input-dependent modeling of the variance. Additional modeling of output uncertainty with UA+ yields performance gain in most cases.
\input{patient}

\vspace{-0.2in}
\paragraph{Interpretability and accuracy of generated attentions} To obtain more insight, we further analyze the contribution of each feature in PhysioNet mortality task in Figure~\ref{fig:attention} for a patient at the timestep with the highest attention $\alpha$, with the help of a physician. The table in Figure~\ref{fig:attention} is the value of the variables at the previous checkpoints and the current timestep. 

The difference between the current and the previous tmesteps is significant - the patient is applied mechanical ventilation; the body temperature, diastolic arterial blood pressure, and heart rate dropped, and GCS, which is a measure of consciousness, dropped from 15 to 10. The fact that the patient is applied mechanical ventilation, and that the GCS score is lowered, are both very important markers for assessing patient's condition. Our model correctly attends to those two variables, with very low uncertainty. SysABP and DiasABP are variables that has cyclic change in value, and are all within normal range; however RETAIN-DA attended to these variables, perhaps due to having a deterministic model which led it to overfit. Heart rate is out of normal range (60-90), which is problematic but is not definitive, and thus UA attended to it with high variance. RETAIN-SA results in overly incorrect and noisy attention except for FiO2 that did not change its value. Attention on Urine by all models may be the artifact that comes from missing entry in the previous timestep. In this case, UA assigned high variance, which shows that it is uncertain about this prediction. %Please see supplementary file for more examples.

The previous example shows another advantage of our model: it provides a richer interpretations of why the model has made such predictions, compared to ones provided by deterministic or stochastic model without input-dependent modeling of uncertainty. This additional information can be taken account by clinicians when making diagnosis, and thus can help with prediction reliability. %However, it is not feasible for the clinicians to examine all the information given by the model. Thus, it would be helpful if the model can perform some screening and present only the most uncertain cases to them.  In next paragraph, we show how to utilize our model for this purpose.

\input{patient_quantified}
We further compared UA against RETAIN-DA for accuracy of the attentions, using variables selected meaningful by clinicians as ground truth labels (avg. $132$ variables per record), from EHRs for a male and a female patient randomly selected from 10 age groups (40s-80s), on PhysioNet-Mortality. We observe that UA generates accurate interpretations that better comply with clinicians' intepretations (Table~\ref{tbl:quantify}).  

\input{ece_table_new}

%\input{uncertainty}
\subsection{Evaluation of prediction reliability}
Another important goal that we aimed to achieve with the modeling of uncertainty in the attention is achieving high reliability in prediction. Prediction reliability is orthogonal to prediction accuracy, and~\cite{ece} showed that state-of-the-art deep networks are not reliable as they are not well-calibrated to correlate model confidence with model strength. Thus, to demonstrate the reliability of our uncertainty-aware attention, we evaluate it for the uncertainty calibration performance against baseline attention models in Table~\ref{tbl:ece}, using Expected Calibration Errors (ECE)~\cite{ece} (Eq.~\eqref{eq:ece}). UA and UA+ are significantly better calibrated than RETAIN-DA, RETAIN-SA as well as UA-independent, which shows that independent modeling of variance is essential in obtaining well-calibrated uncertanties.

%For further qualitative analaysis we show the prediction uncertainty of the baseline RETAIN model and our model on all instances from the PhysioNet Challenge in Figure~\ref{fig:uncertainty}. We observe that our model has larger prediction uncertainty for instances whose prediction is incorrect (blue dots above the prediction strength of 0.5 and red dots below 0.5) or weak (near 0.5), while RETAIN shows similar uncertainty for across all inputs. 
%\input{ece_table}

\paragraph{Prediction with ``I don't know" option}
We further evaluate the reliability of our predictive model by allowing it to say I don't know (IDK), where the model can refrain from making a hard decision of yes or no when it is uncertain about its prediction. This ability to defer decision is crucial for predictive tasks in clinical environments, since those deferred patient records could be given a second round examination by human clinicians to ensure safety in its decision. To this end, we measure the uncertainty of each prediction by sampling the variance of the prediction using both MC-dropout and stochastic Gaussian noise over $30$ runs, and simply predict the label for the instances with standard deviation larger than some set threshold as IDK. 

Note that we use RETAIN-DA with MC-Dropout~\cite{rnn_dropout} as our baseline for this experiment, since RETAIN-DA is deterministic and cannot output uncertainty~\footnote{RETAIN-SA is not compared since it largely underperforms all others and is not a meaningful baseline.} We report the performance of RETAIN + DA, UA, and UA+ for all tasks by plotting the ratio of incorrect predictions as a function of the ratio of correct predictions, by varying the threshold on the model confidence (See Figure~\ref{fig:ratio}). We observe that both UA and UA+ output much smaller ratio of incorrect predictions at the same ratio of correct predictions compared to RETAIN + DA, by saying IDK on uncertain inputs. This suggests that our models are relatively more reliable and safer to use when making decisions for prediction tasks where incorrect predictions can lead to fatal consequences. Please see \textbf{supplementary file} for more results and discussions on this experiment. 
\vspace{-0.1in}

%setting the uncertainty threshold such that the correct prediction rate becomes $0.7$, and report the ratio of IDK and incorrect predictions for all 6 datasets / tasks in Figure~\ref{fig:ratio}. We observe that both UA and UA+ are more likely to say IDK rather than make incorrect predictions when compared against RETAIN + MC-Dropout model, which suggests that they are relatively more reliable, and safer to use for making clinical decisions where incorrect predictions can lead to fatal consequences. For instance, on sepsis prediction task where our model performed similarly to RETAIN, UA+ made incorrect prediction only on $0.17\%$ of the instances ($0.80\%$ for UA) while avoiding $29.83\%$ of potentially incorrect predictions based on uncertainty. On the other hand, RETAIN + MC Dropout predicted incorrectly on $2.51\%$ of the instances with $27.68\%$ IDK prediction.


%For instance, for pancreatic cancer prediction task, our model made $14.32\%$ incorrect predictions with $15.68\%$ IDK decision, while RETAIN + MC Dropout made incorrect prediction on $17.54\%$ of instance with $12.46\%$ IDK decision. This difference is significant considering the severe consequences an incorrect cancer prediction has on the patient.


  




%\paragraph{Learning with few training instances} Bayesian models are most useful when training data is scarce, and we to demonstrate this point, we report the model accuracy as the number of training instances in Figure~\ref{accuracy_over_training}. 


==> idk_numbers.tex <==
\begin{table*}[h]
\small
\centering
\label{idk_numbers}
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{1}{l}{} & False Positive & False Negative & True Positive \\ \midrule
RETAIN-DA & \bf 14  & 14     &  8  \\
%\hline
UA        &  7      & \bf 22 & \bf 10  \\
%\hline
UA+       &  8      & 21     &  9  \\ \bottomrule
\end{tabular}
\vspace{0.1in}
\caption{\small Number of false positives, false negatives, and true positives in IDK holder on PhysioNet-Mortality dataset.}
\end{table*}


==> intro.tex <==
\section{Introduction}
%Despite its recent success, deep learning is not yet fully ready to be actively applied to mission-critical tasks such as healthcare. 
For many real-world safety-critical tasks, achieving high reliablity may be the most important objective when learning predictive models for them, since incorrect predictions could potentially lead to severe consequences. For instance, failure to correctly predict the sepsis risk of a patient in ICU may cost his/her life. Deep learning models, while having achieved impressive performances on multitudes of real-world tasks such as visual recognition~\cite{alexnet,resnet}, machine translation~\cite{Bahdanau15} and risk prediction for healthcare~\cite{retain,futoma17}, may be still susceptible to such critical mistakes since most do not have any notion of predictive uncertainty, often leading to overconfident models~\cite{guo17,deep_ensembles} that are prone to making mistakes. Even worse, they are very difficult to analyze, due to multiple layers of non-linear transformations that involves large number of parameters. 

\input{reliability_diagram}

Attention mechanism~\cite{Bahdanau15} is an effective means of guiding the model to focus on a partial set of most relevant features for each input instance. It works by generating (often sparse) coefficients for the given features in an input-adaptive manner, to allocate more weights to the features that are found to be relevant for the given input. Attention mechanism has been shown to significantly improve the model performance for machine translation~\cite{Bahdanau15} and image annotation~\cite{show_attend_tell} tasks. Another important feature of the attention mechanism is that it allows easy interpretation of the model via the generated attention allocations, and one recent work on healthcare domain~\cite{retain} is focusing on this aspect. 

Although interpretable, attention mechanisms are still limited as means of implementing safe deep learning models for safety-critical tasks, as they are not necessarily reliable. The attention strengths are commonly generated from a model that is trained in a weakly-supervised manner, and could be incorrectly allocated; thus they may not be safe to base final prediction on. To build a reliable model that can prevent itself from making critical mistakes, we need a model that knows its own limitation - \emph{when it is safe to make predictions and when it is not}. However, existing attention model cannot handle this issue as they do not have any notion of predictive uncertainty. This problem is less of an issue in the conventional use of attention mechanisms, such as machine translation or image annotation, where we can often find clear link between the attended parts and the generated output. However, when working with variables that are often noisy and may not be one-to-one matched with the prediction, such as in case of risk predictions with electronic health records, the overconfident and inaccurate attentions can lead to incorrect predictions (See Figure 1).

%, and often generates incorrect attentions that are interpreted in an unexpected way

To tackle this limitation of conventional attention mechanisms, we propose to allow the attention model to output uncertainty on each feature (or input) and further leverage them when making final predictions. Specifically, we model the attention weights as Gaussian distribution with \emph{input-dependent noise}, such that the model generates attentions with small variance when it is confident about the contribution of the given features, and allocates noisy attentions with large variance to uncertain features, for each input. This input-adaptive noise can model \emph{heteroscedastic uncertainty}~\cite{what_uncertainty} that varies based on the instance, which in turn results in uncertainty-based attenuation of attention strength.  We formulate this novel uncertainty-aware attention (UA) model under the Bayesian framework and solve it with variational inference.

We validate UA on tasks such as sepsis prediction in ICU and disease risk prediction from electronic health records (EHR) that have large degree of uncertainties in the input, on which our model outperforms the baseline attention models by large margins. Further quantitative and qualitative analysis of the learned attentions and their uncertainties show that our model can also provide richer interpretations that align well with the clinician's interpretations. For further validation on prediction reliability, we evaluate it for the uncertainty calibration performance, and prediction under the scenario where the model can defer the decision by saying ``I don't know'', whose results show that UA yields significantly better calibrated networks that can better avoid making incorrect predictions on instances that it is uncertain, compared to baseline attention models.

Our contribution in this paper is threefold:
\vspace{-0.1in}
\begin{itemize}
%\item We tackle the relatively less explored problem of achieving reliability in both the model interpretations and predictions, with deep neural networks. 
\item We propose a novel variational attention model with instance-dependent modeling of variance, that captures input-level uncertainty and use it to attenuate attention strengths. 
\item We show that our uncertainty-aware attention yields accurate calibration of model uncertainty as well as attentions that aligns well with human interpretations.
\item We validate our model on six real-world risk prediction problems in healthcare domains, for both the original binary classification task and classification with ``I don't know" decision,  and show that our model obtains significant improvements over existings attention models. 
\end{itemize}


==> other_table.tex <==
\begin{table*}[t]
\caption{Experimental results on MIMIC-Sepsis, Pancreatic Cancer, and P-ICU datasets. The reported numbers are mean AUROC and standard errors for 95\% confidence interval over five random splits.}
\label{tbl:others}
\begin{center}
\begin{tabular}{c | c c c c c}
& MIMIC-Sepsis & Pancreatic Cancer & P-ICU \\
\hline
%RNN & & & &  \\
RETAIN & 0.7952$\pm$ 0.01 & 0.8528$\pm$ 0.01 & 0.9018$\pm$ 0.03\\
RETAIN-SA & 0.7534$\pm$ 0.01 & 0.8444$\pm$ 0.01 & 0.8997$\pm$ 0.01\\
\hline
UCA-Gaussian & 0.7893$\pm$ 0.01 & 0.8612$\pm$ 0.03 & 0.8945$\pm$ 0.01\\
UCA-squashed & 0.7912$\pm$0.01 & 0.8604$\pm$0.01 & 0.9007$\pm$ 0.03\\
UCA-Output & 0.7910$\pm$0.01 & 0.8523$\pm$0.03 & \\
%UCA-PseudoLabel & & & \\
%UCA-TrueLabel & & & \\
\end{tabular}
\end{center}
\end{table*}

==> pancreas_features.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\small
\centering
\caption{Feature information of pancreatic cancer dataset.}
\label{tbl:pancreas_features}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \textbf{Category}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \textbf{Feature}}} \\ \hline
Demographics & \begin{tabular}[c]{@{}l@{}}Age\\ Sex\end{tabular} \\ \hline
Socio-Economic Status & \begin{tabular}[c]{@{}l@{}}Income Level\\ Type of Disability \end{tabular} \\ \hline
Health Screening & \begin{tabular}[c]{@{}l@{}}Body Mass Index (BMI)\\ Waist Circumference\\ Systolic Blood Pressure\\ Diastolic Blood Pressure\\ Fasting Glucose\\ Total Cholesterol\\ Triglyceride\\ Hemoglobin\\ Urine Protein\\ Creatinine\\ HDL Cholesterol\\ LDL Cholesterol\\ Aspartate Aminotransferase\\ Alanine Transaminase\\ Gamma-Glutamyl Transferase\end{tabular} \\ \hline
Family History & \begin{tabular}[c]{@{}l@{}}Liver Disease\\ Stroke\\ Heart Disease\\ Hypertension\\ Diabetes Mellitus\\ Cancer\end{tabular} \\ \hline
Personal History & \begin{tabular}[c]{@{}l@{}}Stroke or Cerebral Infarction-related Disease\\ Heart Disease\\ Hypertension\\ Diabetes Mellitus\\ Hyperlipidemia\\ Tuberculosis\end{tabular} \\ \hline
Social and behavioral Factor & \begin{tabular}[c]{@{}l@{}}Alcohol Consumption\\ Smoking Habit\\ Physical Exercise\end{tabular} \\ \hline
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
%\begin{table}[]
%\centering
%\caption{My caption}
%\label{my-label}
%\begin{tabular}{@{}ll@{}}
%\toprule
%Category                     & Feature                                                                                                                                                                                                                                                                                                                                                      %\\ \midrule
%Demographics                 & \begin{tabular}[c]{@{}l@{}}Age\\ Sex\end{tabular}                                                                                                                                                                                                                                                                                                            %\\
%Socio-Economic Status        & \begin{tabular}[c]{@{}l@{}}Income Level\\ Type of Disability\\ Health Insurance\end{tabular}                                                                                                                                                                                                                                                                 %\\
%Health Screening             & \begin{tabular}[c]{@{}l@{}}Body Mass Index (BMI)\\ Waist Circumference\\ Systolic Blood Pressure\\ Diastolic Blood Pressure\\ Fasting Glucose\\ Total Cholesterol\\ Triglyceride\\ Hemoglobin\\ Urine Protein\\ %Creatinine\\ HDL Cholesterol\\ LDL Cholesterol\\ Aspartate Aminotransferase\\ Alanine Transaminase\\ Gamma-Glutamyl Transferase\end{tabular} \\
%Family History               & \begin{tabular}[c]{@{}l@{}}Liver Disease\\ Stroke\\ Heart Disease\\ Hypertension\\ Diabetes Mellitus\\ Cancer\end{tabular}                                                                                                                                                                                                                                   %\\
%Personal History             & \begin{tabular}[c]{@{}l@{}}Stroke or Cerebral Infarction-related Disease\\ Heart Disease\\ Hypertension\\ Diabetes Mellitus\\ Hyperlipidemia\\ Tuberculosis\end{tabular}                                                                                                                                                                                     %\\
%Social and behavioral Factor & \begin{tabular}[c]{@{}l@{}}Alcohol Consumption\\ Smoking Habit\\ Physical Exercise\end{tabular}                                                                                                                                                                                                                                                             
%\end{tabular}
%\end{table}

==> patient.tex <==
\begin{figure*}[t!]
\begin{center}
\small
\vspace{-0.1in}
\resizebox{12cm}{!}{
\begin{tabular}{l | c c c c c c c c c}
& MechVent & DiasABP & HR & Temp & SysABP & FiO2 & MAP & Urine & GCS\\
\hline
35m 5s& 0 & 81 & 61 & 36.2 & 135 & 1 & 71 & N/A & 15 \\
38m10s&0 & 75 & 64 & 36.7 & 94 & 1 & 74  & N/A & 15 \\
\bf38m \bf55s \textbf{(current)} &\bf1 & \bf67 & \bf57 & \bf35.2 & \bf105 & \bf1 & \bf80 & \bf35 & \bf10 \\
\end{tabular}
}
\begin{tabular}{c c c}
\hspace{-0.1in}
\includegraphics[width=4cm]{figure/RETAIN_attention_analysis_physionet.pdf}&
\hspace{-0.1in}
\includegraphics[width=4cm]{figure/SA_attention_analysis_physionet.pdf}&
\hspace{-0.1in}
\includegraphics[width=4cm]{figure/UCA_attention_analysis_physionet.pdf}\\
(a) RETAIN & (b) RETAIN-SA & (c) UA \\
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\small Visualization of contributions for a selected patient on PhysioNet mortality prediction task. \eat{Contribution indicates the extent to which each individual feature affects patient mortality.} \textbf{MechVent} - Mechanical ventilation, \textbf{DiasABP} - Diastolic arterial blood pressure, \textbf{HR} - Heart rate, \textbf{Temp} - Temperature, \textbf{SysABP} - Systolic arterial blood pressure, \textbf{FiO2} - Fractional inspired Oxygen, \textbf{MAP} - Mean arterial blood pressure, \textbf{Urine} - Urine output, \textbf{GCS} - Glasgow coma score. The table presents the value of physiological variables at the previous and the current timestep. Dots correspond to sampled attention weights.}\label{fig:attention}
\vspace{-0.1in}
\end{figure*}

==> patient_quantified.tex <==
\begin{wraptable}{r}{4.7cm}
\vspace{-0.15in}
%\begin{center}
\resizebox{4.5cm}{!}{

\begin{tabular}{| c | c | c |}

\hline
%RNN & & & \\
                     & \small Sensitivity  & \small Specificity \\
\hline
\small DA & \small 75$\%$       & \small 68$\%$   \\
\hline
\small UA                   & \small \bf 87$\%$   & \small \bf 82$\%$\\
\hline
\end{tabular}
}
\caption{\small Percentage of features selected from each model that match the features selected by the clinicians.}
\label{tbl:quantify}
%\end{center}
\vspace{-0.2in}
\end{wraptable}


==> physionet_table.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{| c | c c c c | c | c |}
\hline
& \multicolumn{4}{c|}{PhysioNet} & Pancreatic & MIMIC \\
\cline{2-5} 
& Mortality & Stay $< 3$ & Cardiac & Recovery & Cancer & Sepsis \\
\hline
%RNN & & & \\
RETAIN-DA~\cite{retain}                    & 0.7652$\pm$ 0.02     & 0.8515$\pm$ 0.02     & 0.9485$\pm$ 0.01     & 0.8830$\pm$ 0.01     & 0.8528$\pm$ 0.01     & 0.7965$\pm$ 0.01\\
RETAIN-SA~\cite{show_attend_tell}       & 0.7635$\pm$ 0.02     & 0.8412$\pm$ 0.02     & 0.9360$\pm$ 0.01     & 0.8582$\pm$ 0.02     & 0.8444$\pm$ 0.01     & 0.7695$\pm$ 0.02 \\
\hline
UA-Independent & 0.7764$\pm$ 0.01      & 0.8572$\pm$ 0.02     & 0.9516$\pm$ 0.01     & 0.8895$\pm$ 0.01     & 0.8533$\pm$ 0.03     & 0.8019$\pm$ 0.01\\
UA              & \bf 0.7827$\pm$ 0.02  & \bf 0.8628$\pm$ 0.02 & 0.9563$\pm$ 0.01     & 0.9049$\pm$ 0.01     & 0.8604$\pm$ 0.01     & 0.8017$\pm$ 0.01\\
UA+            & 0.7770$\pm$ 0.02      & 0.8577$\pm$ 0.01     & \bf 0.9612$\pm$ 0.01 & \bf 0.9074$\pm$ 0.01 & \bf 0.8638$\pm$0.02  & \bf 0.8114$\pm$ 0.01\\
\hline
%UCA-PseudoLabel & & & &\\
%UCA-TrueLabel & & & &\\
\end{tabular}
}
\caption{\small The multi-class classification performance on the three electronic health records datasets. The reported numbers are mean AUROC and standard errors for 95\% confidence interval over five random splits.}
\label{tbl:physionet}
\end{center}
\vspace{-0.15in}
\end{table*}


%UA-Gaussian & 0.7604$\pm$ 0.02 & 0.8554$\pm$ 0.02 & 0.9578$\pm$ 0.01 & 0.9053$\pm$ 0.01 & 0.8612$\pm$ 0.03 & \bf 0.8012$\pm$ 0.01\\



==> refs.tex <==
\begin{thebibliography}

@ARTICLE{bayesian_segnet,
	author = {{Kendall}, A. and {Badrinarayanan}, V. and {Cipolla}, R.},
	title = "{Bayesian SegNet: Model Uncertainty in Deep Convolutional Encoder-Decoder Architectures for Scene Understanding}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1511.02680},
	primaryClass = "cs.CV",
	year = 2015,
	month = nov,
}


@article{dropout,
	author  = {Nitish Srivastava and Geoffrey Hinton and Alex Krizhevsky and Ilya Sutskever and Ruslan Salakhutdinov},
	title   = {Dropout: A Simple Way to Prevent Neural Networks from Overfitting},
	journal = {Journal of Machine Learning Research},
	year    = {2014},
	volume  = {15},
	pages   = {1929-1958}
}

@ARTICLE{concrete_distribution,
	author = {{Maddison}, C.~J. and {Mnih}, A. and {Whye Teh}, Y.},
	title = "{The Concrete Distribution: A Continuous Relaxation of Discrete Random Variables}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1611.00712},
	primaryClass = "cs.LG",
	keywords = {Computer Science - Learning, Statistics - Machine Learning},
	year = 2016,
	month = nov,
}


@ARTICLE{cnn_dropout,
	author = {{Gal}, Y. and {Ghahramani}, Z.},
	title = "{Bayesian Convolutional Neural Networks with Bernoulli Approximate Variational Inference}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1506.02158},
	keywords = {Statistics - Machine Learning, Computer Science - Learning},
	year = 2015,
	month = jun,
}

@ARTICLE{input_uncertainty_augmentation,
	author = {Murat Seckin Ayhan and Philipp Berens},
	title = "{Test-time Data Augmentation for Estimation of Heteroscedastic Aleatoric Uncertainty in Deep Neural Networks}",
	journal = {MIDL},
	year = 2018,
	month = mar
}

@ARTICLE{timeseries_uncertainty_uber,
	author = {{Zhu}, L. and {Laptev}, N.},
	title = "{Deep and Confident Prediction for Time Series at Uber}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1709.01907},
	year = 2017,
	month = sep
}

@ARTICLE{bayesian_lstm,
	author = {{van der Westhuizen}, J. and {Lasenby}, J.},
	title = "{Bayesian LSTMs in medicine}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1706.01242},
	year = 2017,
	month = jun
}

@inproceedings{alexnet,
	title = "{ImageNet Classification with Deep Convolutional Neural Networks}",
	author = {Alex Krizhevsky and Sutskever, Ilya and Geoffrey E. Hinton},
	booktitle = {NIPS},
	year = {2012},
}

@inproceedings{ece,
    	author = {Mahdi Pakdaman Naeini and Gregory F. Cooper and Milos Hauskrecht},
    	title = {Obtaining Well Calibrated Probabilities Using Bayesian Binning},
	booktitle ={AAAI},
	year = {2015},
}

@inproceedings{sepsis3,
    	author = {Singer M and Deutschman CS and Seymour C and et al},
    	title = {The third international consensus definitions for sepsis and septic shock (sepsis-3)},
	booktitle ={JAMA},
	year = {2016},
}

@inproceedings{benchmark_mimic3,
    	author = {Sanjay Purushotham and
               Chuizheng Meng and
               Zhengping Che and
               Yan Liu},
    	title = {Benchmark of Deep Learning Models on Large Healthcare {MIMIC} Datasets},
	booktitle ={CoRR},
	year = {2017},
}

@inproceedings{physio2012,
    	author = {Ivanovitch Silva, Galan Moody, Daniel J Scott, Leo A Celi, and Roger G Mark},
    	title = {Predicting in-hospital mortality of icu patients: The physionet/computing in cardiology challenge 2012},
	booktitle ={In CinC},
	year = {2012},
}

@inproceedings{deep_ensembles,
  author    = {Balaji Lakshminarayanan and
               Alexander Pritzel and
               Charles Blundell},
  title     = {Simple and Scalable Predictive Uncertainty Estimation using Deep Ensembles},
  booktitle = {NIPS},
  pages     = {6405--6416},
  year      = {2017},
}

@inproceedings{guo17,
	author = {Chuan Guo and Geoff Pleiss and Yu Sun and Kilian Q. Weinberger},
	title = {On Calibration of Modern Neural Networks},
	booktitle = {ICML},
	year      = {2017},
}

@ARTICLE{rnn_dropout,
	author = {{Gal}, Y. and {Ghahramani}, Z.},
	title = "{A Theoretically Grounded Application of Dropout in Recurrent Neural Networks}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1512.05287},
}

@inproceedings{futoma17,
  author    = {Joseph Futoma and
               Sanjay Hariharan and
               Katherine A. Heller},
  title     = {Learning to Detect Sepsis with a Multitask Gaussian Process {RNN}
               Classifier},
  booktitle = {ICML},
  year      = {2017},
}

@article{adam,
  author    = {Diederik P. Kingma and
               Jimmy Ba},
  title     = {Adam: {A} Method for Stochastic Optimization},
  journal   = {CoRR},
  volume    = {abs/1412.6980},
  year      = {2014},
}

@inproceedings{concrete_dropout,
title = {Concrete Dropout},
author = {Gal, Yarin and Hron, Jiri and Kendall, Alex},
booktitle = {NIPS},
editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
year = {2017},
}

@InProceedings{dropout_as_bayesian,
  title = 	 {Dropout as a Bayesian Approximation: Representing Model Uncertainty in Deep Learning},
  author = 	 {Yarin Gal and Zoubin Ghahramani},
  booktitle = 	 {ICML},
  year = 	 {2016},
 }

@incollection{variational_memory,
title = {Variational Memory Addressing in Generative Models},
author = {Bornschein, J\"{o}rg and Mnih, Andriy and Zoran, Daniel and Jimenez Rezende, Danilo},
booktitle = {Advances in Neural Information Processing Systems 30},
year = {2017}
}

@article{peterson87,
author="Peterson, C.",
title="A mean field theory learning algorithm for neural networks",
journal="Complex Systems",
ISSN="",
publisher="",
year="1987",
}

@ARTICLE{variational_dropout,
	author = {{Kingma}, D.~P. and {Salimans}, T. and {Welling}, M.},
	title = "{Variational Dropout and the Local Reparameterization Trick}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1506.02557},
	primaryClass = "stat.ML",
	keywords = {Statistics - Machine Learning, Computer Science - Learning, Statistics - Computation},
	year = 2015,
	month = jun,
	adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150602557K},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{e2ememnet,
 author = {Sukhbaatar, Sainbayar and Szlam, Arthur and Weston, Jason and Fergus, Rob},
 title = {End-to-end Memory Networks},
 booktitle = {NIPS},
 year = {2015},
} 

@inproceedings{what_uncertainty,
	author = {{Kendall}, A. and {Gal}, Y.},
	title = "{What Uncertainties Do We Need in Bayesian Deep Learning for Computer Vision?}",
	 booktitle = {NIPS},
	year = 2017,
}

@article{Bahdanau15,
  author    = {Dzmitry Bahdanau and
               Kyunghyun Cho and
               Yoshua Bengio},
  title     = {Neural Machine Translation by Jointly Learning to Align and Translate},
  journal   = {ICLR},
  year      = {2015},
}

@inproceedings{show_attend_tell,
 author = {Xu, Kelvin and Ba, Jimmy Lei and Kiros, Ryan and Cho, Kyunghyun and Courville, Aaron and Salakhutdinov, Ruslan and Zemel, Richard S. and Bengio, Yoshua},
 title = {Show, Attend and Tell: Neural Image Caption Generation with Visual Attention},
 booktitle = {ICML},
 year = {2015},
} 

@incollection{retain,
	title = {RETAIN: An Interpretable Predictive Model for Healthcare using Reverse Time Attention Mechanism},
	author = {Choi, Edward and Bahadori, Mohammad Taha and Sun, Jimeng and Kulas, Joshua and Schuetz, Andy and Stewart, Walter},
	booktitle = {NIPS},
	year = {2016}
}

@incollection{cvae,
	title = {Learning Structured Output Representation using Deep Conditional Generative Models},
	author = {Kihyuk Sohn and Honglak Lee and Xinchen Yan},
	booktitle = {NIPS},
	year = {2015},
}

@incollection{vae,
	title = {Auto Encoding Variational Bayes},
	author = {Diederik P. Kingma and Max Welling},
	booktitle = {ICLR},
	year = {2014},
}

@inproceedings{resnet,
    author = {Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun},
    title = {{Deep Residual Learning for Image Recognition}},
    booktitle = {CVPR},
    year = {2016}
}

@inproceedings{wrn,
  title= {{Wide Residual Networks}},
  author={Zagoruyko, Sergey and Komodakis, Nikos},
  booktitle={BMVC},
  year={2016}
}

@incollection{Xu2012,
	author = {Yangyang Xu and Wotao Yin},
	title = {A block coordinate descent method for regularized multi-convex optimization with applications to nonnegative tensor factorization and completion},
	year = {2012},
	publisher = {Unpublished},
}

@inproceedings{ranzato07,
title = {Efficient Learning of Sparse Representations with an Energy-Based Model},
author = {Marc Aurelio Ranzato and Christopher Poultney and Sumit Chopra and Yann L. Cun},
booktitle = nips,
editor = {P. B. Sch\"{o}lkopf and J. C. Platt and T. Hoffman},
pages = {1137--1144},
year = {2007},
publisher = {MIT Press},
}

@inproceedings{dae,
 author = {Vincent, Pascal and Larochelle, Hugo and Bengio, Yoshua and Manzagol, Pierre-Antoine},
 title = {Extracting and Composing Robust Features with Denoising Autoencoders},
 booktitle = icml,
 year = {2008},
 location = {Helsinki, Finland},
 pages = {1096--1103},
 numpages = {8},
 acmid = {1390294},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article {hinton2006science,
	author = {Hinton, G. E. and Salakhutdinov, R. R.},
	title = {Reducing the Dimensionality of Data with Neural Networks},
	volume = {313},
	number = {5786},
	pages = {504--507},
	year = {2006},
	doi = {10.1126/science.1127647},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	journal = {Science}
}

@incollection{autoencoder,
 author = {Rumelhart, D. E. and Hinton, G. E. and Williams, R. J.},
 chapter = {Learning Internal Representations by Error Propagation},
 title = {Parallel Distributed Processing: Explorations in the Microstructure of Cognition, Vol. 1},
 editor = {Rumelhart, David E. and McClelland, James L. and PDP Research Group, CORPORATE},
 year = {1986},
 pages = {318--362},
 numpages = {45},
 acmid = {104293},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@inproceedings{amtl,
  title={Asymmetric Multi-task Learning Based on Task Relatedness and Confidence},
  author={Lee, G and Yang, E and Hwang, S},
  booktitle={ICML},
  year={2016},
  organization={ICML}
}

@InProceedings{maurer2012sparse,
  title={Sparse coding for multitask and transfer learning},
  author={Maurer, Andreas and Pontil, Massimiliano and Romera-Paredes, Bernardino},
  booktitle = {ICML},
  year =      {2012}
}
@inproceedings{saha11,
  author    = {Avishek Saha and
               Piyush Rai and
               Hal Daum{\'{e}} III and
               Suresh Venkatasubramanian},
  title     = {Online Learning of Multiple Tasks and Their Relationships},
  booktitle = {AISTATS 2011},
  pages     = {643--651},
  year      = {2011},
  crossref  = {DBLP:conf/aistats/2011},
  timestamp = {Thu, 11 Sep 2014 07:28:56 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/jmlr/SahaRDV11},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{self-tuning,
title = {Self-Tuning Spectral Clustering},
author = {Lihi Zelnik-manor and Pietro Perona},
booktitle = {Advances in Neural Information Processing Systems 17},
editor = {L.K. Saul and Y. Weiss and L. Bottou},
pages = {1601--1608},
year = {2005},
publisher = {MIT Press},
}

@article{leen,
year={2012},
issn={0885-6125},
journal={Machine Learning},
volume={89},
number={1-2},
author={Leen, Gayle and Peltonen, Jaakko and Kaski, Samuel},
title={Focused multi-task learning in a Gaussian process framework},
publisher={Springer US},
keywords={Gaussian processes; Multi-task learning; Transfer learning; Negative transfer},
pages={157-182},
language={English}
}

@article{GorskiPK07,
	author = {Gorski, Jochen and Pfeuffer, Frank and Klamroth, Kathrin},
	journal = {Math. Meth. of OR},
	number = 3,
	pages = {373-407},
	title = {Biconvex sets and optimization with biconvex functions: a survey and extensions.},
	volume = 66,
	year = 2007
}


@inproceedings{zhanguai,
  author    = {Yu Zhang and
               Dit{-}Yan Yeung},
  title     = {A Convex Formulation for Learning Task Relationships in Multi-Task
               Learning},
  booktitle = {UAI},
  pages     = {733--442},
  year      = {2010},
  crossref  = {DBLP:conf/uai/2010},
  timestamp = {Wed, 06 May 2015 15:02:55 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/uai/ZhangY10},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@InProceedings{kang11,
  author =    {Zhuoliang Kang and Kristen Grauman and Fei Sha},
  title =     {Learning with Whom to Share in Multi-task Feature Learning },
  booktitle = {ICML},
  year =      {2011},
  pages=      {521--528},
}

@InProceedings{pentina15,
author = {Pentina, Anastasia and Sharmanska, Viktoriia and Lampert, Christoph H.},
title = {Curriculum Learning of Multiple Tasks},
booktitle = {CVPR},
month = {June},
year = {2015}
}

@inproceedings{curriculum,
  title = {Curriculum Learning},
  author = {Y. Bengio and J. Louradour and R. Collobert and J. Weston},
  booktitle = {ICML},
  year = {2009}
}

@article{evgeniou2007multi,
  title={Multi-task feature learning},
  author={Evgeniou, A and Pontil, Massimiliano},
  journal={Advances in neural information processing systems},
  volume={19},
  pages={41},
  year={2007}
}

@inproceedings{go-mtl,
  author = {Abhishek Kumar and Daume III, Hal},
  booktitle = {ICML},
  title = {Learning Task Grouping and Overlap in Multi-task Learning.},
  year = {2012},
}
@article{zhang2012convex,
  title={A convex formulation for learning task relationships in multi-task learning},
  author={Zhang, Yu and Yeung, Dit-Yan},
  journal={arXiv preprint arXiv:1203.3536},
  year={2012},
}

@article{armijo1966minimization,
  title={Minimization of functions having Lipschitz continuous first partial derivatives},
  author={Armijo, Larry and others},
  journal={Pacific Journal of mathematics},
  volume={16},
  number={1},
  pages={1--3},
  year={1966}
}
\end{thebibliography}

@INPROCEEDINGS{peronatree, 
author={Gregory Griffin and Pietro Perona}, 
booktitle = cvpr, 
title={Learning and using taxonomies for fast visual categorization}, 
year={2008}, 
pages={1--8}, 
keywords={computational complexity;greedy algorithms;pattern classification;trees (mathematics);classification trees;computational complexity;fast visual categorization;greedy algorithm;sublinear classification costs;Classification algorithms;Classification tree analysis;Computational complexity;Costs;Fasteners;Greedy algorithms;Image databases;Indexes;Taxonomy;Testing}, 
doi={10.1109/CVPR.2008.4587410}, 
ISSN={1063-6919},}

@article{gao11,
author = {Tianshi Gao and Daphne Koller},
title = {Discriminative learning of relaxed hierarchy for large-scale visual recognition},
journal = iccv,
year = {2011},
pages = {2072--2079},
doi = {http://doi.ieeecomputersociety.org/10.1109/ICCV.2011.6126481},
address = {Los Alamitos, CA, USA},
}

@inproceedings{Donahue_ICML2014,
author={Jeff Donahue and Yangqing Jia and Oriol Vinyals and Judy Hoffman and Ning Zhang and Eric Tzeng and Trevor Darrell},
title={{DeCAF}: A Deep Convolutional Activation Feature for Generic Visual Recognition},
Booktitle = icml, 
year={2014},
}


@inproceedings{wsabie,
title = {Wsabie: Scaling Up To Large Vocabulary Image Annotation},
author  = {Jason Weston and Samy Bengio and Nicolas Usunier},
year  = 2011,
booktitle = ijcai
}


@article{fobos,
author={John Duchi and Yoram Singer}, 
Title={Efficient Online and Batch Learning Using Forward Backward Splitting},
journal={Journal of Machine Learning Research},
volume={10}, 
year = {2009},
}



@article{spams,
 author = {Mairal, Julien and Bach, Francis and Ponce, Jean and Sapiro, Guillermo},
 title = {Online Learning for Matrix Factorization and Sparse Coding},
 journal = {J. Mach. Learn. Res.},
 issue_date = {3/1/2010},
 volume = {11},
 month = mar,
 year = {2010},
 issn = {1532-4435},
 pages = {19--60},
 numpages = {42},
 acmid = {1756008},
 publisher = {JMLR.org},
} 

@inproceedings{proximalhier,
  title={Proximal methods for sparse hierarchical dictionary learning},
  author={Jenatton, Rodolphe and Mairal, Julien and Bach, Francis R and Obozinski, Guillaume R},
  booktitle={Proceedings of the 27th International Conference on Machine Learning (ICML-10)},
  pages={487--494},
  year={2010}
}

@inproceedings{devise,
title = {DeViSE: A Deep Visual-Semantic Embedding Model},
author  = {Andrea Frome and Greg Corrado and Jon Shlens and Samy Bengio and Jeffrey Dean and Marc'Aurelio Ranzato and Tomas Mikolov},
year  = 2013,
booktitle = nips
}

@inproceedings{supervised-dl,
  author    = {Julien Mairal and
               Francis Bach and
               Jean Ponce and
               Guillermo Sapiro and
               Andrew Zisserman},
  title     = {Supervised Dictionary Learning},
  booktitle = nips,
  year      = {2008},
  pages     = {1033--1040},
  ee        = {http://books.nips.cc/papers/files/nips21/NIPS2008_0775.pdf},
  crossref  = {DBLP:conf/nips/2008},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{sparsecodingmtl, 
    Publisher = {JMLR Workshop and Conference Proceedings}, 
    Title = {Sparse coding for multitask and transfer learning}, 
    Url = {http://jmlr.csail.mit.edu/proceedings/papers/v28/maurer13.pdf}, 
    Booktitle = icml, 
    Author = {Andreas Maurer and Massi Pontil and Bernardino Romera-paredes}, 
    Number = {2}, 
    Month = may, 
    Volume = {28}, 
    Editor = {Sanjoy Dasgupta and David Mcallester}, 
    Year = {2013}, 
    Pages = {343-351}, 
    Abstract = {We investigate the use of sparse coding and dictionary learning in the context of multitask and transfer learning. The central assumption of our learning method is that the tasks parameters are well approximated by sparse linear combinations of the atoms of a dictionary on a high or infinite dimensional space. This assumption, together with the large quantity of available data in the multitask and transfer learning settings, allows a principled choice of the dictionary. We provide bounds on the generalization error of this approach, for both settings. Numerical experiments on one synthetic and two real datasets show the advantage of our method over single task learning, a previous method based on orthogonal and dense representation of the tasks and a related method learning task grouping.} 
   }

@inproceedings{regcascade, 
    Author = {Alon Zweig and Daphna Weinshall}, 
    Booktitle = icml, 
    Title = {Hierarchical Regularization Cascade for Joint Learning}, 
    Number = {3}, 
    Volume = {28}, 
    Year = {2013}, 
    Pages = {37-45}, 
    Abstract = {As the sheer volume of available benchmark datasets increases, the problem of joint learning of classifiers and knowledge-transfer between classifiers, becomes more and more relevant. We present a hierarchical approach which exploits information sharing among different classification tasks, in multi-task and multi-class settings. It engages a top-down iterative method, which begins by posing an optimization problem with an incentive for large scale sharing among all classes. This incentive to share is gradually decreased,until there is no sharing and all tasks are considered separately. The method therefore exploits different levels of sharing within a given group of related tasks, without having to make hard decisions about the grouping of tasks. In order to deal with large scale problems, with many tasks and many classes, we extend our batch approach to an online setting and provide regret analysis of the algorithm. We tested our approach extensively on synthetic and real datasets, showing significant improvement over baseline and state-of-the-art methods.} 
   }

@article{hiersparsecoding,
 author = {Jenatton, Rodolphe and Mairal, Julien and Obozinski, Guillaume and Bach, Francis},
 title = {Proximal Methods for Hierarchical Sparse Coding},
 journal = {J. Mach. Learn. Res.},
 issue_date = {2/1/2011},
 volume = {12},
 month = jul,
 year = {2011},
 issn = {1532-4435},
 pages = {2297--2334},
 numpages = {38},
 acmid = {2021074},
 publisher = {JMLR.org},
} 

@InProceedings{neil,
author = {Xinlei Chen and Abhinav Shrivastava and Abhinav Gupta},
title = {NEIL: Extracting Visual Knowledge from Web Data},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {December},
year = {2013}
}

@INPROCEEDINGS{nell,
    author = {Andrew Carlson and Justin Betteridge and Bryan Kisiel and Burr Settles and Estevam R. Hruschka and Tom M. Mitchell},
    title = {Toward an architecture for never-ending language learning},
    booktitle = {In AAAI},
    year = {2010}
}

@INPROCEEDINGS{sharingfeatures, 
author={Sung Ju Hwang and Fei Sha and Kristen Grauman}, 
BOOKTITLE = cvpr,
title={Sharing features between objects and their attributes}, 
year={2011}, 
pages={1761--1768}, 
doi={10.1109/CVPR.2011.5995543}, 
ISSN={1063-6919},}

@misc{caffe,
   Author = {Yangqing Jia},
   Title = { {Caffe}: An Open Source Convolutional Architecture for Fast Feature Embedding},
   Year  = {2013}
}

@inproceedings{deviinteractive,
  author = {Devi Parikh and Kristen Grauman},
  booktitle = cvpr,
  pages = {1681--1688},
  year = {2011}
}

@InProceedings{networkactive,
  author       = "Bilgic, Mustafa and Mihalkova, Lilyana and Getoor, Lise",
  title        = "Active Learning for Networked Data",
  booktitle    = "Proceedings of the 27th International Conference on Machine Learning (ICML-10)",
  year         = "2010",
}

@inproceedings{regularity,
  added-at = {2013-11-11T00:00:00.000+0100},
  author = {Mikolov, Tomas and tau Yih, Wen and Zweig, Geoffrey},
  biburl = {http://www.bibsonomy.org/bibtex/2643988028a079be17b33924255330de5/dblp},
  booktitle = {HLT-NAACL},
  crossref = {conf/naacl/2013},
  ee = {http://aclweb.org/anthology//N/N13/N13-1090.pdf},
  interhash = {14a567771d9ce43df2e38d88cbfc251f},
  intrahash = {643988028a079be17b33924255330de5},
  keywords = {dblp},
  pages = {746-751},
  publisher = {The Association for Computational Linguistics},
  timestamp = {2013-11-11T00:00:00.000+0100},
  title = {Linguistic Regularities in Continuous Space Word Representations.},
  url = {http://dblp.uni-trier.de/db/conf/naacl/naacl2013.html#MikolovYZ13},
  year = 2013
}


@inproceedings{interactivemanifold,
  added-at = {2010-09-01T00:00:00.000+0200},
  author = {Eaton, Eric and Holness, Gary and McFarlane, Daniel},
  biburl = {http://www.bibsonomy.org/bibtex/294e8c24313cd81d386c9508b79a92a2e/dblp},
  booktitle = {AAAI},
  crossref = {conf/aaai/2010},
  editor = {Fox, Maria and Poole, David},
  ee = {http://www.aaai.org/ocs/index.php/AAAI/AAAI10/paper/view/1874},
  interhash = {7b6c5dbb6abd4bc7210dbc0838d04119},
  intrahash = {94e8c24313cd81d386c9508b79a92a2e},
  keywords = {dblp},
  publisher = {AAAI Press},
  timestamp = {2010-09-01T00:00:00.000+0200},
  title = {Interactive Learning Using Manifold Geometry.},
  url = {http://dblp.uni-trier.de/db/conf/aaai/aaai2010.html#EatonHM10},
  year = 2010
}

@article{adriana11,
	Author = {Adriana Kovashka and Sudheendra Vijayanarasimhan and Kristen Grauman},
	Doi = {http://doi.ieeecomputersociety.org/10.1109/ICCV.2011.6126395},
	Isbn = {978-1-4577-1101-5},
	Journal = {Computer Vision, IEEE International Conference on},
	Pages = {1403-1410},
	Publisher = {IEEE Computer Society},
	Title = {Actively selecting annotations among objects and attributes},
	Volume = {0},
	Year = {2011},
}

@inproceedings{adriana12,
	Author = {Adriana Kovashka and Devi Parikh and Kristen Grauman},
	booktitle = {CVPR},
	Title = {WhittleSearch: Image Search with Relative Attribute Feedback},
	Year = {2012},
}

@Article{liblinear,
  author = 	 {Rong-En Fan and Kai-Wei Chang and Cho-Jui Hsieh and Xiang-Rui Wang and Chih-Jen Lin},
  title = 	 {{LIBLINEAR}: A Library for Large Linear Classification},
  journal = 	 {Journal of Machine Learning Research},
  year = 	 {2008},
  volume =	 {9},
  pages =	 {1871--1874}
}

@inproceedings{NNgreedycoord,
author = {{I S Dhillon, P Ravikumar}, and A Tewari},
booktitle = {NIPS2011},
pages = {2160--2168},
title = {{Nearest Neighbor based Greedy Coordinate Descent}},
year = {2011}
}

@inproceedings{activelarge,
author = {Jain, P and Kapoor, A},
booktitle = {2009 IEEE Conference on Computer Vision and Pattern Recognition},
doi = {10.1109/CVPR.2009.5206651},
isbn = {978-1-4244-3992-8},
issn = {10636919},
month = jun,
pages = {762--769},
publisher = {IEEE},
title = {{Active learning for large multi-class problems}},
year = {2009}
}

@inproceedings{ella, 
    Publisher = {JMLR Workshop and Conference Proceedings}, 
    Title = {{ELLA}: An Efficient Lifelong Learning Algorithm}, 
    Abstract = {The problem of learning multiple consecutive tasks, known as lifelong learning, is of great importance to the creation of intelligent, general-purpose, and flexible machines. In this paper, we develop a method for online multi-task learning in the lifelong learning setting. The proposed Efficient Lifelong Learning Algorithm (ELLA) maintains a sparsely shared basis for all task models, transfers knowledge from the basis to learn each new task, and refines the basis over time to maximize performance across all tasks. We show that ELLA has strong connections to both online dictionary learning for sparse coding and state-of-the-art batch multi-task learning methods, and provide robust theoretical performance guarantees. We show empirically that ELLA yields nearly identical performance to batch multi-task learning while learning tasks sequentially in three orders of magnitude (over 1,000x) less time.}, 
    Author = {Eric Eaton and Paul L. Ruvolo}, 
    Number = {1}, 
    Pages = {507-515}, 
    Volume = {28}, 
    Editor = {Sanjoy Dasgupta and David Mcallester}, 
    Year = {2013}, 
    Booktitle = icml 
   }

@INPROCEEDINGS{lifelongactive,
 author = {Paul Ruvolo and Eric Eaton},
 title = {Active Task Selection for Lifelong Machine Learning}, 
 booktitle = {AAAI},
 year = {2013},
 month = {July},
 }

@article{llc,
author = {Wang, Jinjun and Yang, Jianchao and Yu, Kai and Lv, Fengjun and Huang, Thomas and Gong, Yihong},
isbn = {978-1-4244-6984-0},
journal = {2010 IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
month = jun,
pages = {3360--3367},
publisher = {Ieee},
title = {{Locality-constrained Linear Coding for image classification}},
year = {2010}
}


@inproceedings{self-paced,
author = {Kumar, M Pawan and Packer, Ben and Koller, Daphne},
booktitle = {NIPS},
pages = {1--9},
title = {{Self-Paced Learning for Latent Variable Models}},
year = {2010}
}


@INPROCEEDINGS{gse,
     author = {Ouimet, Marie and Bengio, Yoshua},
     editor = {Cowell, Robert G. and Ghahramani, Zoubin},
      title = {Greedy Spectral Embedding},
  	booktitle = {Proceedings of the Tenth International Workshop on Artificial Intelligence and Statistics},
       year = {2005},
      pages = {253--260},
 	 publisher = {Society for Artificial Intelligence and Statistics},
}


@Article{mensink,
  author       = {Thomas Mensink and Jakov Verbeek and Florent Perronnin and Gabriela Csurka},
  title        = {Distance-Based Image Classification: Generalizing to New Classes at Near Zero Cost},
  journal      = {IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  volume     = {35},
  number    = {11},
  year         = {2013},
}

@inproceedings{ale,
author = {Zeynep Akata and Florent Perronnin and Zaid Harchaoui and Cordelia Schmid},
BOOKTITLE = cvpr,
pages = {819--826},
title = {{Label-Embedding for Attribute-Based Classification}},
year = {2013}
}


@inproceedings{multiple13,
author = {Kuzborskij, Ilja and Orabona, Francesco and Caputo, Barbara and Epfl, De Lausanne},
booktitle = cvpr,
year={2013},
title = {{From N to N + 1 : Multiclass Transfer Incremental Learning}}
}

@inproceedings{tommasi10,
author = {Tommasi, T. and Orabona, F. and Caputo, B.},
issn = {1063-6919},
booktitle = {CVPR},
title = {{Safety in numbers: Learning categories from few examples with multi model knowledge transfer}},
year = {2010}
}

@INCOLLECTION{thurn,
  AUTHOR         = {S. Thrun},
    YEAR           = {1995},
	  TITLE          = {A Lifelong Learning Perspective for Mobile Robot Control},
	    BOOKTITLE      = {Intelligent Robots and Systems},
		  EDITOR         = {V. Graefe},
		    PUBLISHER      = {Elsevier}
			}
@inproceedings{cai04svm,
 author = {L. Cai and T. Hofmann},
  title = {Hierarchical Document Categorization with Support Vector Machines},
   booktitle = cikm,
    year = {2004},
	 masid = {1237406}
	  }

@inproceedings{yehdynamic,
  author    = {T. Yeh and T. Darrell},
				   title     = {Dynamic visual category learning},
				     booktitle = cvpr,
					   year      = {2008},
}

@inproceedings{easythingsfirst,
  	author    = {Y. J. Lee and  K. Grauman},
	title     = {Learning the easy things first: Self-paced visual category discovery},
	booktitle = {CVPR},
									  year      = {2011},
									    pages     = {1721-1728},
}

@MISC{ngnips01,
    author = {A. Y. Ng and M. I. Jordan},
	    title = {On Discriminative vs. Generative classifiers: A comparison of logistic regression and naive Bayes},
		    year = {2001},
	booktitle = nips,
}

@inproceedings{boosting,
    author = {Y. Freund and R. E. Schapire},
	    booktitle = icml,
		  crossref = {conf/icml/1996},
		    editor = {Saitta, Lorenza},
					  pages = {148-156},
					    publisher = {Morgan Kaufmann},
						    title = {Experiments with a New Boosting Algorithm.},
							    year = 1996
}


@ARTICLE{logisticboosting,
    author = {Jerome Friedman and Trevor Hastie and Robert Tibshirani},
	    title = {Additive Logistic Regression: a Statistical View of Boosting},
		    journal = {Annals of Statistics},
			    year = {1998},
				    volume = {28},
					    pages = {2000}
						}
@ARTICLE{neuralnetworkimage,
    author = {G. Giancinto and F. Roli},
	    title = {Design of Effective Neural Network Ensembles for Image Classification Purposes},
		    journal = {Image Vison and Computing Journal},
			    year = {2001},
				    volume = {19},
					    pages = {699--707}
}

@INPROCEEDINGS{tomer,
	author = {T. Levinboim and F. Sha},
		title = {Learning the Kernel Matrix with Low-Rank Multiplicative Shaping},
			booktitle = aaai,
				year = {2012},
					keywords = {Multiple Kernel Learning; Low-Rank Matrix},
}

@INPROCEEDINGS{cortes09,
    author = {C. Cortes and M. Mohri and A. Rostamizadeh},
	    title = {Learning Non-linear Combinations of Kernels},
		    booktitle = nips,
			    year = {2009}
}

@INPROCEEDINGS{svm,
    author = {Corinna Cortes and Vladimir Vapnik},
	    title = {Support-Vector Networks},
		    booktitle = {Machine Learning},
			    year = {1995},
				    pages = {273--297}
					}

@INPROCEEDINGS{bayessvm,
    author = {N. Cesa-bianchi and L. Zaniboni},
	title = {Hierarchical classification: Combining bayes with svm},
	booktitle = {In Proceedings of the 23rd International Conference on Machine Learning},
	year = {2006},
	pages = {177--184}
}

@INPROCEEDINGS{pam,
    author = {Wei Li and Andrew Mccallum},
	title = {Pachinko allocation: DAG-structured mixture models of topic correlations},
	booktitle = {In Proceedings of the 23rd International Conference on Machine Learning},
	year = {2006},
	pages = {577--584}
}

@book{logical1,
 author = {R. W. Turner},
  title = {Logic for Artificial Intelligence},
   year = {1984},
    isbn = {0470201231},
	 publisher = {Prentice Hall PTR},
	  address = {Upper Saddle River, NJ, USA},
	  } 

@book{logical2,
 author = {M. R. Genesereth and N. J. Nilsson},
  title = {Logical foundations of artificial intelligence},
   year = {1987},
    isbn = {0-934613-31-1},
	 publisher = {Morgan Kaufmann Publishers Inc.},
	  address = {San Francisco, CA, USA},
	  } 

@article{relativeattributes,
author = {D. Parikh and K. Grauman},
title = {Relative attributes},
journal = iccv,
volume = {0},
isbn = {978-1-4577-1101-5},
year = {2011},
pages = {503-510},
doi = {http://doi.ieeecomputersociety.org/10.1109/ICCV.2011.6126281},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@book{aicogsci,
 author = {M. H. Bickhard  and L. Terveen},
  title = {Foundational Issues in Artificial Intelligence and Cognitive Science: Impasse and Solution},
   year = {1995},
    isbn = {0444820485},
	 publisher = {Elsevier Science Inc.},
	  address = {New York, NY, USA},
	  } 

@techreport{bird200,
	Author = {P. Welinder and S. Branson and T. Mita and C. Wah and F. Schroff and S. Belongie and P. Perona},
		Institution = {California Institute of Technology},
			Number = {CNS-TR-2010-001},
				Title = {{Caltech-UCSD Birds 200}},
					Year = {2010}
}

@inproceedings{mooneyecml13,
	author = {A. Acharya, A. Rawal, R. J. Mooney, and E. R. Hruschka},
	title = {Using Both Latent and Supervised Shared Topics for Multitask Learning},
	booktitle = ecml,
	year = 2013
}

@inproceedings{vapnik96,
  	author    = {Vladimir Vapnik and Steven E. Golowich and Alex J. Smola},
	title     = {Support Vector Method for Function Approximation, Regression Estimation and Signal Processing},
	booktitle = {NIPS},
	year      = {1996},
	pages     = {281-287},												   
	ee        = {http://nips.djvuzone.org/djvu/nips09/0281.djvu},
	crossref  = {DBLP:conf/nips/1996N},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{mikolov2013linguistic,
  title={Linguistic regularities in continuous space word representations},
  author={T. Mikolov  and W. Yih and G. Zweig},
  booktitle=naacl,
  pages={746--751},
  year={2013}
}

@INPROCEEDINGS{crosscut,
    author = {P. Shafto and C. Kemp and V. Mansinghka and M. Gordon and J. B. Tenenbaum},
    title = {Learning Cross-Cutting Systems of Categories},
    booktitle = {Proceedings of the 28th Annual Conference of the Cognitive Science Society},
    year = {2006}
}

@article{nystrom,
 author = {P. Drineas  and M. W. Mahoney},
 title = {On the Nystr\"{o}m Method for Approximating a Gram Matrix for Improved Kernel-Based Learning},
 journal = jmlr,
 issue_date = {12/1/2005},
 volume = {6},
 month = dec,
 year = {2005},
 issn = {1532-4435},
 pages = {2153--2175},
 numpages = {23},
 url = {http://dl.acm.org/citation.cfm?id=1046920.1194916},
 acmid = {1194916},
 publisher = {JMLR.org},
} 

@ARTICLE{hinton06,
    author = {G. E. Hinton and S. Osindero},
    title = {A fast learning algorithm for deep belief nets},
    journal = {Neural Computation},
    year = {2006},
    volume = {18},
    pages = {2006}
}

@inproceedings{logictagging,
author={C. Sacca and M. Diligenti and M. Gori and M. Maggini},
title = {Integrating Logic Knowledge into Graph Regularization: an application to image tagging},
year ={2011},
booktitle={Ninth Workshop on Mining and Learning with Graphs}
}

@inproceedings{farhadiattributes,
  author    = {Ali Farhadi and
               Ian Endres and
               Derek Hoiem and
               David Forsyth},
  title     = {Describing objects by their attributes},
  booktitle = cvpr,
  year      = {2009},
  pages     = {1778-1785},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/CVPRW.2009.5206772},
  crossref  = {DBLP:conf/cvpr/2009},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{structuredoutput,
 author = {I. Tsochantaridis and T. Joachims and T. Hofmann  and Y. Altun},
 title = {Large Margin Methods for Structured and Interdependent Output Variables},
 journal = jmlr,
 issue_date = {12/1/2005},
 volume = {6},
 month = dec,
 year = {2005},
 issn = {1532-4435},
 pages = {1453--1484},
 numpages = {32},
 url = {http://dl.acm.org/citation.cfm?id=1046920.1088722},
 acmid = {1088722},
 publisher = {JMLR.org},
} 

@inproceedings{localizedmkl,
 author = {G\"{o}nen, Mehmet and Alpaydin, Ethem},
 title = {Localized multiple kernel learning},
 booktitle = {Proceedings of the 25th international conference on Machine learning},
 series = {ICML '08},
 year = {2008},
 isbn = {978-1-60558-205-4},
 location = {Helsinki, Finland},
 pages = {352--359},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1390156.1390201},
 doi = {10.1145/1390156.1390201},
 acmid = {1390201},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@incollection{networkmetric,
 title ={Learning a Distance Metric from a Network},
 author={Blake Shaw and Bert Huang and Tony Jebara},
 booktitle = {Advances in Neural Information Processing Systems 24},
 editor = {J. Shawe-Taylor and R.S. Zemel and P. Bartlett and F.C.N. Pereira and K.Q. Weinberger},
 pages = {1899--1907},
 year = {2011}
}

@inproceedings{kaiyu2010,
  author    = {Jianchao Yang and
               Kai Yu and
               Thomas S. Huang},
  title     = {Efficient Highly Over-Complete Sparse Coding Using a Mixture
               Model},
  booktitle = {ECCV (5)},
  year      = {2010},
  pages     = {113-126},
  ee        = {http://dx.doi.org/10.1007/978-3-642-15555-0_9},
  crossref  = {DBLP:conf/eccv/2010-5},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{kaiyu2011,
  author    = {Yuanqing Lin and
               Fengjun Lv and
               Shenghuo Zhu and
               Ming Yang and
               Timoth{\'e}e Cour and
               Kai Yu and
               Liangliang Cao and
               Thomas S. Huang},
  title     = {Large-scale image classification: Fast feature extraction
               and SVM training},
  booktitle = {CVPR},
  year      = {2011},
  pages     = {1689-1696},
  ee        = {http://dx.doi.org/10.1109/CVPR.2011.5995477},
  crossref  = {DBLP:conf/cvpr/2011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{elasso,
  title = {Exclusive Lasso for Multi-task Feature Selection},
  author = {Yang Zhou and Rong Jin and Steven C. H. Hoi},
  year = {2010},
  doi = {http://www.jmlr.org/proceedings/papers/v9/zhou10a.html},
  researchr = {http://researchr.org/publication/ZhouJH10},
  cites = {0},
  citedby = {0},
  journal = {Journal of Machine Learning Research},
  volume = {9},
  pages = {988-995},
}

@ARTICLE{elastic,
    author = {H. Zou and T. Hastie},
    title = {Regularization and variable selection via the Elastic Net},
    journal = {Journal of the Royal Statistical Society, Series B},
    year = {2005},
    volume = {67},
    pages = {301--320}
}

@INPROCEEDINGS{ridge,
    author = {C. Saunders and A. Gammerman and V. Vovk},
    title = {Ridge Regression Learning Algorithm in Dual Variables},
    booktitle = {In Proceedings of the 15th International Conference on Machine Learning},
    year = {1998},
    pages = {515--521},
    publisher = {Morgan Kaufmann}
}

@ARTICLE{lasso,
    author = {R. Tibshirani},
    title = {Regression Shrinkage and Selection Via the Lasso},
    journal = {Journal of the Royal Statistical Society, Series B},
    year = {1994},
    volume = {58},
    pages = {267--288}
}

@article{mln,
 author = {Richardson, Matthew and Domingos, Pedro},
 title = {Markov logic networks},
 journal = {Mach. Learn.},
 issue_date = {February  2006},
 volume = {62},
 number = {1-2},
 month = feb,
 year = {2006},
 issn = {0885-6125},
 pages = {107--136},
 numpages = {30},
 url = {http://dx.doi.org/10.1007/s10994-006-5833-1},
 doi = {10.1007/s10994-006-5833-1},
 acmid = {1113910},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 keywords = {First-order logic, Graphical models, Inductive logic programming, Knowledge-based model construction, Link prediction, Log-linear models, Markov chain Monte Carlo, Markov networks, Markov random fields, Pseudo-likelihood, Satisfiability, Statistical relational learning},
} 

@inproceedings{structuralanalogy,
  title = {Transfer Learning by Structural Analogy},
  author = {Hua-Yan Wang and Qiang Yang},
  year = {2011},
  doi = {http://www.aaai.org/ocs/index.php/AAAI/AAAI11/paper/view/3593},
  researchr = {http://researchr.org/publication/WangY11},
  cites = {0},
  citedby = {0},
  booktitle = {Proceedings of the Twenty-Fifth AAAI Conference on Artificial Intelligence, AAAI 2011, San Francisco, California, USA, August 7-11, 2011},
  editor = {Wolfram Burgard and Dan Roth},
  publisher = {AAAI Press},
}

@ARTICLE{analogy,
    author = {Sabri Bayoudh and Laurent Miclet and Arnaud Delhay},
    title = {A.: Learning by analogy: A classification rule for binary and nominal data},
    journal = ijcai,
    year = {},
    volume = {2007},
    pages = {678--683}
}

@inproceedings{imagenetattr,
author = {O. Russakovsky and L. Fei-Fei},
title = {Attribute Learning in Large-scale Datasets},
booktitle = {European Conference of Computer Vision (ECCV), International Workshop on Parts and Attributes},
year = {2010},
month = {September},
address = {Crete, Greece}
}


@Article{multitaskmkl,
AUTHOR = {Widmer, Christian and Toussaint, Nora and Altun, Yasemin and Ratsch, Gunnar},
TITLE = {Inferring latent task structure for Multitask Learning by Multiple Kernel Learning},
JOURNAL = {BMC Bioinformatics},
VOLUME = {11},
YEAR = {2010},
NUMBER = {Suppl 8},
PAGES = {S5},
URL = {http://www.biomedcentral.com/1471-2105/11/S8/S5},
DOI = {10.1186/1471-2105-11-S8-S5},
PubMedID = {21034430},
ISSN = {1471-2105},
}

@article{obscure,author = {Francesco Orabona and Luo Jie and Barbara Caputo},title = {Online-batch strongly convex Multi Kernel Learning},journal ={Computer Vision and Pattern Recognition, IEEE Computer Society Conference on},volume = {0},isbn = {978-1-4244-6984-0},year = {2010},pages = {787-794},doi = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2010.5540137},publisher = {IEEE Computer Society},address = {Los Alamitos, CA, USA},}

@article{cap,
      author       = "Zhao, Peng and Rocha, Guilherme and Yu, Bin",
      title        = "The composite absolute penalties family for grouped and
                      hierarchical variable selection",
      journal      = "Vol.",
      number       = "arXiv:0909.0411. IMS-AOS-AOS584",
      month        = "Sep",
      year         = "2009",
      note         = "Comments: Published in at
                      http://dx.doi.org/10.1214/07-AOS584 the Annals of Statistics
                      (http://www.imstat.org/aos/) by the Institute of
                      Mathematical Statistics (http://www.imstat.org)",
}

@INPROCEEDINGS{h-mkl,
    author = {F. Bach},
    title = {Exploring large feature spaces with hierarchical multiple kernel learning},
    booktitle = nips,
    year = 2008,
}

@ARTICLE{simplemkl,
    author = {Alain Rakotomamonjy and Université De Rouen and Francis Bach and Stéphane Canu and Yves Grandvalet},
    title = {SimpleMKL},
    journal = {Journal of Machine Learning Research 9},
    year = {2008}
}

@INPROCEEDINGS{randomforests,
    author = {Leo Breiman Statistics and Leo Breiman},
    title = {Random Forests},
    booktitle = {Machine Learning},
    year = {2001},
    pages = {5--32}
}

@inproceedings{10000category,
 author = {Deng, Jia and Berg, Alexander C. and Li, Kai and Fei-Fei, Li},
 title = {What does classifying more than 10,000 image categories tell us?},
 booktitle = {Proceedings of the 11th European conference on Computer vision: Part V},
 series = {ECCV'10},
 year = {2010},
 isbn = {3-642-15554-5, 978-3-642-15554-3},
 location = {Heraklion, Crete, Greece},
 pages = {71--84},
 numpages = {14},
 url = {http://dl.acm.org/citation.cfm?id=1888150.1888157},
 acmid = {1888157},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 


@inproceedings{gehlermkl,
  author    = {P. V. Gehler and
               S. Nowozin},
  title     = {On Feature Combination for Multiclass Object Classification},
  booktitle = iccv,
  year      = {2009},
  pages     = {221-228},
  ee        = {http://dx.doi.org/10.1109/ICCV.2009.5459169},
  crossref  = {DBLP:conf/iccv/2009},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@inproceedings{bachmkl,
 author = {F. Bach. and G. Lanckriet, M. Jordan},
 title = {Multiple kernel learning, conic duality, and the SMO algorithm},
 booktitle = {Proceedings of the twenty-first international conference on Machine learning},
 series = {ICML '04},
 year = {2004},
 acmid = {1015424},
 publisher = {ACM},
 address = {New York, NY, USA},
} 



@TECHREPORT{cca,
    author = {David R. Hardoon and Sandor Szedmak and Or Szedmak and John Shawe-taylor},
    title = {Canonical correlation analysis; An overview with application to learning methods},
    institution = {},
    year = {2007}
}

@inproceedings{disagree,
    author = {Christoudias, C. M. and Urtasun, R. and Darrell, T.},
    booktitle = {Proc. 24th Conference on Uncertainty in Artificial Intelligence (UAI 2008)},
    citeulike-article-id = {4007606},
    keywords = {fusion, multiview, supervised},
    posted-at = {2009-02-04 14:29:21},
    priority = {2},
    title = {{Multi-View Learning in the Presence of View Disagreement}},
    year = {2008}
}

@article{dhillon2003, title={A Divisive Information-Theoretic Feature Clustering Algorithm for Text Classification}, volume={3}, url={http://www.crossref.org/jmlr_DOI.html}, number={7-8}, journal={Journal of Machine Learning Research}, publisher={MIT Press}, author={I. S. Dhillon, and S. Mallela  and R. Kumar}, editor={Guyon, Isabelle and Elisseeff, AndreEditors}, year={2003}, pages={1265--1287}}

@inproceedings{treeguided,
  author    = {S. Kim and E. P. Xing},
  title     = {Tree-Guided Group Lasso for Multi-Task Regression with Structured Sparsity},
  booktitle = icml,
  year      = {2010},
  pages     = {543-550},
}

@inproceedings{ase,
  author    = {Sung Ju Hwang and Kristen Grauman and Fei Sha},
  title     = {Analogy-preserving Semantic Embedding for Visual Object Categorization},
  booktitle = icml,
  year      = {2013},
  pages     = {639-647},
}

@incollection{jiadenglabeltree,
 title ={Fast and Balanced: Efficient Label Tree Learning for Large Scale Object Recognition},
 author={Jia Deng and Sanjeev Satheesh and Alexander C. Berg and Fei Fei F. Li},
 booktitle = {Advances in Neural Information Processing Systems 24},
 editor = {J. Shawe-Taylor and R.S. Zemel and P. Bartlett and F.C.N. Pereira and K.Q. Weinberger},
 pages = {567--575},
 year = {2011}
}

@incollection{borrowing,
 title ={Transfer Learning by Borrowing Examples for Multiclass Object Detection},
 author={Joseph J. Lim and Ruslan R. Salakhutdinov and Antonio Torralba},
 booktitle = {Advances in Neural Information Processing Systems 24},
 editor = {J. Shawe-Taylor and R.S. Zemel and P. Bartlett and F.C.N. Pereira and K.Q. Weinberger},
 pages = {118--126},
 year = {2011}
}

@incollection{chimeric,
 title ={Inductive reasoning about chimeric creatures},
 author={Charles Kemp},
 booktitle = {Advances in Neural Information Processing Systems 24},
 editor = {J. Shawe-Taylor and R.S. Zemel and P. Bartlett and F.C.N. Pereira and K.Q. Weinberger},
 pages = {316--324},
 year = {2011}
}

@incollection{nipscategoryaware,
 title ={Large-Scale Category Structure Aware Image Categorization},
 author={Bin Zhao and Fei Fei F. Li and Eric P. Xing},
 booktitle = {Advances in Neural Information Processing Systems 24},
 editor = {J. Shawe-Taylor and R.S. Zemel and P. Bartlett and F.C.N. Pereira and K.Q. Weinberger},
 pages = {1251--1259},
 year = {2011}
}

@inproceedings{mkltransfer,
    author = {Jie, Luo and Tommasi, Tatiana and Caputo, Barbara},
    booktitle = {ICCV 2011},
    title = {Multiclass Transfer Learning from Unconstrained Priors},
    year = {2011}
}


@electronic{multicluster,
    author = {Niu, Donglin and Dy, Jennifer G. and Jordan, Michael I.},
    keywords = {cluster, hsic},
    posted-at = {2010-10-19 09:24:38},
    priority = {0},
    title = {{Multiple Non-Redundant Spectral Clustering Views}},
    url = {http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.170.1490}
}

@inproceedings{mklgenerality,
 author = {M. Varma, and B. R. Babu,},
 title = {More generality in efficient multiple kernel learning},
 booktitle = {Proceedings of the 26th Annual International Conference on Machine Learning},
 series = {ICML '09},
 year = {2009},
 isbn = {978-1-60558-516-1},
 location = {Montreal, Quebec, Canada},
 pages = {1065--1072},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1553374.1553510},
 doi = {http://doi.acm.org/10.1145/1553374.1553510},
 acmid = {1553510},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{multiclassmkl,
 author = {Zien, Alexander and Ong, Cheng Soon},
 title = {Multiclass multiple kernel learning},
 booktitle = {Proceedings of the 24th international conference on Machine learning},
 series = {ICML '07},
 year = {2007},
 isbn = {978-1-59593-793-3},
 location = {Corvalis, Oregon},
 pages = {1191--1198},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1273496.1273646},
 doi = {http://doi.acm.org/10.1145/1273496.1273646},
 acmid = {1273646},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{generalmkl,
    abstract = {{While classical kernel-based learning algorithms are based on a single kernel, in practice it is often desirable to use multiple kernels. Lankriet et al. (2004) considered conic combinations of kernel matrices for classification, leading to a convex quadratically constraint quadratic program. We show that it can be rewritten as a semi-infinite linear program that can be efficiently solved by recycling the standard SVM implementations. Moreover, we generalize the formulation and our method to a larger class of problems, including regression and one-class classification. Experimental results show that the proposed algorithm helps for automatic model selection, improving the interpretability of the learning result and works for hundred thousands of examples or hundreds of kernels to be combined.}},
    address = {Cambridge, MA},
    author = {Sonnenburg, S\"oren and R\"atsch, Gunnar and Sch\"afer, Christin},
    booktitle = {Advances in Neural Information Processing Systems 18},
    citeulike-article-id = {2305988},
    editor = {Weiss, Y. and Sch\"{o}lkopf, B. and Platt, J.},
    keywords = {svm},
    pages = {1273--1280},
    pdf = {http://books.nips.cc/papers/files/nips18/NIPS2005\_0674.pdf},
    posted-at = {2008-01-30 05:38:07},
    priority = {2},
    publisher = {MIT Press},
    title = {{A General and Efficient Multiple Kernel Learning Algorithm}},
    year = {2006}
}

@InProceedings{hybrid,
  author =    {Anjum Gupta and Sanjoy Dasgupta},
  title =     {Hybrid Hierarchical Clustering: Forming a Tree From Multiple Views},
  booktitle = {Workshop on Learning With Multiple Views, at the 22th International Conference on Machine Learning (ICML-05)},
  series =    {ICML '11},
  year =      {2005},
}

@InProceedings{lampertmultiview,
  author =    {Novi Quadrianto and Christoph Lampert},
  title =     {Learning Multi-View Neighborhood Preserving Projections },
  booktitle = {Proceedings of the 28th International Conference on Machine Learning (ICML-11)},
  series =    {ICML '11},
  year =      {2011},
  editor =    {Lise Getoor and Tobias Scheffer},
  location =  {Bellevue, Washington, USA},
  isbn =      {978-1-4503-0619-5},
  month =     {June},
  publisher = {ACM},
  address =   {New York, NY, USA},
  pages=      {425--432},
}

@INPROCEEDINGS{sundataset, 
author={Jianxiong Xiao and Hays, J. and Ehinger, K.A. and Oliva, A. and Torralba, A.}, 
booktitle={Computer Vision and Pattern Recognition (CVPR), 2010 IEEE Conference on}, title={SUN database: Large-scale scene recognition from abbey to zoo}, 
year={2010}, 
month={june}, 
volume={}, 
number={}, 
pages={3485 -3492}, 
keywords={SUN database;abbey;computer vision;finer-grained scene representation;human scene classification performance;large-scale scene recognition;object categorization;scene categorization;scene category;scene understanding database;scene understanding research;state-of-the-art algorithms;zoo;computer vision;human factors;image classification;object recognition;visual databases;}, 
doi={10.1109/CVPR.2010.5539970}, 
ISSN={1063-6919},}

@incollection{graphsaliency,
 title = {Graph-Based Visual Saliency},
 author = {Jonathan Harel and Christof Koch and Pietro Perona},
 booktitle = {Advances in Neural Information Processing Systems 19},
 editor = {B. Sch\"{o}lkopf and J. Platt and T. Hoffman},
 publisher = {MIT Press},
 address = {Cambridge, MA},
 pages = {545--552},
 year = {2007}
}

@InProceedings{dagicml2011,
  author =    {Wei Bi and James Kwok},
  title =     {Multi-Label Classification on Tree- and DAG-Structured Hierarchies },
  booktitle = {Proceedings of the 28th International Conference on Machine Learning (ICML-11)},
  series =    {ICML '11},
  year =      {2011},
  editor =    {Lise Getoor and Tobias Scheffer},
  location =  {Bellevue, Washington, USA},
  isbn =      {978-1-4503-0619-5},
  month =     {June},
  publisher = {ACM},
  address =   {New York, NY, USA},
  pages=      {17--24},
}

@inproceedings{gong,
  author    = {Yunchao Gong and Svetlana Lazebnik},
  title     = {Iterative quantization: A procrustean approach to learning binary codes},
  booktitle = {CVPR},
  year      = {2011},
  pages     = {817-824},
  ee        = {http://dx.doi.org/10.1109/CVPR.2011.5995432},
  crossref  = {DBLP:conf/cvpr/2011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{gordo,
  author    = {Albert Gordo and Florent Perronnin},
  title     = {Asymmetric distances for binary embeddings},
  booktitle = {CVPR},
  year      = {2011},
  pages     = {729-736},
  ee        = {http://dx.doi.org/10.1109/CVPR.2011.5995505},
  crossref  = {DBLP:conf/cvpr/2011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{stickbreaking,
 title = {Learning concept graphs from text with stick-breaking priors},
 author = {America Chambers and Padhraic Smyth and Mark Steyvers},
 booktitle = {Advances in Neural Information Processing Systems 23},
 editor = {J. Lafferty and C. K. I. Williams and J. Shawe-Taylor and R.S. Zemel and A. Culotta},
 pages = {334--342},
 year = {2010}
}

@inProceedings{kulis09,
 title = {Learning to Hash with Binary Reconstructive Embeddings},
 author = {Brian Kulis and Trevor Darrell},
 booktitle = {Advances in Neural Information Processing Systems 22},
 editor = {Y. Bengio and D. Schuurmans and J. Lafferty and C. K. I. Williams and A. Culotta},
 pages = {1042--1050},
 year = {2009}
}

@inProceedings{spec,
author = {Ruei-Sung Lin and David A. Ross and Jay Yagnik},
title = {SPEC hashing: Similarity preserving algorithm for entropy-based coding},
journal ={Computer Vision and Pattern Recognition, IEEE Computer Society Conference on},volume = {0},isbn = {978-1-4244-6984-0},
year = {2010},pages = {848-854},doi = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2010.5540129},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

@InProceedings{largescaleembedding,
  author =    {Yann Dauphin and Xavier Glorot and Yoshua Bengio},
  title =     {Large-Scale Learning of Embeddings with Reconstruction Sampling},
  booktitle = {Proceedings of the 28th International Conference on Machine Learning (ICML-11)},
  series =    {ICML '11},
  year =      {2011},
  editor =    {Lise Getoor and Tobias Scheffer},
  location =  {Bellevue, Washington, USA},
  isbn =      {978-1-4503-0619-5},
  month =     {June},
  publisher = {ACM},
  address =   {New York, NY, USA},
  pages=      {945--952},
}

@InProceedings{minlosshash,
  author =    {Mohammad Norouzi and David Fleet},
  title =     {Minimal Loss Hashing for Compact Binary Codes},
  booktitle = {Proceedings of the 28th International Conference on Machine Learning (ICML-11)},
  series =    {ICML '11},
  year =      {2011},
  editor =    {Lise Getoor and Tobias Scheffer},
  location =  {Bellevue, Washington, USA},
  isbn =      {978-1-4503-0619-5},
  month =     {June},
  publisher = {ACM},
  address =   {New York, NY, USA},
  pages=      {353--360},
}

@InProceeding{treepreserving,
  author =    {A. Shieh and T. Hashimoto and E. Airoldi},
  title =     {Tree Preserving Embedding},
  booktitle = icml,
  year =      {2011},
  editor =    {Lise Getoor and Tobias Scheffer},
  location =  {Bellevue, Washington, USA},
  isbn =      {978-1-4503-0619-5},
  month =     {June},
  publisher = {ACM},
  address =   {New York, NY, USA},
  pages=      {753--760},
}

@inproceedings{embeddingdocument,
  author = {Kilian Q. Weinberger and Olivier Chapelle},
  title = {Large Margin Taxonomy Embedding for Document Categorization},
  booktitle = nips,
  year = {2009},
  pages = {1737--1744}
}

@inproceedings{embeddingtree,
    author = {Samy Bengio and Jason Weston and David Grangier},
    booktitle = nips,
    citeulike-article-id = {8737118},
    keywords = {decision\_tree, multiclass},
    posted-at = {2011-02-01 11:46:01},
    priority = {2},
    title = {{Label Embedding Trees for Large Multi-Class Task}},
    year = {2010}
}

@INPROCEEDINGS{kang04,
    author = {Dae-ki Kang and Adrian Silvescu and Jun Zhang and Vasant Honavar},
    title = {Generation of Attribute Value Taxonomies from Data for Data-Driven Construction of Accurate and Compact Classifiers},
    booktitle = {In: Proceedings of the 4th IEEE International Conference on Data Mining (ICDM 2004)},
    year = {2004},
    pages = {1--4}
}

@INPROCEEDINGS{vocabularyforest, 
author={Yeh, T. and Lee, J. and Darrell, T.}, 
booktitle={Computer Vision, 2007. ICCV 2007. IEEE 11th International Conference on}, title={Adaptive Vocabulary Forests br Dynamic Indexing and Category Learning}, 
year={2007}, 
month={oct.}, 
volume={}, 
number={}, 
pages={1 -8}, 
keywords={adaptive vocabulary forests;category learning;compute set-of-trees forest vocabulary representations;dynamic indexing;dynamic recognition;feature space;forward filesystem;histogram pyramid database;histogram pyramid representations;histogram pyramids;image indexing;image recognition;inverted file system;leaf nodes;pyramid match kernel;visual words;vocabulary tree indexing;image recognition;image representation;indexing;vocabulary;}, 
doi={10.1109/ICCV.2007.4409053}, 
ISSN={1550-5499},}

@INPROCEEDINGS{learningdecision,
    author = {Jun Zhang and Vasant Honavar},
    title = {Learning Decision Tree Classifiers from Attribute Value Taxonomies and Partially Specified Data},
    booktitle = {In: Proceedings of the International Conference on Machine Learning},
    year = {2003}
}

@article{incremental,
 author = {Gennari, J. H. and Langley, P. and Fisher, D.},
 title = {Models of incremental concept formation},
 journal = {Artif. Intell.},
 volume = {40},
 issue = {1-3},
 month = {September},
 year = {1989},
 issn = {0004-3702},
 pages = {11--61},
 numpages = {51},
 url = {http://dl.acm.org/citation.cfm?id=74807.74809},
 doi = {10.1016/0004-3702(89)90046-5},
 acmid = {74809},
 publisher = {Elsevier Science Publishers Ltd.},
 address = {Essex, UK},
} 

@ARTICLE{tongdecision,
AUTHOR = "Weida Tong and Huixiao Hong and Hong Fang and Qian Xie and Roger Perkins",
TITLE = "Decision Forest: Combining the Predictions of Multiple Independent Decision Tree Models.",
JOURNAL = "Journal of Chemical Information and Computer Sciences",
PAGES = {525-531},
YEAR = {2003}  
}		

@ARTICLE{automaticconstruction,
    author = {Sreerama K. Murthy},
    title = {Automatic Construction of Decision Trees from Data: A Multi-Disciplinary Survey},
    journal = {Data Mining and Knowledge Discovery},
    year = {1997},
    volume = {2},
    pages = {345--389}
}

@inproceedings{lem,
    author = {Mikhail Belkin and Partha Niyogi},
    title = {Laplacian Eigenmaps and Spectral Techniques for Embedding and Clustering},
    booktitle = {Advances in Neural Information Processing Systems 14},
    year = {2001},
    pages = {585--591},
    publisher = {MIT Press}
}

@incollection{graphsaliency,
 title = {Graph-Based Visual Saliency},
 author = {Jonathan Harel and Christof Koch and Pietro Perona},
 booktitle = {Advances in Neural Information Processing Systems 19},
 editor = {B. Sch\"{o}lkopf and J. Platt and T. Hoffman},
 publisher = {MIT Press},
 address = {Cambridge, MA},
 pages = {545--552},
 year = {2007}
}

@inproceedings{ dale09,
author = {K. Dale and M. K. Johnson and K. Sunkavalli and W. Matusik and H. Pfister},
title = {Image restoration using online photo collections},
booktitle = {International Conference on Computer Vision}, 
year = {2009}
}

@article{ vandeWeijer07,
author = {J. van de Weijer and T. Gevers and A. Gijsenij},
title = {Edge-Based Color Constancy},
journal = {IEEE Transactions on Image Processing}, 
month = {September},
year = {2007},
volume = {16},
number = {9} 
}

@inproceedings{ Finlayson04,
author = {G. Finlayson and E. Trezzi},
title = {Shades of gray and colour constancy},
booktitle = {IST Conference on Color Imaging}, 
pages = {37–41},
year = {2004}
}

@inproceedings{ 08,
   
author = {P. V. Gehler and C. Rother and A. Blake and T. Minka and T. Sharp},
   
title = {Bayesian Color Constancy Revisited},
   
year = {2008},
   
pages = {1-8},
   
month = {June},
   
booktitle = {IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
}

@inproceedings{ Rosenberg03,
author = {C. Rosenberg and T. Minka and A. Ladsariya},
title = {Bayesian color constancy with non-Gaussian models},
booktitle = {Conference on Neural Information Processing Systems}, 
month = {December},
year = {2003}
}

@INPROCEEDINGS{kangcvpr10, 
author={S. B. Kang and A. Kapoor and D. Lischinski}, 
booktitle={Computer Vision and Pattern Recognition (CVPR), 2010 IEEE Conference on}, 
title={Personalization of Image Enhancement}, 
year={2010}, 
month={june}, 
}

@INPROCEEDINGS{juancvpr11, 
author={J. C. Caicedo and A. Kapoor and S. B. Kang}, 
booktitle={Computer Vision and Pattern Recognition (CVPR), 2011 IEEE Conference on}, 
title={Collaborative Personalization of Image Enhancement}, 
year={2011}, 
month={june}, 
}

@INPROCEEDINGS{globalcvpr11, 
author={V. Bychkovsky and S. Paris and E. Chan and F. Durand}, 
booktitle={Computer Vision and Pattern Recognition (CVPR), 2011 IEEE Conference on}, 
title={Learning Photographic Global Tonal Adjustment with a Database of Input/Output Image Pairs}, 
year={2011}, 
month={june}, 
}

@INPROCEEDINGS{luo08, 
author={Y. Luo and X. Tang}, 
booktitle={European Conference on Computer Vision (ECCV), 2008}, 
title={Photo and Video Quality Evaluation: Focusing on the Subject}, 
year={2008}, 
}

@INPROCEEDINGS{outsample,
TITLE = {Out-of-Sample Extensions for LLE, Isomap, MDS, Eigenmaps, and Spectral Clustering},
AUTHOR = {Y. Bengio and J.-F. Paiement and P. Vincent},
BOOKTITLE = nips,
YEAR = {2003},
}



@article{deep,
 author = {Bengio, Yoshua},
 title = {Learning Deep Architectures for AI},
 journal = {Found. Trends Mach. Learn.},
 volume = {2},
 number = {1},
 year = {2009},
 issn = {1935-8237},
 pages = {1--127},
 doi = {http://dx.doi.org/10.1561/2200000006},
 publisher = {Now Publishers Inc.},
 address = {Hanover, MA, USA},
 }




@ARTICLE{lle,
TITLE = {Nonlinear dimensionality reduction by locally linear embedding},
AUTHOR = {S. Roweis and L. Saul},
JOURNAL = {Science},
YEAR = {2000},
MONTH = {December},
VOLUME = {290},
NUMBER = {5500},
PAGES = {2323-2326},
}

@ARTICLE{isomap,
TITLE = {A Global Geometric Framework for Nonlinear Dimensionality Reduction},
AUTHOR = {J. Tenenbaum and V. de Silva and J. Langford},
JOURNAL = {Science},
YEAR = {2000},
MONTH = {December},
VOLUME = {290},
NUMBER = {5500},
PAGES = {2319-2323},
}


@INPROCEEDINGS{wang-attributes,
AUTHOR = {Y. Wang and G. Mori},
TITLE = {A {D}iscriminative {L}atent {M}odel of {O}bject {C}lasses and {A}ttributes},
BOOKTITLE = eccv,
YEAR = {2010},
}



@INPROCEEDINGS{auto-context,
  AUTHOR =       {Z. Tu},
  TITLE =        {Auto-context and {I}ts {A}pplication to {H}igh-level {V}ision {T}asks},
  BOOKTITLE =    cvpr,
  YEAR =         {2008},
}


@INPROCEEDINGS{klsh,
AUTHOR = {B. Kulis and K. Grauman},
TITLE = {Kernelized {L}ocality-{S}ensitive {H}ashing for {S}calable {I}mage {S}earch},
BOOKTITLE = iccv,
YEAR = {2009},
}


@INPROCEEDINGS{fastsearch,
AUTHOR = {P. Jain and B. Kulis and K. Grauman},
TITLE = {Fast {I}mage {S}earch for {L}earned {M}etrics},
BOOKTITLE = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
YEAR = {2008},
}



@ARTICLE{brian-pami2009,
TITLE = {Fast {S}imilarity {S}earch for {L}earned {M}etrics},
AUTHOR = {B. Kulis and P. Jain and K. Grauman},
JOURNAL = pami,
YEAR = {2009},
VOLUME = {31},
}


@INPROCEEDINGS{onlinemetric,
TITLE = {Online {M}etric {L}earning and {F}ast {S}imilarity {S}earch},
AUTHOR = {P. Jain and B. Kulis and I. Dhillon and K. Grauman},
BOOKTITLE = nips,
YEAR = {2008},
}


@INPROCEEDINGS{sudheendra-cvpr2008,
title = {Keywords to {V}isual {C}ategories: {M}ultiple-{I}nstance {L}earning for {W}eakly {S}upervised {O}bject {C}ategorization},
author = {S. Vijayanarasimhan and K. Grauman},
booktitle = cvpr,
year = {2008},
}


@INPROCEEDINGS{sonal,
TITLE = {Watch, {L}isten \& {L}earn: {C}o-training on {C}aptioned {I}mages and {V}ideos},
AUTHOR = {S. Gupta and J. Kim and K. Grauman and R. Mooney},
BOOKTITLE = {Proceedings of the European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases (ECML PKDD)},
YEAR = {2008},
}


@inproceedings{tom,
  author    = {Sung Ju Hwang and
               Kristen Grauman and
               Fei Sha},
  title     = {Learning a Tree of Metrics with Disjoint Visual Features},
  booktitle = {NIPS},
  year      = {2011},
  pages     = {621-629},
  ee        = {http://books.nips.cc/papers/files/nips24/NIPS2011_0439.pdf},
  crossref  = {DBLP:conf/nips/2011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@Proceedings{hierarchicaldesc,
  author       = {R. Mittelman and M. Sun and B. Kuipers and S. Savarese},
  title        = {Learning Hierarchical Linguistic Descriptions of Visual Datasets},
  booktitle    = {NAACL-HLT},
  year         = {2013},
}

@INPROCEEDINGS{vaquero,
AUTHOR = {D. Vaquero and R. Feris and L. Brown and A. Hampapur},
TITLE = {Attribute-based {P}eople {S}earch in {S}urveillance {E}nvironments},
BOOKTITLE = wacv,
YEAR = {2009},
}


@INPROCEEDINGS{sudheendra-cvpr2009,
    author = {S. Vijayanarasimhan and K. Grauman},
    title = {What's {I}t {G}oing to {C}ost {Y}ou?: {P}redicting {E}ffort vs. {I}nformativeness for {M}ulti-{L}abel {I}mage {A}nnotations.},
    booktitle = cvpr,
    year = {2009},
}

@INPROCEEDINGS{farhadi-cvpr2009,
AUTHOR = {Ali Farhadi and
               Ian Endres and
               Derek Hoiem and
               David Forsyth},
TITLE = {Describing {O}bjects by their {A}ttributes},
BOOKTITLE = cvpr,
YEAR = {2009},
}

@BOOK{wordnet,
EDITOR = {C. Fellbaum},
TITLE = {Word{N}et An {E}lectronic {L}exical {D}atabase},
YEAR = {1998},
MONTH = {May},
PUBLISHER = {MIT Press},
}

@ARTICLE{kobus-eval,
AUTHOR = {K. Barnard and Q. Fan and R. Swaminathan and A. Hoogs and R. Collins and P. Rondot and J. Kaufhold},
TITLE = {Evaluation of localized semantics: data, methodology, and experiments},
JOURNAL = {International Journal of Computer Vision},
VOLUME = {77},
PAGES = {199--217},
YEAR = {2008},
}


@INPROCEEDINGS{lampert-attributes,
AUTHOR = {Christoph Lampert and Hannes Nickisch and Stefan Harmeling},
TITLE = {Learning To {D}etect {U}nseen {O}bject {C}lasses by {B}etween-{C}lass {A}ttribute {T}ransfer},
BOOKTITLE = {CVPR},
YEAR = {2009},
}


@INPROCEEDINGS{simile,
TITLE = {{Attribute and Simile Classifiers for Face Verification}},
AUTHOR = {N. Kumar and A. Berg  and P. Belhumeur  and S. Nayar},
BOOKTITLE = iccv,
YEAR = {2009},
}


@INPROCEEDINGS{ferrari-attributes,
TITLE = {Learning {V}isual {A}ttributes},
BOOKTITLE = nips,
YEAR = {2007},
AUTHOR = {V. Ferrari and A. Zisserman},
}

@ARTICLE{sudheendra-ijcv2010,
TITLE = {Cost-{S}ensitive {A}ctive {V}isual {C}ategory {L}earning},
AUTHOR = {S. Vijayanarasimhan and K. Grauman},
JOURNAL = ijcv,
YEAR = {2010},
}


@INPROCEEDINGS{sudheendra-cvpr2010,
TITLE = {Far-{S}ighted {A}ctive {L}earning on a {B}udget for {I}mage and {V}ideo {R}ecognition},
AUTHOR = {S. Vijayanarasimhan and P. Jain and K. Grauman},
BOOKTITLE = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
YEAR = {2010},
}


@INPROCEEDINGS{sudheendra-nips2008,
TITLE = {Multi-{L}evel {A}ctive {P}rediction of {U}seful {I}mage {A}nnotations for {R}ecognition},
AUTHOR = {S. Vijayanarasimhan and K. Grauman},
BOOKTITLE = nips,
YEAR = {2008},
}

@INPROCEEDINGS{branson-eccv2010,
AUTHOR = {S. Branson and C. Wah and F. Schroff and B. Babenko and P. Welinder and P. Perona and S. Belongie},
BOOKTITLE = eccv,
YEAR = {2010},
TITLE = {Visual Recognition with Humans in the Loop},
}


@INPROCEEDINGS{sungju-cvpr2010,
AUTHOR = {S. J. Hwang and K. Grauman},
TITLE = {Reading Between The Lines: Object Localization Using Implicit Cues from Image Tags},
BOOKTITLE = cvpr,
YEAR = {2010},
}



@INPROCEEDINGS{sungju-bmvc2010,
AUTHOR = {S. J. Hwang and K. Grauman},
TITLE = {Accounting for the Relative Importance of Objects in Image Retrieval},
BOOKTITLE = bmvc,
YEAR = {2010},
}



@INPROCEEDINGS{qi,
AUTHOR = {G. Qi and X. Hua and Y. Rui and J. Tang and H. Zhang},
TITLE = {Two-Dimensional {A}ctive {L}earning for {I}mage {C}lassification},
BOOKTITLE = cvpr,
YEAR = {2008},
}


@INPROCEEDINGS{fink2004,
TITLE = {Learning from a {S}mall {N}umber of {E}xamples by {E}xploiting {O}bject {C}ategories},
AUTHOR = {K. Levi and M. Fink and Y. Weiss},
BOOKTITLE = {Workshop of Learning in Computer Vision (LCVPR)},
YEAR = {2004},
}



@INPROCEEDINGS{ariadna-transfer,
TITLE = {Transfer {L}earning for {I}mage {C}lassification with {S}parse {P}rototype {R}epresentations},
AUTHOR = {A. Quattoni and M. Collins and T. Darrell},
YEAR = {2008},
BOOKTITLE = cvpr,
}


@INPROCEEDINGS{loeff,
AUTHOR = {N. Loeff and A. Farhadi},
TITLE = {Scene {D}iscovery by {M}atrix {F}actorization},
BOOKTITLE = eccv,
YEAR = {2008},
}

@InProceedings{bart,
Author = "E. Bart and S. Ullman",
Title = "Cross-{G}eneralization: {L}earning {N}ovel {C}lasses from a {S}ingle {E}xample by {F}eature {R}eplacement",
BookTitle = cvpr,
Year = "2005",
}

@INPROCEEDINGS{ariadna-captions,
AUTHOR = {A. Quattoni and M. Collins and T. Darrell},
TITLE = {Learning {V}isual {R}epresentations {U}sing {I}mages with {C}aptions},
BOOKTITLE = cvpr,
YEAR = {2007},
}



@InProceedings{oneshot,
TITLE = {A {B}ayesian {A}pproach to {U}nsupervised {O}ne-{S}hot {L}earning of {O}bject {C}ategories},
AUTHOR = {L. Fei-Fei and R. Fergus and P. Perona},
BOOKTITLE = iccv,
YEAR = {2003},
}

@INPROCEEDINGS{tamara-eccv2010,
YEAR = {2010},
TITLE = {Automatic {A}ttribute {D}iscovery and {C}haracterization from {N}oisy {W}eb {D}ata},
AUTHOR = {T. Berg and A. Berg and J. Shih},
BOOKTITLE = eccv,
}


@INPROCEEDINGS{wang-attributes-bmvc,
TITLE = {Learning {M}odels for {O}bject {R}ecognition from {N}atural {L}anguage {D}escriptions},
BOOKTITLE = bmvc,
YEAR = {2009},
AUTHOR = {J. Wang and K. Markert and M. Everingham},
}

@INPROCEEDINGS{weinshall-novelty,
AUTHOR = {D. Weinshall and H. Hermansky and A. Zweig and J. Luo and H. Jimison and F. Ohl and M. Pavel},
TITLE = {{Beyond Novelty Detection: Incongruent Events, when General and Specific Classifiers Disagree}},
BOOKTITLE = nips,
YEAR = {2008},
}

@INPROCEEDINGS{sivic-hierarchy,
AUTHOR = {J. Sivic and B. Russell and A. Zisserman and W. Freeman and A. Efros},
TITLE = {Unsupervised discovery of visual object class hierarchies},
YEAR = {2008},
BOOKTITLE = cvpr,
}


@INPROCEEDINGS{taxonomy-perona,
AUTHOR = {E. Bart and I. Porteous and P. Perona and M. Welling},
TITLE = {Unsupervised learning of visual taxonomies},
BOOKTITLE = cvpr,
YEAR = {2008},
}

@INPROCEEDINGS{ahuja-taxonomy,
AUTHOR = {N. Ahuja and S. Todorovic},
TITLE = {Learning the taxonomy and models of categories present in arbitrary images},
BOOKTITLE = iccv,
YEAR = {2007},
}

@INPROCEEDINGS{marszalek-hierarchy,
AUTHOR = {Marcin Marszalek and Cordelia Schmid},
TITLE = {Constructing Category Hierarchies for Visual Recognition},
YEAR = {2008},
BOOKTITLE = eccv,
}



@INPROCEEDINGS{miller-transfer,
AUTHOR = {E. Miller and N. Matsakis and P. Viola},
TITLE = {Learning from {O}ne {E}xample through {S}hared {D}ensities on {T}ransforms},
YEAR = {2000},
BOOKTITLE = cvpr,
}





@inproceedings {schiele-eccv2010,
TITLE = {Combining Language Sources and Robust Semantic Relatedness for Attribute-Based Knowledge Transfer},
AUTHOR = {M. Rohrbach and M. Stark and G. Szarvas and B. Schiele},
BOOKTITLE = {Parts and Attributes Workshop},
YEAR = {2010},
}


@inproceedings {rohrbach10cvpr,
YEAR = {2010},
AUTHOR = {M. Rohrbach and M. Stark and G. Szrvas and I. Gurevych and B. Schiele},
TITLE = {What {H}elps {W}here and {W}hy? {S}emantic {R}elatedness for {K}nowledge {T}ransfer},
BOOKTITLE = cvpr,
}




@ARTICLE{antonio-sharing,
TITLE = {Sharing {V}isual {F}eatures for {M}ulticlass and {M}ultiview {O}bject {D}etection},
AUTHOR = {A. Torralba and K. Murphy},
YEAR = {2007},
JOURNAL = {PAMI},
VOLUME = {29},
NUMBER = {5},
}

@INPROCEEDINGS{gangwang-cvpr2010,
TITLE = {Comparative object similarity for improved recognition with few or zero examples},
AUTHOR = {G. Wang and D. Forsyth and D. Hoeim},
BOOKTITLE = cvpr,
YEAR = {2010},
}


@INPROCEEDINGS{xing,
TITLE = {Distance {M}etric {L}earning, with {A}pplication to {C}lustering with {S}ide-{I}nformation},
AUTHOR = {E. Xing and A. Ng and M. Jordan and S. Russell},
BOOKTITLE = nips,
YEAR = {2002},
}


@INPROCEEDINGS{weinberger,
AUTHOR = {K. Q. Weinberger and J. Blitzer and L. Saul},
TITLE = {Distance {M}etric {L}earning for {L}arge {M}argin {N}earest {N}eighbor {C}lassification},
BOOKTITLE = nips,
YEAR = {2006},
}


@INPROCEEDINGS{weinberger08,
author = {K. Q. Weinberger and L. Saul},
title = {Fast {S}olvers and {E}fficient {I}mplementations for {D}istance {M}etric {L}earning},
booktitle = icml,
year = {2008}
}

@INPROCEEDINGS{orthogonal,
author = {D. Zhou and L. Xiao, and M. Wu},
title = {Hierarchical {C}lassification via {O}rthogonal {T}ransfer},
booktitle = icml,
year = {2011}
}

@INPROCEEDINGS{globerson,
AUTHOR = {A. Globerson and S. Roweis},
TITLE = {Metric {L}earning by {C}ollapsing {C}lasses},
BOOKTITLE = nips,
YEAR = {2005},
}


@ARTICLE{rca,
AUTHOR = "A. Bar-Hillel and T. Hertz and N. Shental and D. Weinshall",
TITLE = "Learning a {M}ahalanobis {M}etric from {E}quivalence {C}onstraints",
journal = "Journal of Machine Learning Research",
VOLUME = 6,
pages = "937--965",
month = "June",
YEAR = "2005",
}


@InProceedings{frome07,
AUTHOR = {A. Frome and Y. Singer and F. Sha and J. Malik},
TITLE = {Learning {G}lobally-{C}onsistent {L}ocal {D}istance {F}unctions for {S}hape-{B}ased {I}mage {R}etrieval and {C}lassification},
BOOKTITLE = iccv,
YEAR = {2007},
}


@INPROCEEDINGS{metric-learning,
AUTHOR = {J. Davis and B. Kulis and P. Jain and S. Sra and I. Dhillon},
TITLE = {Information-{T}heoretic {M}etric {L}earning},
BOOKTITLE = icml,
YEAR = {2007},
}


@INPROCEEDINGS{schultz,
TITLE = {Learning a {D}istance {M}etric from {R}elative {C}omparisons},
AUTHOR = {M. Schultz and T. Joachims},
BOOKTITLE = nips,
YEAR = {2003},
}


@ARTICLE{gist,
TITLE = {Contextual {P}riming for {O}bject {D}etection},
AUTHOR = {A. Torralba},
JOURNAL = ijcv,
VOLUME = {53},
NUMBER = {2},
PAGES = {169--191},
YEAR = {2003},
}


@ARTICLE{hoiem,
TITLE = {Putting {O}bjects in {P}erspective},
AUTHOR = {D. Hoiem and A. Efros and M. Hebert},
JOURNAL = ijcv,
VOLUME = {80},
NUMBER = {1},
MONTH = {October},
YEAR = {2008},
}


@INBOOK{murphy,
  AUTHOR =       {K. Murphy and A. Torralba and D. Eaton and W. Freeman},
  TITLE =        {Towards Category-Level Object Recognition},
  CHAPTER =      {Object {D}etection and {L}ocalization {U}sing {L}ocal and {G}lobal {F}eatures},
  PUBLISHER =    {LNCS},
  YEAR =         {2006},
}


@INPROCEEDINGS{verbeek,
AUTHOR = {J. Verbeek and B. Triggs},
TITLE = {Scene {S}egmentation with {C}{R}{F}s {L}earned from {P}artially {L}abeled {I}mages},
BOOKTITLE = nips,
YEAR = {2007},
}


@INPROCEEDINGS{gupta-nips08,
AUTHOR = {A. Gupta and J. Shi and L. Davis},
TITLE = {A {S}hape {A}ware {M}odel for {S}emi-{S}upervised {L}earning of {O}bjects and its {C}ontext},
BOOKTITLE = nips,
YEAR = {2008},
}



@INPROCEEDINGS{galleguillos,
AUTHOR = {C. Galleguillos and A. Rabinovich and S. Belongie},
TITLE = {Object {C}ategorization {U}sing {C}o-{O}ccurrence, {L}ocation and {A}ppearance},
BOOKTITLE = cvpr,
YEAR = {2008},
}


@ARTICLE{gould,
TITLE = {Multi-Class {S}egmentation with {R}elative {L}ocation {P}rior},
AUTHOR = {S. Gould and J. Rodgers and D. Cohen and G. Elidan and D. Koller},
MONTH = {April},
YEAR = {2008},
  journal    = ijcv,
  volume     = {80},
  number     = {3},
  pages      = {300--316},

}

@ARTICLE{sudderth-ijcv2008,
AUTHOR = {E. Sudderth and A. Torralba and W. Freeman and A. Willsky},
TITLE = {Describing {V}isual {S}cenes {U}sing {T}ransformed {O}bjects and {P}arts},
JOURNAL = ijcv,
YEAR = {2008},
VOLUME = {77},
}

@INPROCEEDINGS{feifei-scenes,
AUTHOR = {L.-J. Li and L. Fei-Fei},
TITLE = {What, where and who? Classifying event by scene and object recognition},
BOOKTITLE = iccv,
YEAR = {2007},
}




@inproceedings{malisiewicz-nips09,
  Author =       {T. Malisiewicz and A. Efros},
  Booktitle =    nips,
  Title =        {{Beyond Categories: The Visual Memex Model for Reasoning Abou\
t Object Relationships}},
  Month =        {December},
  Year =         2009,
}

@INPROCEEDINGS{malisiewicz-cvpr2008,
YEAR = {2008},
TITLE = {Recognition by Association via Learning Per-exemplar Distances},
AUTHOR = {T. Malisiewicz and A. Efros},
BOOKTITLE = cvpr,
}




@INPROCEEDINGS{shotton-eccv06,
  AUTHOR =       {J. Shotton and J. Winn and C. Rother and A. Criminisi},
  TITLE =        {TextonBoost: {J}oint {A}ppearance, {S}hape and {C}ontext {M}odeling for
{M}ulti-{C}lass {O}bject {R}ecognition and {S}egmentation},
  BOOKTITLE =    eccv,
  YEAR =         {2006},
}

@INPROCEEDINGS{he-cvpr04,
  AUTHOR =       {X. He and  R. Zemel and M. Carreira-Perpinan},
  TITLE =        {Multiscale {C}onditional {R}andom {F}ields for {I}mage {L}abeling},
  BOOKTITLE =    cvpr,
  YEAR =         {2004},
}


@INPROCEEDINGS{heiz-eccv08,
  AUTHOR =       {G. Heitz and D. Koller},
  TITLE =        {Learning {S}patial {C}ontext: {U}sing {S}tuff to {F}ind {T}hings},
  BOOKTITLE =    eccv,
  YEAR =         {2008},
}

@INPROCEEDINGS{object-graph,
TITLE = {Object-{G}raphs for {C}ontext-{A}ware {C}ategory {D}iscovery},
AUTHOR = {Y. J. Lee and K. Grauman},
BOOKTITLE = cvpr,
YEAR = {2010},
}


@techreport{caltech256,
Author = {G. Griffin and A. Holub and P. Perona},
Title = {Caltech-256 Object Category Dataset},
Institution = {California Institute of Technology},
    Year = {2007},
    URL = {http://authors.library.caltech.edu/7694},
    Number = {7694},
}


@INPROCEEDINGS{sundb,
AUTHOR = {M. J. Choi and J. J. Lim and  A. Torralba and A. S. Willsky},
TITLE = {Exploiting Hierarchical Context on a Large Database of Object Categories},
BOOKTITLE = cvpr,
YEAR = {2010},
}

@INPROCEEDINGS{coredb,
TITLE = {The Benefits and Challenges of Collecting Richer Object Annotations},
AUTHOR = {I. Endres and A. Farhadi and D. Hoiem and D. Forsyth},
BOOKTITLE = {ACVHL in conjunction with CVPR},
YEAR = {2010},
}


@INPROCEEDINGS{imagenet,
AUTHOR = {J. Deng and W. Dong and R. Socher and L.-J. Li and K. Li and L. Fei-F\
ei},
TITLE = {ImageNet: A {L}arge-{S}cale {H}ierarchical {I}mage {D}atabase},
BOOKTITLE = {CVPR},
YEAR = {2009},
}




@INPROCEEDINGS{desai,
AUTHOR = {C. Desai and D. Ramanan and C. Fowlkes},
TITLE = {Discriminative Models for Multi-Class Object Layout},
BOOKTITLE = iccv,
YEAR = {2009},
}


@TECHREPORT{labelme,
  AUTHOR =       {B. Russell and A. Torralba and K. Murphy and W. Freeman},
  TITLE =        {LabelMe: a {D}atabase and {W}eb-{B}ased {T}ool for {I}mage {A}nnotation},
  INSTITUTION =  {MIT},
  YEAR =         {2005},
  }


@INPROCEEDINGS{palatucci,
AUTHOR = {M. Palatucci and D. Pomerleau and G. Hinton and T. Mitchell},
BOOKTITLE = nips,
TITLE = {Zero-{S}hot {L}earning with {S}emantic {O}utput {C}odes},
YEAR = {2009},
}

@INPROCEEDINGS{max-margin-clustering,
TITLE = {Maximum Margin Clustering},
AUTHOR = {L. Xu and J. Neufeld and B. Larson and D. Schuurmans},
BOOKTITLE = nips,
YEAR = {2004},
}


@ARTICLE{ando05,
TITLE = {A {F}ramework for {L}earning {P}redictive {S}tructures from {M}ultiple {T}asks and {U}nlabeled {D}ata},
AUTHOR = {R. Ando and T. Zhang},
JOURNAL = jmlr,
VOLUME = {6},
YEAR = {2005},
}

@INPROCEEDINGS{golland,
AUTHOR = {P. Golland},
TITLE = {Discriminative Direction for Kernel Classifiers},
BOOKTITLE = nips,
YEAR = {2002},
}

@INPROCEEDINGS{indoor,
AUTHOR = {A. Quattoni and A. Torralba},
BOOKTITLE = cvpr,
YEAR = {2009},
TITLE = {Recognizing {I}ndoor {S}cenes},
}

@ARTICLE{outdoor,
TITLE = {Modeling the {S}hape of the {S}cene: a {H}olistic {R}epresentation of the {S}patial {E}nvelope},
AUTHOR = {A. Oliva and A. Torralba},
JOURNAL = ijcv,
VOLUME = {42},
NUMBER = {3},
YEAR = {2001},
}


@misc{pascal,
	author = "Everingham, M. and Van~Gool, L. and Williams, C. K. I. and Winn, J. and Zisserman, A.",
	title = "The {PASCAL} {V}isual {O}bject {C}lasses {C}hallenge 2008 {(VOC2008)} {R}esults",
	howpublished = "http://www.pascal-network.org/challenges/VOC/voc2008/workshop/index.html"}	

@ARTICLE{pedro-2008,
AUTHOR = {P. Felzenszwalb and R. Girshick and D. McAllester and D. Ramanan},
TITLE = {Object Detection with Discriminatively Trained Part Based Models},
JOURNAL = pami,
VOLUME = {32},
NUMBER = {9},
YEAR = {2010},
MONTH = {September},
}


@INPROCEEDINGS{fergus-eccv2010,
TITLE = {Semantic Label Sharing for Learning with Many Categories},
AUTHOR = {R. Fergus and H. Bernal and Y. Weiss and A. Torralba},
BOOKTITLE = eccv,
YEAR = {2010},
}


@ARTICLE{tiny,
TITLE = {80 million {T}iny {I}mages: a {L}arge {D}ataset for {N}on-{P}arametric\
 {O}bject and {S}cene {R}ecognition},
AUTHOR = {A. Torralba and R. Fergus and W. T. Freeman},
JOURNAL = pami,
YEAR = {2008},
VOLUME = {30},
NUMBER = {11},
PAGES = {1958--1970},
}


@InProceedings{fergus03,
  author = "R. Fergus and P. Perona and A. Zisserman",
  title = "Object {C}lass {R}ecognition by {U}nsupervised {S}cale-{I}nvariant {\
L}earning",
  year = "2003",
  BookTitle = cvpr,
   }


@InProceedings{leibe04,
Title = {Combined {O}bject {C}ategorization and {S}egmentation with an {I}mplic\
it {S}hape {M}odel},
Author = {B. Leibe and A. Leonardis and B. Schiele},
BookTitle = {Workshop on Statistical Learning in Computer Vision},
Year = {2004},
}

@INPROCEEDINGS{hog,
AUTHOR = {N. Dalal and B. Triggs},
TITLE = {Histograms of {O}riented {G}radients for {H}uman {D}etection},
BOOKTITLE = cvpr,
YEAR = {2005},
}



@Article{lowe,
  Author         = "D. Lowe",
  Title          = "Distinctive {I}mage {F}eatures from {S}cale-{I}nvariant {K}\
eypoints",
  Journal        = ijcv,
  Volume         = "60",
  Number         = "2",
  year           = 2004,
}


@ARTICLE{yuille,
AUTHOR = {A. Yuille and P. Hallinan and D. Cohen},
TITLE = {Feature {E}xtraction from {F}aces using {D}eformable {T}emplates},
JOURNAL = ijcv,
VOLUME = {8},
NUMBER = {2},
YEAR = {1992},
MONTH = {August},
}

@ARTICLE{aam,
AUTHOR = {T. F. Cootes and C. J. Taylor and D. H. Cooper and J. Graham},
TITLE = {Active shape models-their training and application},
JOURNAL = {Computer Vision and Image Understanding},
VOLUME = {61},
NUMBER = {1},
PAGES = {38--59},
YEAR = {1995},
}

@ARTICLE{schmid-mohr,
AUTHOR = {C. Schmid and R. Mohr},
YEAR = {1997},
TITLE = {Local {G}rayvalue {I}nvariants for {I}mage {R}etrieval},
JOURNAL = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
VOLUME = {19},
NUMBER = {5},
PAGES = {530--534},
}

@INPROCEEDINGS{nister,
  AUTHOR =       {D. Nister and H. Stewenius},
  TITLE =        {Scalable {R}ecognition with a {V}ocabulary {T}ree},
  BOOKTITLE =    cvpr,
  YEAR =         {2006},
 }


@InProceedings{viola,
Author = "P. Viola and M. Jones",
Title = "Rapid {O}bject {D}etection using a {B}oosted {C}ascade of {S}imple {F}\
eatures",
BookTitle = cvpr,
Year = "2001",
}

@Article{rowley,
TITLE = {Neural {N}etwork-{B}ased {F}ace {D}etection},
AUTHOR = {H. Rowley and S. Baluja and T. Kanade},
JOURNAL = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
VOLUME = {20},
NUMBER = {1},
PAGES = {23--38},
MONTH = {January},
YEAR = {1998},
}

@InProceedings{dance,
  Author = "G. Csurka and C. Bray and C. Dance and L. Fan",
  Title = "Visual {C}ategorization with {B}ags of {K}eypoints",
BookTitle = eccv,
Year = "2004",
}

@Article{belongie,
  Author = "S. Belongie and J. Malik and J. Puzicha",
  Title = "Shape {M}atching and {O}bject {R}ecognition {U}sing {S}hape {C}ontex\
ts",
  Journal  = pami,
  Year = 2002,
  Volume = 24,
  Number = 24,
  Pages = "509--522",
}

@INPROCEEDINGS{iccv2005,
  AUTHOR =       {K. Grauman and T. Darrell},
  TITLE =        {The {P}yramid {M}atch {K}ernel: {D}iscriminative {C}lassifica\
tion with {S}ets of {I}mage {F}eatures},
  BOOKTITLE =    iccv,
  YEAR =         {2005},
}


@INPROCEEDINGS{lana-cvpr06, AUTHOR = {S. Lazebnik and C. Schmid and
J. Ponce}, TITLE = {Beyond {B}ags of {F}eatures: {S}patial {P}yramid
{M}atching for {R}ecognizing {N}atural {S}cene {C}ategories},
BOOKTITLE = cvpr, YEAR = 2006, }



@InProceedings{lecun06,
AUTHOR = {F. Huang and Y. LeCun},
TITLE = {Large-scale {L}earning with {S}{V}{M} and {C}onvolutional for {G}eneri\
c {O}bject {C}ategorization},
BOOKTITLE = cvpr,
YEAR = {2006},
}



@INPROCEEDINGS{gu,
TITLE = {Recognition using regions},
BOOKTITLE = cvpr,
YEAR = {2009},
AUTHOR = {C. Gu and J. Lim and P. Arbelaez and J. Malik},
}

@INPROCEEDINGS{siftflow,
AUTHOR = {C. Liu and J. Yuen and A. Torralba and J. Sivic and W. Freeman},
BOOKTITLE = eccv,
YEAR = {2008},
TITLE = {S{I}{F}{T} flow: dense correspondence across different scenes},
}


@INPROCEEDINGS{gould-iccv09,
  AUTHOR    = {S. Gould and R. Fulton and D. Koller},
  TITLE     = {Decomposing a {S}cene into {G}eometric and {S}emantically {C}onsistent {R}egions},
  BOOKTITLE = iccv,
  YEAR      = {2009}
}
@INPROCEEDINGS{holub-iccv2005,
TITLE = {Combining Generative Models and Fisher Kernels for Object Recognition},
AUTHOR = {A. Holub and M. Welling and P. Perona},
BOOKTITLE = iccv,
YEAR = {2005},
}

@ARTICLE{ullman-2002,
AUTHOR = {S. Ullman and  M. Vidal-Naquet and  E. Sali},
TITLE = {Visual Features of Intermediate Complexity and their Use in Classification},
JOURNAL = {Nature Neuroscience},
VOLUME = {5},
PAGES = {682--7},
YEAR = {2002},
}

@INPROCEEDINGS{zhang-hybrid,
AUTHOR = {D. Zhang and S.-F. Chang},
TITLE = {A Generative-Discriminative Hybrid Method for Multi-View Object Detection},
BOOKTITLE = cvpr,
YEAR = {2006},
}

@INPROCEEDINGS{fritz-iccv2005,
AUTHOR = {M. Fritz and B. Leibe and B. Caputo and B. Schiele},
TITLE = {Integrating Representative and Discriminant Models for Object Category Detection},
BOOKTITLE = iccv,
YEAR = {2005},
}


@INPROCEEDINGS{fink-icml2007,
TITLE = {Uncovering {S}hared {S}tructures in {M}ulticlass {C}lassification},
AUTHOR = {Y. Amit and M. Fink and N. Srebro and S. Ullman},
BOOKTITLE = {ICML},
YEAR = {2007},
}


@INPROCEEDINGS{stark-iccv2009,
TITLE = {A {S}hape-based {O}bject {C}lass {M}odel for {K}nowledge {T}ransfer},
AUTHOR = {M. Stark and M. Goesele and B. Schiele},
BOOKTITLE = iccv,
YEAR = {2009},
}


@InProceedings{weber,
AUTHOR = {M. Weber and M. Welling and P. Perona},
TITLE = {Unsupervised {L}earning of {M}odels for {R}ecognition},
BOOKTITLE = eccv,
YEAR = {2000},
}


@ARTICLE{saxena,
TITLE = {Make3{D}: Learning 3-D Scene Structure from a Single Still Image},
AUTHOR = {A. Saxena and M. Sun and A. Ng},
JOURNAL = pami,
YEAR = {2008},
}

@INPROCEEDINGS{gangwang-iccv2009,
AUTHOR = {G. Wang and D. Forsyth},
TITLE = {Joint {L}earning of {V}isual {A}ttributes {O}bject {C}lasses and {V}isual {S}alience},
BOOKTITLE = iccv,
YEAR = {2009},
}

@ARTICLE{mimic3_ref,
AUTHOR = {Alistair E.W. Johnson and Tom J. Pollard and Lu Shen and Li-wei H. Lehman and Mengling Feng and Mohammad Ghassemi and Benjamin Moody and Peter Szolovits and Leo Anthony Celi and Roger G. Mark},
TITLE = {Mimic-iii, a freely accessible critical care database},
BOOKTITLE = Scientific Data,
YEAR = {2016},
}

@ARTICLE{Olshausen,
AUTHOR = {B. Olshausen and D. Field},
TITLE = {Emergence of {S}imple-{C}ell {R}eceptive {F}ield {P}roperties by {L}earning a {S}parse {C}ode for {N}atural {I}mages},
JOURNAL = {Nature},
VOLUME = {381},
PAGES = {607--609},
YEAR = {1996},
}

@INPROCEEDINGS{yuan2010,
AUTHOR = {X.-T. Yuan and S. Yan},
TITLE = {Visual {C}lassification with {M}ulti-{T}ask {J}oint {S}parse {R}epresentation},
BOOKTITLE = cvpr,
YEAR =  {2010},
}

@INPROCEEDINGS{ahmed2008,
AUTHOR = {A. Ahmed and K. Yu and W. Xu and Y. Gong and E. Xing},
TITLE = {Training {H}ierarchical {F}eed-{F}orward {V}isual {R}ecognition {M}odels using {T}ransfer {L}earning from {P}seudo-{T}asks},
BOOKTITLE = eccv,
YEAR = {2008},
}

@article{argyriou08,
author= {Andreas Argyriou, and Theodoros Evgeniou, and Massimiliano Pontil},
title={Convex {M}ulti-task {F}eature {L}earning},
journal={Machine Learning},
volume={73},
number={3},
pages={243--272},
year={2008}
}

@INPROCEEDINGS{argyriou-nips06,
TITLE = {Multi-{T}ask {F}eature {L}earning},
AUTHOR = {A. Argyriou and T. Evgeniou and M. Pontil},
BOOKTITLE = nips,
YEAR = {2006},
}

@ARTICLE{caruana97,
AUTHOR = {R. Caruana},
TITLE = {Multitask {L}earning},
JOURNAL = {Machine Learning},
YEAR = {1997},
}

@ARTICLE{osherson,
AUTHOR = {D. Osherson and J. Stern and O. Wilkie and M. Stob and E. Smith},
TITLE = {Default {P}robability},
JOURNAL = {Cognitive Science},
VOLUME = {15},
YEAR = {1991},
NUMBER = {2},
}

@ARTICLE{crammer01,
AUTHOR = {K. Crammer and Y. Singer},
TITLE = {On the {A}lgorithmic {I}mplementation of {M}ulti-class {S}{V}{M}s},
JOURNAL = jmlr,
YEAR = {2001},
}

@ARTICLE{yuan07,
AUTHOR = {M. Yuan  and Y. Lin},
YEAR = {2007},
TITLE = {Model {S}election and {E}stimation in {R}egression with {G}rouped {V}ariables},
JOURNAL = {Journal of the Royal Statistics Socieity},
VOLUME = {68},
NUMBER = {1},
PAGES = {49-�67},
}

@ARTICLE{obozinski09,
TITLE = {Joint {C}ovariate {S}election and {J}oint {S}ubspace {S}election for {M}ultiple {C}lassification {P}roblems},
AUTHOR = {G. Obozinksi and B. Taskar and M. Jordan},
JOURNAL = {Stat Comput},
YEAR = {2009},
}


@Manual{libsvm,
  author =	 {C. C. Chang and C. J. Lin},
  title =	 {LIBSVM: A Library for Support Vector Machines},
  year =	 {2011},
	journal = {ACM Transactions on Intelligent Systems and Technology}
}

@BOOK{wahba90,
AUTHOR = {G. Wahba},
TITLE = {Spline {M}odels for {O}bservational {D}ata},
YEAR = {1990},
}


@article{NRWY12,
    author = "S. Negahban and P. Ravikumar and M. J. Wainwright and B. Yu",
	title = "A unified framework for high-dimensional analysis of {M}-estimators with decomposable regularizers",
	journal = "Statistical Science",
	volume = "27",
	Number = "4",
	pages = "538--557",
	year = "2012"
}


@article{Lipton16,
  author    = {Zachary Chase Lipton and
               David C. Kale and
               Charles Elkan and
               Randall C. Wetzel},
  title     = {Learning to Diagnose with {LSTM} Recurrent Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1511.03677},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.03677},
  archivePrefix = {arXiv},
  eprint    = {1511.03677},
  timestamp = {Wed, 07 Jun 2017 14:40:10 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LiptonKEW15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article {Goldbergere215,
	author = {Goldberger and Ary L. and Amaral, Luis A. N. and Glass, Leon and Hausdorff, Jeffrey M. and Ivanov, Plamen Ch. and Mark, Roger G. and Mietus, Joseph E. and Moody, George B. and Peng, Chung-Kang and Stanley, H. Eugene},
	title = {PhysioBank, PhysioToolkit, and PhysioNet},
	volume = {101},
	number = {23},
	pages = {e215--e220},
	year = {2000},
	journal = {Circulation}
}

==> related.tex <==
\section{Related Work}

\paragraph{Prediction reliability}
There has been work on building a \emph{reliable} deep learning model\cite{timeseries_uncertainty_uber,bayesian_segnet,what_uncertainty}; that is, a deep network that can avoid making incorrect predictions when it is not sufficiently certain about its prediction. To achieve this goal, a model should know the limitation in the data, and in itself. One way to quantify such limitations is by measuring the \emph{predictive uncertainty} using Bayesian models. Recently, \cite{dropout_as_bayesian, rnn_dropout, cnn_dropout} showed that deep networks with dropout sampling \cite{dropout} can be understood as Bayesian neural networks. To obtain better calibrated dropout uncertainties, \cite{variational_dropout,concrete_dropout} proposed to automatically learn the dropout rates with proper reparameterization tricks \cite{concrete_distribution, vae}. While the aformentioned work mostly focus on accurate calibration of uncertainty itself, \cite{what_uncertainty} utilized dropout sampling to model predictive uncertainty in computer vision \cite{bayesian_segnet}, and also modeled label noise with learned variances, to implicitly attenuate loss for the highly uncertain instances. Our work has similar motivation, but we model the uncertainty in the \emph{input data} rather than in labels. By doing so, we can accurately calibrate deep networks for improved reliability. \cite{input_uncertainty_augmentation} has a similar motivation to ours, but with different applications and approaches. 
%There exists quite a few work on this topic recently~\cite{guo17,deep_ensembles}.
There exists quite a few work about uncertainty calibration and its quantification.
\cite{guo17} showed that the modern deep networks are poorly calibrated despite their accuracies, and proposed to tune factors such as depth, width, weight decay for better calibration of the model, and~\cite{deep_ensembles} proposed ensemble and adversarial training for the same objective. 

%which allows easy interpretation of the complex deep learning models via the learned attentions. Choi et al. mainly focus on this interpretability of the attention 

\paragraph{Attention mechanism}
%Attention mechanism~\cite{Bahdanau15} is an approach to adaptively select only the partial set of features (or inputs) for each input, such that the model input-adaptively focuses on more relevant features for prediction. 
The literature on the attention mechanism is vast, which includes its application to machine translation~\cite{Bahdanau15}, memory-augmented networks~\cite{e2ememnet}, and for image annotation~\cite{show_attend_tell}. Attention mechanisms are also used for interpretability, as in Choi et al.~\cite{retain} which proposed a RNN-based attention generator for EHR that can provide attention on both the hospital visits and variables for further analysis by clincians. Attentions can be either deterministic or probabilistic, and soft (non-sparse) or hard (sparse). Some probabilistic attention models~\cite{show_attend_tell} use variational inference as used in our model. However, while their direct learning of multinoulli distribution only considers whether to attend or not without consideration of variance, our attention mechanism models varying degree of uncertainty for each input by input-dependent learning of attention noise (variance).

%\paragraph{Variational inference for DNNs}
%Variational inference~\cite{peterson87} is a technique to solve intractable posterior estimation problem by fitting a parametric distribution to it. Finding its optimal parameter then can be done by maximizing the evidence lower bound (ELBO), but obtaining analytic solutions is difficult for complex models such as deep networks. To tackle this challenge, \cite{vae} recently proposed a reparametrization trick that enables to solve ELBO with stochastic gradient descent. \cite{cvae} proposed a conditional variational inference framework, which learns the parametric distribution $q$ conditioned on the input data and the label. Our model uses this conditional framework as the attention should be generated input-adaptively for each given data instance.

\paragraph{Risk analysis from electronic health records} Our work is mainly motivated by the needs of performing reliable risk prediction with electronic health records. There exists plentiful prior work on this topic, but to mention a few, Choi et al.~\cite{retain} proposed to predict heart failure risk with attention generating RNNs and Futoma et al.~\cite{futoma17} proposed to predict sepsis using RNN, preprocssing the input data using multivariate GP to resolve uneven spacing and missing entry problems. %This can be viewed as another way of input-level uncertainty modeling, while still orthogonal to our work.

==> reliability_diagram.tex <==
%\begin{wrapfigure}{r}{0.5\textwidth}
    %\centering
%    \vspace{-0.6in}
%    \subfigure[RETAIN]{\includegraphics[height=0.455\linewidth]{figure/RETAIN_reliability.pdf}\label{RETAIN}}
%    \hfill
%    \subfigure[SA]{\includegraphics[height=0.455\linewidth]{figure/SA_reliability.pdf}\label{SA}}
%	\hfill
%    \subfigure[UA]{\includegraphics[height=0.455\linewidth]{figure/UA_reliability.pdf}\label{UA}}	    
%    \vspace{-0.1in}
%    \caption{\small Reliability diagrams on Physio-Mortality task.}

    %\caption{\small Uncertainty over prediction strength on PhysioNet Challenge dataset. For both models, we measured the prediction uncertainty by using MC-dropout with $30$ samples}
%    \label{model}
%    \vspace{-0.1in}
%\end{wrapfigure}



\begin{figure*}[ht!]
\vspace{-0.1in}
\begin{center}
\small
\begin{tabular}{c c c}
\includegraphics[width=2.8cm]{figure/RETAIN_reliability.pdf}&
\hspace{0.3in}
\includegraphics[width=2.8cm]{figure/SA_reliability.pdf}&
\hspace{0.3in}
\includegraphics[width=2.8cm]{figure/UA_reliability.pdf}\\
(a) Deterministic Attention~\cite{retain} & (b) Stochastic Attention~\cite{show_attend_tell} & (c) Uncertainty-aware Attention (Ours) \\
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\small Reliability diagrams~\cite{guo17} which shows the accuracy as a function of model confidence, generated from RNNs trained for mortality risk analysis from ICU records (PhysioNet-Mortality). ECE~\cite{ece} in \eqref{eq:ece} denotes Expected Calibration Error, which is 
%a measure of calibration accuracy.
the weighted-average gap between model confidence and actual accuracy. (Gap is shown in green bars.)
Conventional attention models result in poorly calibrated networks while our UA yields a well-calibrated one. Such accurately calibrated networks allow us to perform reliable prediction by leveraging prediction confidence to decide whether to predict or defer prediction.}\label{fig:reliability_diagram}
\vspace{-0.2in}
\end{figure*}

==> sepsis_feature_table.tex <==
\begin{table*}[t]
\small
\vspace{-0.3in}
\begin{center}
\label{tbl:sepsis_feature_table}
\caption{Feature information of MIMIC-Sepsis dataset.}
\vspace{0.1in}
\begin{tabular}{|l|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}\textbf{Features}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Item-ID}}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Name of Item}}                                                                                                                                                              \\ \hline
Age                                                             & N/A                                                                                 & \begin{tabular}[c]{@{}l@{}}intime\\ dob\end{tabular}                                                                                                                                                                            \\ \hline
Heart rate                                                      & \begin{tabular}[c]{@{}l@{}}211\\ 22045\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}Heart Rate\\ Heart Rate\end{tabular}                                                                                                                                                                 \\ \hline
FiO2                                                            & \begin{tabular}[c]{@{}l@{}}223835\\ 3420\\ 3422\\ 190\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}Inspired O2 Fraction\\ FiO2\\ FiO2 {[}Meas{]}\\ FiO2 set\end{tabular}                                                                                                                                \\ \hline
Temperature                                                     & \begin{tabular}[c]{@{}l@{}}676\\ 678\\ 223761\\ 223762\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}Temperature C\\ Temperature F\\ Temperature Fahrenheit\\ Temperature Celsius\end{tabular}                                                                                                            \\ \hline
Systolic Blood Pressure                                         & \begin{tabular}[c]{@{}l@{}}51\\ 442\\ 455\\ 6701\\ 220179\\ 220050\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Arterial BP{[}Systolic{]}\\ Manual BP{[}Systolic{]}\\ NBP{[}Systolic{]}\\ Arterial BP \#2 {[}Systolic{]}\\ Non Invasive Blood Pressure{[}systolic{]}\\ Arterial Blood Pressure{[}systolic{]}\end{tabular}   \\ \hline
Diastolic Blood Pressure                                        & \begin{tabular}[c]{@{}l@{}}8368\\ 8440\\ 8441\\ 8555\\ 220051\\ 220180\end{tabular} & \begin{tabular}[c]{@{}l@{}}Arterial BP{[}Diastolic{]}\\ Manual BP{[}Diastolic{]}\\ NBP{[}Diastolic{]}\\ Arterial BP \#2{[}Diastolic{]}\\ Non Invasive Blood Pressure{[}Diastolic{]}\\ Arterial Blood Pressure{[}Diastolic{]}\end{tabular} \\ \hline
PaO2                                                            & \begin{tabular}[c]{@{}l@{}}50821\\ 50816\end{tabular}                               & \begin{tabular}[c]{@{}l@{}}PO2\\ Oxygen\end{tabular}                                                                                                                                                                            \\ \hline
GCS - Verbal Response                                           & 223900                                                                              & Verbal Response                                                                                                                                                                                                                 \\ \hline
GCS - Motor Response                                            & 223901                                                                              & Motor Response                                                                                                                                                                                                                  \\ \hline
GCS - Eye Opening                                               & 220739                                                                              & Eye Opening                                                                                                                                                                                                                     \\ \hline
Serum Urea Nitrogen Level                                       & 51006                                                                               & Urea Nitrogen                                                                                                                                                                                                                   \\ \hline
Sodium Level                                                    & 950824                                                                              & Sodium Whole Blood                                                                                                                                                                                                              \\ \hline
White Blood Cells Count                                         & \begin{tabular}[c]{@{}l@{}}51300\\ 51301\end{tabular}                               & \begin{tabular}[c]{@{}l@{}}WBC Count\\ White Blood Cells\end{tabular}                                                                                                                                                           \\ \hline
Urine Output                                                    & \begin{tabular}[c]{@{}l@{}}40055\\ 43175 \\ 40069 \\ 40094 \\ 40715 \\40473 \\ 40085 \\ 40057 \\ 40056 \\ 40405 \\ 40428 \\ 40086 \\ 40096 \\ 40651 \\ 226559 \\ 226560 \\ 226561 \\ 226584 \\ 226563 \\ 226564 \\ 226565 \\ 226567 \\ 226557 \\ 226558 \\ 227488 \\ 227489 \end{tabular}                                        & \begin{tabular}[c]{@{}l@{}}Urine Out Foley \\ Urine \\ Urine Out Void \\ Urine Out Condom Cath \\ Urine Out Suprapubic \\ Urine Out IleoConduit \\ Urine Out Incontinent \\ Urine Out Rt Nephrostomy \\ Urine Out Lt Nephrostomy \\ Urine Out Other \\ Urine Out Straight Cath \\ Orine Out Incontinent \\ Urine Out Ureteral Stent $\#$1 \\ Urine Out Ureteral Stent $\#$2 \\ Foley \\ Void \\ Condom Cath \\ Ileoconduit \\ Suprapubic \\ R Nephrostomy \\ L Nephrostomy \\ Straight Cath \\ R Ureteral Stent \\ L Ureteral Stent \\ GU Irrigant Volumne In \\ GU Irrigant/Urine Volume Out\end{tabular} \\ \hline
\end{tabular}
\end{center}
\end{table*}


==> strings.tex <==
@string{wacv = "IEEE Workshop on the Applications of Computer Vision"}
@string{cikm = "ACM International Conference on Information and Knowledge Management"}
@string{jair = "Journal of Artificial Intelligence Research"}
@string{aaai = "Proceedings of the AAAI Conference on Artificial Intelligence"} 
@string{ai= "Artificial
Intelligence"} @string{berk = "University of California Berkeley"}
@string{biocyb = "Biological Cybernetics"} @string{cmu =
"Carnegie-Mellon University"} @string{cacm = "Communications of the
ACM"} @string{capami = "Proc. 1987 Workshop on Comp. Arch. for Patt.
Anal. and Mach. Intell."} @string{vs99 = "Second IEEE Workshop on
Visual Surveillance"} @string{computer = "IEEE Computer"}
@string{cgip = "Computer Graphics and Image Processing"}
@string{cvgip = "Computer Vision, Graphics, and Image Processing"}
@string{cviu = "Computer Vision and Image Understanding"}
@string{cvpr = "IEEE Conference on Computer Vision and Pattern Recognition (CVPR)"} 
@string{focs = "Proceedings Symposium on
Foundations of Comp. Sci."} @string{iccv = "International Conference on Computer Vision (ICCV)"} @string{icpp =
"Proceedings Int. Conf. on Parallel Processing"} @string{icpr =
"International Conference on Pattern Recognition"} @string{ieee =
"Proceedings  of the IEEE"} @string{ijcai = "International Joint Conferences on Artificial Intelligence (IJCAI)"}
@string{ijcv = "International Journal of Computer Vision"} @string{iu = "Proceedings Image Understanding
Workshop"} @string{josa = "Journal of the Optical Society of
America"} @string{jrr = "International Journal of Robotics
Research"} @string{mit = "Massachusetts Institute of Technology"}
@string{bmvc = "Proceedings of the British Machine Vision Conference"}
@string{mitai = "Artificial Intelligence Laboratory, Massachusetts
Institute of Technology"} @string{opteng = "Optical Engineering"}
@string{pami = "Transactions of Pattern Analysis and Machine Intelligence"} @string{patt = "Proceedings Int. Conf. on Pattern
Recognition"} @string{pnas = "Proceedings of the National Academy of
Science"} @string{pr = "Pattern Recognition"} @string{prip =
"Proceedings of IEEE Computer Society Conference on Pattern
Recognition and Image Processing"} @string{prsl = "Proceedings of
the  Royal Society of London"} @string{prslb = "Proceedings of the
Royal Society of London B"} @string{robau = "Proceedings of IEEE
Conference on Robotics and Automation"} @string{sciam = "Scientific
American"} @string{siam = "SIAM J. Comp."} @string{stoc =
"Proceedings ACM Symposium on Theory of Computing"} @string{tmc =
"Thinking Machines Corporation"} @string{visres = "Vision Research"}
@string{jcogneuro = "Journal of Cognitive Neuroscience"}
@string{jexppsych = "Journal of Experimental Psychology"}
@string{annrevneuro = "Annual Review of Neuroscience"}
@string{Ailab = "MIT Artificial Intelligence Laboratory"}
@string{media-vision = "MIT Media Laboratory Vision and Modeling Group"}
@string{aaai-87 = "Sixth National Conference on Artificial Intelligence"}
@string{bbs = "Brain and Behavioral Sciences"}
@string{belknap = "The Belknap Press of Harvard University Press"}
@string{mit = "Massachusetts Institute of Technology"}
@string{mitpress = "MIT Press"}
@string{ieee-proc = "Proceedings of the IEEE"}
@string{ieee-ra = "IEEE Journal of Robotics and Automation"}
@string{ieee-ra-86 = "The 1986 IEEE Conference an Robotics and Automation"}
@string{ieee-smc = "IEEE Transactions on Systems, Man, and Cybernetics"}
@string{ieee-com = "IEEE Transactions on Communications"}
@string{ieee-nn = "IEEE Transactions on Neural Networks"}
@string{ijcai-87 = "Tenth International Joint Conference on Artificial Intelligence"}
@string{umass = "University of Massachusetts at Amherst"}
@string{nips = "Neural Information Processing Systems (NIPS)"}
@string{Tnips2 = "Advances in Neural Information Processing 2"}
@string{Tnips3 = "Advances in Neural Information Processing 3"}
@string{Tnips4 = "Advances in Neural Information Processing 4"}
@string{Tnips5 = "Advances in Neural Information Processing 5"}
@string{Tnips6 = "Advances in Neural Information Processing 6"}
@string{jneusci= "Journal of Neuroscience"}
@string{icsi = "Internation Computer Science Institute"}
@string{neuropros = "Placed in the Neuroprose archive."}
@string{aaaisymp93 = "AAAI Fall Symposium Series Working Notes"}
@string{colt = "Proceedings of the Conference on Computational Learning Theory"}
@string{ACM = "Association for Computing Machinery"}
@string{FG = "Proceedings of the Int. Conf. on Automatic Face \& Gesture Recognition"}
@string{eccv = "European Conference on Computer Vision (ECCV)"}
@string{icml = "International Conference on Machine Learning (ICML)"}
@string{humot = "IEEE Human Motion Workshop"}
@string{jasa = "Journal of American Statistical Association"}
@string{jmlr = "Journal of Machine Learning Research"}
@string{ecml = "Proceedings of the European Conference on Machine Learning"}
@string{chi = "CHI"}

==> uncertainty.tex <==
\begin{figure*}[t]
\vspace{-0.2in}
%\small
\begin{tabular}{c c c}
\hspace{-0.25in}
\includegraphics[height=5cm, width=5.2cm]{figure/retain_uncertainty.png}&
\hspace{-0.35in}
\includegraphics[height=5cm, width=5.2cm]{figure/uca_uncertainty.png}&
\hspace{-0.35in}
\includegraphics[height=5cm, width=5.2cm]{figure/uca_output_uncertainty.png}\\
\hspace{-0.30in} (a)RETAIN&(b)UA &(c)UA+ \\
\end{tabular}
\caption{\small Uncertainty over prediction strength on PhysioNet Challenge dataset. For all models, we measured the prediction uncertainty by using MC-dropout with $30$ samples.}\label{fig:uncertainty}
\end{figure*}


%\begin{wrapfigure}{r}{0.5\textwidth}
%    %\centering
%    \vspace{-0.55in}
%    \subfigure[RETAIN]{\includegraphics[height=0.455\linewidth]{figure/retain_uncertainty.png}\label{RETAIN}}
%    \hfill
%    \subfigure[UA+]{\includegraphics[height=0.455\linewidth]{figure/uca_output_uncertainty}\label{UCA}}
%    \vspace{-0.15in}
%    \caption{\small Uncertainty over prediction strength on PhysioNet Challenge dataset.}
%
    %\caption{\small Uncertainty over prediction strength on PhysioNet Challenge dataset. For both models, we measured the prediction uncertainty by using MC-dropout with $30$ samples}
%    \label{model}
%    \vspace{-0.1in}
%\end{wrapfigure}
